Machine Learning Hamiltonians are Accurate Energy-Force Predictors

Recently, machine learning Hamiltonian (MLH) models have gained traction as fast approximations of electronic structures such as orbitals and electron densities, while also enabling direct evaluation of energies and forces from their predictions. However, despite their physical grounding, existing Hamiltonian models are evaluated mainly by reconstruction metrics, leaving it unclear how well they perform as energy-force predictors. We address this gap with a benchmark that computes energies and forces directly from predicted Hamiltonians. Within this framework, we propose QHFlow2, a state-of-the-art Hamiltonian model with an SO(2)-equivariant backbone and a two-stage edge update. QHFlow2 achieves $40\%$ lower Hamiltonian error than the previous best model with fewer parameters. Under direct evaluation on MD17/rMD17, it is the first Hamiltonian model to reach NequIP-level force accuracy while achieving up to $20\times$ lower energy MAE. On QH9, QHFlow2 reduces energy error by up to $20\times$ compared to MACE. Finally, we demonstrate that QHFlow2 exhibits consistent scaling behavior with respect to model capacity and data, and that improvements in Hamiltonian accuracy effectively translate into more accurate energy and force computations.

==> 3_1_explain.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% PAPER ANALYSIS - SECTION 3.1 (EXPLAIN)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% STRENGTHS:
% + The commented content shows good thinking about SCF-free challenges
% + Covers important concepts: orbital ordering sensitivity, subspace stability
%
% WEAKNESSES:
% - ENTIRE SECTION IS COMMENTED OUT - this is a major structural issue
% - The insights here are valuable but not appearing in the paper
% - Motivation for why "accurate Hamiltonian -> good E/F" is not explained
%
% STRUCTURAL SUGGESTIONS:
% [S1] CRITICAL: Decide if this section should be included or removed
% [S2] If kept, this content provides key motivation for why accuracy matters
% [S3] Could be condensed into a "Why Hamiltonian Accuracy Matters" subsection
% [S4] The orbital ordering sensitivity concept is important - include it
%
% STORYLINE NOTES:
% This file appears to be a placeholder for explaining why accurate
% Hamiltonian prediction is challenging/important for energy/force
% evaluation. The commented content discusses sensitivity to orbital
% ordering and subspace stabilization - these are valuable insights
% that should appear somewhere in the paper to support the main claim.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% \section{Toward SCF-Free DFT}

% \subsection{Problem Formulation}

% Let $\mathbf H^\star = \mathcal H(\mathbf C^\star)$ denote the converged
% KS Hamiltonian obtained by the SCF procedure, with corresponding
% orbitals $\mathbf C^\star$ and occupied index set $\mathcal O^\star$.
% In standard KS-DFT, physical observables are evaluated from $\mathbf C^\star$
% and the induced electron density.

% In the \emph{SCF-free} setting, we instead assume access to a predicted
% Hamiltonian $\hat{\mathbf H}$ and perform a single generalized eigendecomposition
% \begin{equation}
%     \hat{\mathbf H}\hat{\mathbf C}
%     =
%     \mathbf S \hat{\mathbf C}\hat{\boldsymbol{\epsilon}},
% \end{equation}
% from which orbital occupations $\hat{\mathcal O}$ are determined by eigenvalue
% ordering of $\hat{\mathbf{\epsilon}}$. All observables are then evaluated directly from $\hat{\mathbf C}$ and $\hat{\mathbf{\epsilon}}$, without iterative refinement of the Hamiltonian.

% The SCF-free problem can therefore be stated as follows:
% \emph{under what conditions does a single predicted Hamiltonian
% $\hat{\mathbf H}$ induce orbitals and occupations that are sufficiently close
% to those of $\mathbf H^\star$ to yield accurate energies and forces?}


% \subsection{Sensitivity to Orbital Ordering}

% In SCF-free DFT, orbital occupations are determined solely by the ordering of
% generalized eigenvalues $\{\hat{\epsilon}_i\}$.
% For Hamiltonians with small spectral gaps, perturbations $\Delta \mathbf H$ may
% change the relative ordering of near-degenerate eigenvalues, yielding a different
% occupied set $\hat{\mathcal O} \neq \mathcal O^\star$.

% Since the electron density is defined as
% \begin{equation}
%     \hat{\rho}(\mathbf r)
%     =
%     \sum_{i \in \hat{\mathcal O}} |\hat{\psi}_i(\mathbf r)|^2,
% \end{equation}
% such changes induce discontinuous variations in the density that are not controlled
% by entry-wise proximity between $\hat{\mathbf H}$ and $\mathbf H^\star$.

% Consequently, spectral accuracy alone is insufficient to characterize the
% usefulness of a predicted Hamiltonian in the SCF-free regime.

% \subsection{Loss of Subspace Stabilization}

% The SCF procedure enforces stationarity of the energy with respect to orbital
% rotations, which implies vanishing occupied--virtual coupling at convergence
% (Section~\ref{sec:preliminaries}).
% This iterative process stabilizes the occupied subspace
% $\mathrm{span}(\mathbf C_{\mathrm{occ}}^\star)$ under updates of the Hamiltonian.

% In contrast, the SCF-free setting admits no such corrective mechanism.
% Given $\hat{\mathbf H} = \mathbf H^\star + \Delta \mathbf H$, even small
% perturbations $\Delta \mathbf H$ may induce nonzero occupied--virtual couplings
% with respect to the SCF reference subspace,
% \begin{equation}
%     (\mathbf C_{\mathrm{occ}}^\star)^\top
%     \hat{\mathbf H}
%     \mathbf C_{\mathrm{virt}}^\star
%     \;\neq\;
%     \mathbf 0,
% \end{equation}
% leading to rotations of the occupied subspace after diagonalization.

% As a result, SCF-free DFT is inherently sensitive to perturbations that alter the
% \emph{subspace structure} of the Hamiltonian, rather than merely its entry-wise
% values.


% \subsection{Implications for Hamiltonian Learning}

% Entry-wise regression of Hamiltonian matrices,
% \begin{equation}
%     \mathcal L_{\mathrm{entry}}
%     =
%     \|\hat{\mathbf H} - \mathbf H^\star\|,
% \end{equation}
% provides a natural and scalable supervision signal.
% However, in the SCF-free setting, small values of
% $\mathcal L_{\mathrm{entry}}$ do not imply preservation of the occupied subspace
% or the induced density.

% This observation implies that SCF-free Hamiltonian prediction cannot be fully
% characterized by the choice of loss function alone.
% Instead, the structure of the hypothesis class—namely, how Hamiltonian entries
% are coupled and constrained—plays a central role in determining whether
% entry-wise supervision yields physically usable Hamiltonians.

% \subsection{Design-Space Perspective}

% Taken together, SCF-free DFT imposes requirements that are absent in SCF-based
% workflows: a predicted Hamiltonian must induce a stable occupied subspace and a
% consistent electron density under a single diagonalization.

% In the following sections, we analyze architectural design choices for learning
% Hamiltonians under these constraints. We focus on how symmetry-aware and structured models can compensate for the absence of iterative self-consistency while retaining entry-wise supervision.

==> 3_prelim_new.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% PAPER ANALYSIS - PRELIMINARIES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% STRENGTHS:
% + Covers DFT and equivariance background appropriately for ML audience
% + Good use of equations with clear notation
% + Irreps explanation is accessible and well-structured
% + Connects Hamiltonian symmetry to model design motivation
%
% WEAKNESSES:
% - Missing: How energy/force are computed from H (critical for main claim)
% - The connection between preliminaries and the method is implicit
% - Section 3.2 on symmetry could be shorter or integrated into method
% - Appendix references are placeholders (XXX)
%
% STRUCTURAL SUGGESTIONS:
% [S1] Add a subsection on "Energy and Force from Hamiltonian" here or ensure
%      it appears before method section - this is central to the paper's thesis
% [S2] Consider merging symmetry discussion into method section where it's used
% [S3] Fix placeholder references (Appendix XXX)
%
% STORYLINE NOTES:
% This section establishes the mathematical foundation but doesn't yet
% connect to the paper's key question (can Hamiltonian prediction yield
% good energies/forces?). The energy/force evaluation procedure is
% described later in Section 4 (method), but arguably belongs in
% preliminaries since it's fundamental to the evaluation paradigm.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Preliminaries}
\label{sec:prelim}

Density functional theory (DFT) provides a practical framework for computing
electronic structure, by reformulating the many-electron Schr\"odinger equation
in terms of the electron density~\cite{hohenberg1964inhomogeneous,kohn1965self}.
In addition, Kohn-Sham DFT (KS-DFT) simplifies the many-electron interaction system with an
auxiliary system of non-interacting single-particle orbitals
$\{\psi_i\}_{i=1}^{N}$, where $\psi_i : \mathbb{R}^3 \rightarrow \mathbb{C}$, which successfully reproduces the original ground-state electron density
$\rho(\mathbf r): \mathbb{R}^3 \rightarrow \mathbb{R}_{>0}$.
Given that the ground-state energy of the system can be expressed as a functional of the ground-state electron density, one can calculate the ground-state energy without including costly many-electron interaction.

Such orbitals and the corresponding electron density used by KS-DFT are obtained by solving the Kohn-Sham equations:
\begin{equation}
    \hat H_{\mathrm{KS}}[\rho]\psi_i(\mathbf r) = \epsilon_i \psi_i(\mathbf r),
    \qquad
    \rho(\mathbf r) = \sum_{i=1}^{N} |\psi_i(\mathbf r)|^2,
    \label{eq:KS}
\end{equation}
where $\epsilon_i$ denotes the orbital energies. The KS Hamiltonian operator $\hat H_{\mathrm{KS}}[\rho]$ depends explicitly on the electron density $\rho$, which is itself constructed from the orbitals.

\textbf{Matrix formulation.} In practice, the KS equations are solved numerically by expanding the orbitals in a finite set of basis functions $\{\phi_b(\mathbf r)\}_{b=1}^{B}$, and each single particle orbital is expressed as $\psi_i(\mathbf r) = \sum_{b=1}^{B} C_{bi}\phi_b(\mathbf r)$. Substituting this expansion into the Kohn-Sham equations yields the Roothaan-Hall equation~\citep{roothaan_1951,hall_1951}:
\begin{equation}
    \mathbf H\mathbf C = \mathbf S \mathbf C \boldsymbol{\epsilon},
    \label{eq:RH}
\end{equation}
where $\mathbf C \in \mathbb{R}^{B \times N}$ is the molecular orbital coefficient matrix 
and $\mathbf S \in \mathbb{R}^{B \times B}$ is the overlap matrix with elements:
\begin{equation}
    S_{ij} = \int \phi_i^\dagger(\mathbf r)\phi_j(\mathbf r)\, \mathrm d\mathbf r,
\end{equation}
and $\boldsymbol{\epsilon}\in\mathbb{R}^{N\times N}$ is the diagonal matrix of orbital energies.
The Hamiltonian matrix $\mathbf H = \mathcal H(\mathbf C) \in \mathbb{R}^{B \times B}$ is obtained by mapping the orbital coefficients $\mathbf C$ to a density-dependent Hamiltonian, making the eigenvalue problem nonlinear. We provide the details about the KS-DFT in \cref{app:background}.

\paragraph{Energy and force evaluation in KS-DFT.}
In KS-DFT, physical observables are computed from the electron density
$\rho(\mathbf r)$ induced by the Kohn-Sham orbitals.
The total energy is defined by the Kohn-Sham energy functional:
\begin{equation}
E_{\mathrm{KS}}[\rho]
=
T_s[\rho]
+
\int v_{\mathrm{ext}}(\mathbf r)\rho(\mathbf r)\,d\mathbf r
+
E_{\mathrm{H}}[\rho]
+
E_{\mathrm{xc}}[\rho]
+
E_{\mathrm{nn}},
\end{equation}
where $T_s$ is the non-interacting kinetic energy, $v_{\mathrm{ext}}$ is the
external (electron–nuclear) potential, $E_{\mathrm{H}}$ is the Hartree energy,
$E_{\mathrm{xc}}$ is the exchange–correlation energy, and $E_{\mathrm{nn}}$ is
the nuclear repulsion energy.
Atomic force $\mathbf F_i$ on $i$-th atom is defined as the derivative of the total energy with respect to
nuclear coordinates $\mathbf r_i$ as follows:
\begin{equation}
\mathbf F_i = -\nabla_{\mathbf r_i} E_{\mathrm{KS}}[\rho].
\end{equation}
We defer the concrete evaluation procedure used in this work from a Hamiltonian
matrix to \cref{app:ef_eval}.
%and \cref{app:ef_eval}.




% \subsection{Symmetry and equivariant structure}
% \label{sec:prelim_symmetry}

% \paragraph{Equivariance.}
% Let $R\in\mathrm{SO}(3)$ be a 3D rotation. A mapping $\Phi$ is
% \emph{SO(3)-equivariant} if rotating the input results in a predictable rotation
% of the output:
% \begin{equation}
% \Phi(R\,\mathbf x) = \mathbf D_{\mathrm{out}}(R)\,\Phi(\mathbf x),
% \end{equation}
% where $\mathbf D_{\mathrm{out}}(R)$ specifies how the output transforms under
% rotations. In practice, designing an equivariant model ensures that every intermediate feature follows the same rule.

% \paragraph{Irreducible representations (irreps).}
% Irreducible representations (irreps) provide a canonical way to specify and
% organize rotation transformation rules. An irrep of degree $\ell$ is a
% $(2\ell+1)$-dimensional feature that transforms as
% \begin{equation}
% \mathbf f[\ell]\mapsto \mathbf D^{(\ell)}(R)\,\mathbf f[\ell],
% \qquad
% \mathbf f[\ell]\in\mathbb R^{2\ell+1},
% \end{equation}
% where $\mathbf D^{(\ell)}(R)$ is the degree-$\ell$ rotation matrix.
% By representing features as a direct sum of irreps,
% \begin{equation}
% \mathbf f=\bigoplus_{\ell=0}^{\ell_{\max}} \mathbf f[\ell],
% \end{equation}
% we make their rotation behavior explicit: $\ell=0$ components are invariant
% (scalars), while $\ell>0$ components rotate (e.g., vectors for $\ell=1$). Our model stores intermediate features in this irrep form and uses SO(3)-equivariant
% layers to preserve these transformation rules throughout. Details are provided
% in Appendix~XX.


% REVIEW [MINOR] STYLE: Long sentence (38 words). Consider splitting after "frame".
% SUGGESTION [A]: The Hamiltonian operator is rotation-invariant, but its \emph{matrix} representation depends on the coordinate frame because the underlying atomic orbital basis rotates. Let $\mathbf H$ denote the Hamiltonian matrix in an atom-centered orbital basis, and let $\mathbf D(R)$ be the representation of the rotation acting on that basis.
% SUGGESTION [B]: The Hamiltonian operator is rotation-invariant, but its matrix representation depends on the coordinate frame. This is because the underlying atomic orbital basis rotates with the molecule.
% ---
%\paragraph{Rotational equivariance of the Hamiltonian.}
%The Hamiltonian operator is rotation-invariant, but its \emph{matrix} representation depends on the coordinate frame because the underlying atomic orbital basis rotates. Let $\mathbf H$ denote the Hamiltonian matrix in an atom-centered orbital basis, and let $\mathbf D(R)$ be the representation of a global rotation $R$ acting on that basis. Under $R$, the Hamiltonian matrix transforms equivariantly as \begin{equation} \mathbf H' = \mathbf D(R)\,\mathbf H\,\mathbf D(R)^{-1}, \label{eq:H_equiv} \end{equation} where $\mathbf D(R)=\bigoplus_{\ell}\mathbf D^{(\ell)}(R)$ is block-diagonal with respect to orbital angular momentum $\ell$. Here $\mathbf D^{(\ell)}(R)$ denotes the $(2\ell+1)$-dimensional irreducible representation (irrep) of SO(3) (i.e., the Wigner-$D$ matrix at degree $\ell$). This similarity transform preserves the spectrum of $\mathbf H$ and motivates organizing model features using the same $\ell$-wise irrep decomposition.  Additional background on group theory and equivariance is provided in \cref{app:background}.


% \seongsu{
% \paragraph{Hamiltonian symmetry and equivariance.}
% The Kohn-Sham Hamiltonian obeys rotational symmetry.
% Let $R \in \mathrm{SO(3)}$ be a global rotation acting on a molecular structure
% $\mathcal M$.
% Under this transformation, the Hamiltonian expressed in an atomic orbital basis
% transforms as
% \begin{equation}
% \mathbf H(R\mathcal M)
% =
% \mathbf D_R\,\mathbf H(\mathcal M)\,\mathbf D_R^{-1},
% \end{equation}
% where $\mathbf D_R=\bigoplus_{\ell} D^{(\ell)}(R)$ is the block-diagonal
% representation induced by orbital angular momentum $\ell$.
% Accordingly, we construct the predictor $f_\theta$ to satisfy the equivariance
% condition
% \begin{equation}
% f_\theta\!\left(
% R\mathcal M,\, t,\,
% \mathbf D_R\,\mathbf H_t\,\mathbf D_R^{-1}
% \right)
% =
% \mathbf D_R\,
% f_\theta\!\left(
% \mathcal M,\, t,\, \mathbf H_t
% \right)
% \mathbf D_R^{-1}.
% \end{equation}
% Background on irreducible representations and tensor products is provided in
% Appendix~XX.
% }

% \paragraph{Hamiltonian symmetry and equivariance.}
% The Kohn--Sham Hamiltonian obeys rotational symmetry: under a global rotation
% $R \in \mathrm{SO(3)}$, its representation must transform consistently.
% We formalize this using SO(3)-equivariant mappings.

% A function $f$ is SO(3)-equivariant if
% \begin{equation}
%     f(R \cdot x) = R \cdot f(x), \qquad \forall R \in \mathrm{SO(3)} .
% \end{equation}
% In practice, equivariant representations are constructed from irreducible
% representations (irreps) of SO(3), indexed by angular momentum $\ell$.
% Under rotation, features of degree $\ell$ transform according to the Wigner
% matrix $D^{(\ell)}(R)$.

% In Kohn--Sham DFT, atomic orbitals are labeled by angular momentum.
% Grouping orbital coefficients by angular momentum channels, their transformation
% under rotation can be written as
% \begin{equation}
%     \mathbf C \;\mapsto\; \mathbf D(R)\,\mathbf C,
%     \qquad
%     \mathbf D(R) = \bigoplus_{\ell} D^{(\ell)}(R).
% \end{equation}
% Consequently, the Hamiltonian matrix $\mathbf H$ must satisfy
% \begin{equation}
%     \mathbf H \;\mapsto\; \mathbf D(R)\,\mathbf H\,\mathbf D(R)^{-1},
% \end{equation}
% ensuring rotational equivariance.

% Details on SO(3) representations and tensor product constructions are provided
% in Appendix~XX.




% \textbf{Kohn-Sham Density Functional Theory.} The fundamental challenge in quantum chemistry is solving the many-body Schrödinger equation for an $N$-electron system. Since the exact solution is computationally intractable due to the exponential scaling with $N$, Kohn-Sham Density Functional Theory (KS-DFT)~\cite{hohenberg1964inhomogeneous, kohn1965self} offers a tractable alternative. KS-DFT posits that the ground-state energy is a functional of the electron density $\rho(\mathbf{r})$ and introduces a fictitious system of non-interacting orbitals $\{\psi_{i}\}_{i=1}^{N}$ that yield the same density as the interacting system. These orbitals are solutions to the Kohn-Sham equations:
% \begin{equation}
% \hat{H}_{\text{KS}}[\rho]\psi_{i}(\mathbf{r}) = \epsilon_{i}\psi_{i}(\mathbf{r}), \qquad \rho(\mathbf{r}) = \sum_{i=1}^{N}|\psi_{i}(\mathbf{r})|^{2},\label{eq:KS}
% \end{equation}
% where $\epsilon_{i}$ are the orbital energies. Crucially, the Hamiltonian operator $\hat{H}_{\text{KS}}[\rho]$ depends on the electron density $\rho$, which is itself constructed from the orbitals.
% % This creates a circular dependency, implying that the Hamiltonian depends on its own eigenvectors

% \textbf{Roothaan-Hall Equation.} To solve \cref{eq:KS} numerically, the orbitals are expanded using a finite set of basis functions $\{\phi_{b}(\mathbf{r})\}_{b=1}^{B}$ (e.g., Gaussian-type orbitals), such that $\psi_{i}(\mathbf{r}) = \sum_{b=1}^{B} C_{bi}\phi_{b}(\mathbf{r})$. This discretization converts the continuous differential equations into a matrix eigenvalue problem known as the Roothaan-Hall equations~\cite{roothaan_1951, hall_1951}:\begin{equation}\mathbf{H}(\mathbf{C})\mathbf{C} = \mathbf{S}\mathbf{C}\boldsymbol{\epsilon}.\label{eq:RH}\end{equation}Here, $\mathbf{C} \in \mathbb{R}^{B \times N}$ is the orbital coefficient matrix, and $\mathbf{S} \in \mathbb{R}^{B \times B}$ is the overlap matrix with entries $S_{ij} = \int \phi_i^*(\mathbf{r})\phi_j(\mathbf{r}) d\mathbf{r}$. The Hamiltonian matrix $\mathbf{H}(\mathbf{C}) \in \mathbb{R}^{B \times B}$ is constructed from the density matrix (derived from $\mathbf{C}$), explicitly highlighting the non-linear dependence of the Hamiltonian on the coefficients $\mathbf{C}$.

% \textbf{Self-Consistent Field (SCF) and SCF-Free.} Because $\mathbf{H}$ depends on $\mathbf{C}$, \cref{eq:RH} cannot be solved via a single diagonalization. Instead, it requires the Self-Consistent Field (SCF) procedure: an iterative algorithm that starts with an initial guess for $\mathbf{C}$, constructs $\mathbf{H}(\mathbf{C})$, diagonalizes it to update coefficients, and repeats this cycle until the input and output densities converge. This iterative loop constitutes the primary computational cost in DFT, typically scaling as $\mathcal{O}(N^3)$ or $\mathcal{O}(N^4)$ with respect to the system size.

% In this context, \textit{SCF-free} prediction offers a direct alternative to the iterative procedure. The objective is to predict the converged Hamiltonian $\mathbf{H}^*$ directly from the molecular geometry, effectively bypassing the repeated construction and diagonalization steps of the SCF loop. This approach eliminates the computational overhead of the iterative solver, provided that the predicted Hamiltonian possesses sufficient fidelity to derive accurate physical observables without requiring subsequent SCF cycles for refinement.

% \sungs{Sungsoo: Add preliminaries for computing energy and force field from the approximate Hamiltonian.}

% \subsection{Equivariant Graph Neural Networks}
% Molecular systems are naturally represented as geometric graphs $\mathcal{G}=(\mathcal{V}, \mathcal{E})$, where nodes $i \in \mathcal{V}$ correspond to atoms with positions $\mathbf{r}_i \in \mathbb{R}^3$ and features $\mathbf{h}_i$. A critical requirement for modeling such physical systems is equivariance under Euclidean symmetries. Formally, a function $\Phi$ is equivariant to a symmetry group $G$ (e.g., $\mathrm{SO}(3)$) if it commutes with the group action: $\Phi(D_{\text{in}}(g)\mathbf{x}) = D_{\text{out}}(g)\Phi(\mathbf{x})$ for any $g \in G$, where $D(g)$ denotes the group representation.

% \textbf{SO(3) Equivariance via Tensor Products.} To capture full 3D rotational symmetry, $\mathrm{SO}(3)$-equivariant networks organize node features into irreducible representations (irreps) of degree $l$, where type-$l$ features correspond to vectors of dimension $2l+1$. Interactions between these features rely on the tensor product, which combines irreps using Clebsch-Gordan coefficients to produce new equivariant features. While this approach provides a rigorous geometric description, the computation of high-order tensor products is computationally intensive, scaling steeply with both the maximum degree $l$ and the number of feature channels.

% \textbf{Efficient SO(2) Convolution.} Alternatively, operations can be formulated under $\mathrm{SO}(2)$ symmetry, which describes rotations within a 2D plane. In this regime, the representations simplify significantly, behaving as complex phasors (analogous to Fourier coefficients) rather than dense tensors. Consequently, the interaction between features reduces from a complex tensor product to efficient complex-valued multiplications or standard linear operations. This simplification allows $\mathrm{SO}(2)$-based layers to function as efficient "convolutions," enabling the construction of deeper and wider networks with substantially lower computational overhead compared to their fully $\mathrm{SO}(3)$-equivariant counterparts.

==> 4_method.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% PAPER ANALYSIS - METHOD (QHFLOW2)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% STRENGTHS:
% + Clear problem setup and notation
% + Well-structured with logical paragraph organization
% + Two-stage pair update is clearly motivated and explained
% + Energy/force evaluation procedure is complete and clear
% + Good use of equations with consistent notation
%
% WEAKNESSES:
% - Very long section (450+ lines including comments) - could be more concise
% - Lots of commented-out alternative formulations create clutter
% - Appendix references are placeholders (XX, XXX)
% - The "key insight" (two-stage edge update) could be highlighted earlier
% - Missing: explicit comparison of what's new vs QHFlow v1
%
% STRUCTURAL SUGGESTIONS:
% [S1] Add a brief "Key differences from QHFlow" paragraph at the start
% [S2] Consider moving Energy/Force evaluation to Preliminaries (Section 3)
%      since it's part of the evaluation paradigm, not the method contribution
% [S3] Clean up commented-out code blocks before submission
% [S4] Make the two-stage pair update contribution more prominent
%
% STORYLINE NOTES:
% This section delivers on the technical contribution well. The flow is:
% problem setup -> flow matching -> embeddings -> backbone -> two-stage
% update -> Hamiltonian construction -> energy/force evaluation. The
% energy/force evaluation is somewhat misplaced here (belongs with
% evaluation framework), but including it ensures readers understand
% the full pipeline.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\section{QHFlow2}

We propose \textbf{QHFlow2}, a highly accurate Hamiltonian predictor based on an equivariant framework.
QHFlow2 improves the prior work~\citep[QHFlow;][]{kim2025high} with enhanced scalability through SO(2)-equivariant convolutions~\cite{passaro2023reducing,fu2025learning} and a two-stage update of pairwise representations.
These design choices strengthen Hamiltonian prediction and enable stable downstream energy and force evaluation with fewer parameters.

\subsection{Problem setup and downstream evaluation}

\paragraph{Problem setup.}
Given a molecular structure $\mathcal M = \{(Z_i,\mathbf r_i)\}_{i=1}^N$, our goal is to predict the reference Hamiltonian $\mathbf H^\star\in\mathbb{R}^{B\times B}$, where $B$ is the total number of basis functions.
We adopt a flow-based formulation in which the model is conditioned on an intermediate Hamiltonian state $\mathbf H_t$ at flow time $t\in[0,1)$.
Concretely, the model implements
\begin{equation}
    \hat{\mathbf H}^\star
    =
    f_\theta\!\left(\mathcal M,\, t,\, \mathbf H_t;\, \{\mathbf F_k\}\right),
\end{equation}
where $\{\mathbf F_k\}$ denotes optional conditioning matrices that are deterministically computed from $\mathcal M$ and share the same symmetry and block structure as $\mathbf H^\star$ (e.g., the overlap matrix or an initial Hamiltonian).

We model the Hamiltonian as a coupled object and learn the conditional
distribution of Hamiltonians using conditional flow matching~\cite{lipmanflow}.
Following prior work~\cite{kim2025high}, we adopt this formulation, which has proven effective for Hamiltonian prediction.
Given a flow time $t\in[0,1)$, we define a linear interpolation between an
initial noise sample $\mathbf H_0$ and the target Hamiltonian
$\mathbf H^\star$,
\begin{equation}
    \mathbf H_t = (1-t)\mathbf H_0 + t \mathbf H^\star .
\end{equation}
The model parameterizes a time-dependent vector field
\(
v_t^\theta(\mathbf H_t, \mathcal M)
=
(\mathbf{H}^\theta_1-\mathbf{H}_t)/(1-t)
\)
using a neural network that predicts a terminal Hamiltonian
$\mathbf{H}^\theta_1$.
Training minimizes the standard flow-matching objective
\begin{equation}
\mathcal L_{\mathrm{CFM}}
=
\mathbb E
\left[
\left\|
v_t^\theta(\mathbf H_t,\mathcal M)
-
\frac{\mathbf H^\star - \mathbf H_0}{1-t}
\right\|^2
\right].
\end{equation}
The noise $\mathbf H_0$ is sampled from a
distribution that preserves the same equivariance and block structure as
$\mathbf H^\star$.

\textbf{Energy and force evaluation from Hamiltonian.}
\label{sec:ef_eval}
We evaluate energies and forces from the predicted Hamiltonian
$\hat{\mathbf H}$ by solving a single generalized
eigenvalue problem and computing the KS energy and forces in
PySCF~\cite{sun2018pyscf}.
Given the overlap matrix $\mathbf S\in\mathbb{R}^{B\times B}$, we first solve the generalized eigenvalue problem
\begin{equation}
\hat{\mathbf H}\hat{\mathbf C}
=
\mathbf S\,\hat{\mathbf C}\,\hat{\boldsymbol\epsilon},
\end{equation}
where $\hat{\mathbf C}\in\mathbb{R}^{B\times B}$ and $\hat{\boldsymbol\epsilon}\in\mathbb{R}^{B}$ are the molecular-orbital coefficients and orbital energies.

We then determine orbital occupations by eigenvalue ordering.
To enforce a restricted (closed-shell) occupation pattern with $N_e$ electrons, we set
$n_{\mathrm{occ}}=\lceil N_e/2\rceil$ and define
\begin{equation}
\hat{o}_p =
\begin{cases}
2, & p \le n_{\mathrm{occ}},\\
0, & p > n_{\mathrm{occ}}.
\end{cases}
\end{equation}
This yields the density matrix
\begin{equation}
\hat{\mathbf D}
=
\hat{\mathbf C}\,\mathrm{diag}(\hat{\mathbf o})\,\hat{\mathbf C}^{\top}
\in\mathbb R^{B\times B}.
\end{equation}

Finally, following the KS energy and force definitions in \cref{sec:prelim}, we provide $\hat{\mathbf D}$ to PySCF while holding the DFT configuration fixed (basis, functional, and numerical grids).
PySCF evaluates $E_{\mathrm{KS}}$ and analytic nuclear gradients, yielding atomic forces $\mathbf F_I\in\mathbb R^3$.


% We evaluate energies and forces from the predicted Hamiltonian
% $\hat{\mathbf H}\in\mathbb R^{B\times B}$ by solving a single generalized
% eigenvalue problem and computing the resulting KS energy and forces in
% PySCF~\cite{sun2018pyscf}. Given the overlap matrix
% $\mathbf S\in\mathbb R^{B\times B}$, we solve the generalized eigenvalue problem
% \begin{equation}
% \hat{\mathbf H}\hat{\mathbf C}
% =
% \mathbf S\,\hat{\mathbf C}\,\hat{\boldsymbol\epsilon},
% \end{equation}
% where $\hat{\mathbf C}\in\mathbb R^{B\times B}$ and
% $\hat{\boldsymbol\epsilon}\in\mathbb R^{B}$ denote molecular-orbital
% coefficients and orbital energies, respectively.

% We assign orbital occupations by eigenvalue ordering. For closed-shell systems
% with $N_e$ electrons, we set $n_{\mathrm{occ}}=N_e/2$ and define
% \begin{equation}
% \hat{o}_p =
% \begin{cases}
% 2, & p \le n_{\mathrm{occ}},\\
% 0, & p > n_{\mathrm{occ}}.
% \end{cases}
% \end{equation}
% The resulting density matrix is
% \begin{equation}
% \hat{\mathbf D}
% =
% \hat{\mathbf C}\,\mathrm{diag}(\hat{\mathbf o})\,\hat{\mathbf C}^{\top}
% \in\mathbb R^{B\times B}.
% \end{equation}
% Following the KS energy and force definitions in \cref{sec:prelim}, we
% evaluate $E_{\mathrm{KS}}$ and $\mathbf F_I$ by providing the density matrix
% $\hat{\mathbf D}$ to PySCF under a fixed DFT setup (basis, functional, and
% numerical grids). PySCF computes the density-dependent energy terms and the
% corresponding analytic nuclear gradients, yielding atomic forces
% $\mathbf F_I\in\mathbb R^3$.


\subsection{Model architecture}


\paragraph{Embeddings.}
We initialize atom-wise node features from the molecular structure
$\mathcal{M}$, the flow time $t$, and the intermediate Hamiltonian state
$\mathbf H_t$.
The atomic number $Z_i$ is embedded in an SO(3)-invariant feature
$\mathbf a_i = g_{\mathrm{atom}}(Z_i)$, and the $t$ is embedded by a
sinusoidal encoding
$\boldsymbol{\tau}_t = g_{\mathrm{time}}(t)$.

The intermediate Hamiltonian $\mathbf H_t$ is embedded into an SO(3)-equivariant
irreps feature using a matrix encoder,
\begin{equation}
\mathbf f_H = g_{\mathrm{matrix}}^{(H)}(\mathbf H_t)
=
\{\mathbf f_H[\ell]\}_{\ell=0}^{\ell_{\max}},
\end{equation}
where $\mathbf f_H[\ell]\in\mathbb R^{2\ell+1}$ denotes the irreps component of
degree $\ell$.
Additional conditioning matrices $\{\mathbf F_k\}$, when used, are embedded in
the same manner,
$\mathbf f_k = g_{\mathrm{matrix}}^{(k)}(\mathbf F_k)
= \{\mathbf f_k[\ell]\}_{\ell=0}^{\ell_{\max}}$.

The initial node feature is then constructed by combining only the invariant
($\ell=0$) components,
\begin{equation}
\begin{aligned}
\mathbf z_i[0] &=
g_{\mathrm{mix}}\!\left(
\mathbf a_i,\,
\boldsymbol{\tau}_t,\,
\mathbf f_H[0],\,
\{\mathbf f_k[0]\}
\right), \\
\mathbf z_i[\ell] &=
\mathbf f_H[\ell] +
\sum_{k} \mathbf f_k[\ell],
\qquad \ell > 0 .
\end{aligned}
\end{equation}
Here, $g_{\mathrm{mix}}$ produces atom-dependent scalar features, while all
non-scalar irreps components $(\ell>0)$ are initialized directly from the sum of
the matrix embeddings.


\paragraph{SO(2)-equivariant message passing backbone.}
We adopt the SO(2)-equivariant edgewise--nodewise update flow of eSEN~\cite{fu2025learning}.
We use the node features from the input embeddings as the backbone input,
setting $\mathbf x_i^{(0)} \leftarrow \mathbf z_i$.
The backbone then applies $L$ layers of SO(2)-equivariant edgewise convolutions
without storing persistent edge features.

At each layer $l$, an SO(2)-equivariant edgewise message is constructed on-the-fly
for each ordered atom pair $(i,j)$ using relative geometry.
The interatomic displacement vector $\mathbf r_{ij}=\mathbf r_j-\mathbf r_i$
defines a local coordinate frame, and radial information is encoded via a
distance embedding $\phi_{\mathrm{rbf}}(r_{ij})$ with a finite cutoff $r_c$.
We define the neighborhood as $\mathcal N(i) = \{\, j \neq i \mid r_{ij} < r_c \,\}$, and set $\phi_{\mathrm{rbf}}(r_{ij})=\mathbf 0$ for $r_{ij}\ge r_c$.
Concretely, $\phi_{\mathrm{rbf}}$ expands the scalar distance into a fixed-length
radial feature using a set of basis functions,
\begin{equation}
\phi_{\mathrm{rbf}}(r_{ij}) =
\Big[\, b_1(r_{ij}),\,\ldots,\, b_M(r_{ij}) \,\Big],
\end{equation}
where $\{b_m\}_{m=1}^M$ are smooth radial basis functions (e.g., Gaussian or
Bessel bases) multiplied by a smooth cutoff envelope.

An edgewise message is then computed as
\begin{equation}
\mathbf m_{ij}^{(l)} =
\mathrm{SO2Conv}_{\mathrm{pair}}^{(l)}\!\left(
[\mathbf x_i^{(l)} \Vert \mathbf x_j^{(l)}],\,
\phi_{\mathrm{rbf}}(r_{ij})
\right),
\end{equation}
where $[\cdot\Vert\cdot]$ denotes concatenation.
This operation corresponds to the SO(2)-equivariant edgewise convolution used in
eSEN~\cite{fu2025learning} and preserves the SO(3) irreps structure of the node
features.

The edgewise messages are aggregated over neighbors and used to update node
features via a nodewise equivariant feed-forward block,
\begin{equation}
\mathbf x_i^{(l+1)} =
\mathbf x_i^{(l)} +
\mathrm{SO2Conv}_{\mathrm{self}}^{(l)}\!\left(
\mathbf x_i^{(l)},\,
\sum_{j\in\mathcal N(i)} \mathbf m_{ij}^{(l)}
\right).
\end{equation}
Here, $\mathrm{SO2Conv}_{\mathrm{self}}^{(l)}$ denotes the nodewise feed-forward
network of eSEN, which operates independently on each irreps component and
preserves SO(3) equivariance.
Stacking $L$ such layers yields the final node features $\{\mathbf x_i^{(L)}\}$.

\paragraph{Two-stage pair update.}
For Hamiltonian prediction, we require an explicit representation for each atom
pair $(i,j)$ used in Hamiltonian assembly, since off-diagonal Hamiltonian blocks
depend on atom--atom interactions.
We therefore construct \emph{pairwise features} $\mathbf e_{ij}$ after the
backbone from the final node features $\{\mathbf x_i^{(L)}\}$.
Unlike the edgewise messages computed within each message-passing layer,
$\mathbf e_{ij}$ are carried forward to subsequent pairwise processing and are
used directly for Hamiltonian construction.

First, we initialize an intermediate pairwise feature using an SO(2)-equivariant
pair encoder driven by a radial distance embedding,
\begin{equation}
\tilde{\mathbf e}_{ij} =
\mathrm{SO2Conv}_{\mathrm{pair}}\!\left(
[\mathbf x_i^{(L)} \Vert \mathbf x_j^{(L)}],\,
\phi_{\mathrm{rbf}}(r_{ij})
\right),
\end{equation}
where $\phi_{\mathrm{rbf}}(r_{ij})$ denotes the radial basis embedding.

In practice, we find that the diagonal-block accuracy can be overly sensitive to
the choice of the radial basis hyperparameters in this initialization.
To mitigate this dependence, we apply a second refinement stage that injects
pairwise interactions through an alternative SO(3)-equivariant coupling
mechanism, rather than relying solely on the same radial encoding.
Concretely, we update the pairwise feature as
\begin{equation}
\mathbf e_{ij} =
\tilde{\mathbf e}_{ij} +
g_{\mathrm{ref}}\!\left(
\tilde{\mathbf e}_{ij},\,
\mathbf x_i^{(L)},\,
\mathbf x_j^{(L)},\,
r_{ij}
\right),
\end{equation}
where $g_{\mathrm{ref}}$ is an SO(3)-equivariant tensor-product-based layer that refines $\tilde{\mathbf e}_{ij}$ using the node
irreps and pair geometry. Detail implementations in \cref{app:model_implementation}.

\paragraph{Equivariant vector-to-matrix Hamiltonian construction.}
The backbone produces final node features $\{\mathbf x_i^{(L)}\}$ and explicit
pairwise features $\{\mathbf e_{ij}\}$, which we convert into the predicted
Hamiltonian $\hat{\mathbf H}$ in an atom-centered orbital basis.
Let $B_i$ denote the number of basis functions (orbitals) associated with atom
$i$; in our setting $B_i$ is determined by the atomic species $Z_i$.
We construct $\hat{\mathbf H}$ as a block matrix
$\hat{\mathbf H}=[\hat{\mathbf H}_{ij}]_{i,j=1}^N$ with $\hat{\mathbf H}_{ij}\in\mathbb R^{B_i\times B_j}$.


For each atom pair $(i,j)$, we first select an equivariant feature to represent
their interaction,
\begin{equation*}
\mathbf q_{ij} \;=\;
\begin{cases}
\mathbf x_i^{(L)}, & i=j,\\
\mathbf e_{ij}, & i\neq j,
\end{cases}
\end{equation*}
and map it to the orbital-pair block via a tensor expansion module adapted from
QHNet~\cite{yu2023efficient},
\begin{equation}
\hat{\mathbf H}_{ij} = \mathcal E_{Z_i,Z_j}\!\left(\mathbf q_{ij}\right),
\quad
\mathcal E_{Z_i,Z_j}:\{\mathbf q[\ell]\}_{\ell=0}^{\ell_{\max}}
\rightarrow \mathbb R^{B_i\times B_j}.
\end{equation}
The expansion $\mathcal E_{Z_i,Z_j}$ is an SO(3)-equivariant linear readout that
converts irreps components into the matrix block of the corresponding
atom-type pair; details are provided in \cref{app:model_implementation}.

Finally, we enforce Hermiticity by symmetrization,
\begin{equation}
\hat{\mathbf H} \leftarrow \tfrac12(\hat{\mathbf H}+\hat{\mathbf H}^{\top}).
\end{equation}



% \paragraph{Input embeddings.}
% We initialize node- and pair-level features from atomic identity, geometry, flow
% time, and optional auxiliary matrices.
% Atomic numbers are mapped to rotation-invariant features
% $\mathbf a_i=g_{\mathrm{atom}}(Z_i)$, and the flow time is embedded as
% $\boldsymbol{\tau}_t=g_{\mathrm{time}}(t)$.
% When available, each auxiliary matrix $\mathbf F_k$ is embedded into
% SO(3)-equivariant features
% $\mathbf f_k=g_{\mathrm{matrix}}^{(k)}(\mathbf F_k)$, represented as collections
% of irreducible components up to angular momentum $\ell_{\max}$.

% Initial node features are constructed by combining invariant components,
% \begin{equation}
% \mathbf x_i^{(0)} =
% g_{\mathrm{mix}}\!\left(
% \mathbf a_i,\,
% \boldsymbol{\tau}_t,\,
% \{\mathbf f_k^{(0)}\}_{k=1}^K
% \right),
% \end{equation}
% while higher-order SO(3) components are initialized directly from the
% equivariant matrix embeddings (see Appendix~XX).
% Pair features are initialized from relative geometry using a radial distance
% embedding with a finite cutoff,
% \begin{equation}
% \mathbf e_{ij}^{(0)}=\phi_{\mathrm{rbf}}(r_{ij}), \qquad
% r_{ij}=\|\mathbf r_i-\mathbf r_j\|.
% \end{equation}

% \paragraph{SO(2)-equivariant message passing backbone.}
% Each atom $i$ is associated with a node feature $\mathbf x_i$, and each atom pair
% $(i,j)$ with a pair feature $\mathbf e_{ij}$.
% These features take values in spaces carrying SO(3) irreducible representations,
% so that their transformation behavior under rotation is well defined.

% Feature updates are implemented using SO(2)-equivariant convolutions in local
% coordinate frames, which provide an efficient parameterization for propagating
% and mixing SO(3)-equivariant features.
% Starting from $\{\mathbf x_i^{(0)}\}$ and $\{\mathbf e_{ij}^{(0)}\}$, we apply $L$
% layers of message passing.
% At layer $l$, pair features are updated as
% \begin{equation}
% \mathbf e_{ij}^{(l+1)} =
% \Phi_e^{(l)}\!\left(
% \mathbf e_{ij}^{(l)}, \mathbf x_i^{(l)}, \mathbf x_j^{(l)}, \phi_{\mathrm{rbf}}(r_{ij})
% \right),
% \end{equation}
% where $\phi_{\mathrm{rbf}}$ denotes a fixed radial basis embedding of the
% interatomic distance $r_{ij}$, and $\Phi_e^{(l)}$ is a learnable SO(2)-equivariant
% operator that updates pair features while preserving their SO(3) representation
% structure.

% Node features are then updated by aggregating incoming pair features,
% \begin{equation}
% \mathbf x_i^{(l+1)} =
% \Phi_x^{(l)}\!\left(
% \mathbf x_i^{(l)}, \sum_{j\in\mathcal N(i)} \mathbf e_{ij}^{(l+1)}
% \right),
% \end{equation}
% where $\Phi_x^{(l)}$ is a learnable type-preserving update operator acting on node
% features, implemented using the same SO(2)-equivariant parameterization.

% \paragraph{Input embeddings.}
% We initialize atom-wise node features from the molecular structure $\mathcal{M}$, the flow time $t$, and the intermediate Hamiltonian state $\mathbf H_t$.
% The atomic number $Z_i$ is embedded in a SO(3)-invariant feature $\mathbf a_i = g_{\mathrm{atom}}(Z_i)$, and $t$ is embedded using a sinusoidal encoding $\boldsymbol{\tau}_t = g_{\mathrm{time}}(t)$.

% The intermediate Hamiltonian $\mathbf H_t$ is embedded into SO(3)-equivariant irreps features using a matrix encoder $g_{\mathrm{matrix}}$,
% Additional conditioning matrices $\{\mathbf F_k\}$, when used, are embedded in the same manner.

% The initial node feature is constructed by mixing the invariant components,
% \begin{equation}
% \mathbf x_i^{(0)} =
% g_{\mathrm{mix}}\!\left(
% \mathbf a_i,\,
% \boldsymbol{\tau}_t,\,
% \mathbf f_i^{(H,\,\ell=0)},\,
% \{\mathbf f_i^{(k,\,\ell=0)}\}_{k=1}^K
% \right),
% \end{equation}
% while higher-order irreps components $(\ell>0)$ are initialized directly from
% the corresponding matrix embeddings (Appendix~XX).

% Geometric information enters only through relative distances
% $r_{ij}=\|\mathbf r_i-\mathbf r_j\|$ via a radial basis embedding
% $\phi_{\mathrm{rbf}}(r_{ij})$, which is used in the edgewise message passing of
% the backbone.

% \paragraph{Input embeddings.}
% We initialize atom-wise node features from the molecular structure $\mathcal{M}$, the flow time $t$, and the intermediate Hamiltonian state $\mathbf H_t$.
% The atomic number $Z_i$ is embedded in a SO(3)-invariant feature $\mathbf a_i = g_{\mathrm{atom}}(Z_i)$, and $t$ is embedded using a sinusoidal encoding $\boldsymbol{\tau}_t = g_{\mathrm{time}}(t)$.

% The intermediate Hamiltonian $\mathbf H_t$ is embedded into
% SO(3)-equivariant irreps feature using a matrix encoder,
% \begin{equation}
% \mathbf f_H = g_{\mathrm{matrix}}^{(H)}(\mathbf H_t)
% =
% \bigoplus_{\ell=0}^{\ell_{\max}} \mathbf f_H^{(\ell)} .
% \end{equation}
% Additional conditioning matrices $\{\mathbf F_k\}$, when used, are embedded in the same manner 
% $\mathbf f_k = g_{\mathrm{matrix}}^{(k)}(\mathbf F_k)$.

% The initial node feature is then defined by combining only the invariant
% ($\ell=0$) components,
% \begin{equation}
% \begin{aligned}
% \mathbf z_i^{(0)} &=
% g_{\mathrm{mix}}\!\left(
% \mathbf a_i,\,
% \boldsymbol{\tau}_t,\,
% \mathbf f_H^{(0)},\,
% \{\mathbf f_k^{(0)}\}
% \right), \\
% \mathbf z_i^{(\ell)} &=
% \mathbf f_H^{(\ell)} +
% \sum \mathbf f_k^{(\ell)},
% \qquad \ell > 0 .
% \end{aligned}
% \end{equation}

% where $g_{\mathrm{mix}}$ produces atom-dependent scalar features, while all
% higher-order irreps components are initialized from the sum of the matrix
% embeddings.

% Relative geometry enters the model only through edge features, which are
% initialized from interatomic displacement vectors
% $\mathbf r_{ij}$ via a radial distance embedding and used in subsequent
% message passing.









% \paragraph{SO(2)-equivariant message passing backbone.}
% The backbone propagates information across the molecular graph using layered
% \emph{edgewise convolutions}~\cite{fu2025learning}.
% Each atom $i$ is associated with a node representation $\mathbf{x}_i^{(l)}$
% that transforms as a collection of SO(3) irreps.
% Edge representations are not stored explicitly. Instead, for each ordered atom pair $(i,j)$, edgewise messages are computed
% on-the-fly by combining the current node representations
% $\mathbf{x}_i^{(l)}$ and $\mathbf{x}_j^{(l)}$ with relative geometric information and are discarded after the message passing step.


% Each layer alternates between edgewise and nodewise updates.
% At layer $l$, for each ordered pair $(i,j)$, an edgewise message is computed via
% an SO(2) convolution in a local frame aligned with the interatomic
% displacement $\mathbf r_{ij}$,
% \begin{equation}
% \mathbf m_{ij}^{(l)} =
% \mathrm{SO2Conv}_{\text{pair}}^{(l)}\!\left(
% \mathbf x_i^{(l)},\, \mathbf x_j^{(l)},\, \phi_{\mathrm{rbf}}(r_{ij})
% \right),
% \end{equation}
% where $\phi_{\mathrm{rbf}}$ is a radial distance embedding with a finite cutoff.
% Messages are aggregated and used to update node representations,
% \begin{equation}
% \mathbf x_i^{(l+1)} =
% \mathbf x_i^{(l)} +
% \mathrm{FFN}^{(l)}\!\left(
% \mathbf x_i^{(l)},\, \sum_{j\in\mathcal N(i)} \mathbf m_{ij}^{(l)}
% \right).
% \end{equation}
% Stacking $L$ layers yields the final node representations
% $\{\mathbf x_i^{(L)}\}$.




% \textbf{Energy and force evaluation from Hamiltonian.}
% We evaluate energies and forces directly from the predicted Hamiltonian
% $\hat{\mathbf H}\in\mathbb R^{B\times B}$ using a one-shot KS-DFT evaluation in
% PySCF. Given the overlap matrix $\mathbf S\in\mathbb R^{B\times B}$, we solve the
% generalized eigenvalue problem
% \begin{equation}
% \hat{\mathbf H}\hat{\mathbf C}
% =
% \mathbf S\,\hat{\mathbf C}\,\hat{\boldsymbol\epsilon},
% \end{equation}
% where $\hat{\mathbf C}\in\mathbb R^{B\times B}$ collects molecular orbital
% coefficients and $\hat{\boldsymbol\epsilon}\in\mathbb R^{B}$ are the orbital
% energies.

% To construct the electron density, we assign an occupation vector
% $\hat{\mathbf o}\in\mathbb R^{B}$ by eigenvalue ordering. For closed-shell
% systems with $N_e$ electrons, we set $n_{\mathrm{occ}}=N_e/2$ and define
% \begin{equation}
% \hat{o}_p =
% \begin{cases}
% 2, & p \le n_{\mathrm{occ}},\\
% 0, & p > n_{\mathrm{occ}}.
% \end{cases}
% \end{equation}
% The density matrix is then
% \begin{equation}
% \hat{\mathbf D}
% =
% \hat{\mathbf C}\,\mathrm{diag}(\hat{\mathbf o})\,\hat{\mathbf C}^{\top}
% \in\mathbb R^{B\times B}.
% \end{equation}
% Using $\hat{\mathbf D}$, we evaluate the KS total energy
% \begin{equation}
% E_{\mathrm{KS}}
% =
% E_{\mathrm{nuc}}
% +
% \mathrm{Tr}\!\left[\hat{\mathbf D}\,\mathbf h_{\mathrm{core}}\right]
% +
% E_{\mathrm{coul}}[\hat{\mathbf D}]
% +
% E_{\mathrm{xc}}[\hat{\mathbf D}],
% \end{equation}
% where $E_{\mathrm{nuc}}$ is the nuclear repulsion energy,
% $\mathbf h_{\mathrm{core}}\in\mathbb R^{B\times B}$ is the one-electron core
% Hamiltonian, and $E_{\mathrm{coul}}$ and $E_{\mathrm{xc}}$ are the Hartree and
% exchange–correlation contributions computed from $\hat{\mathbf D}$
% (Appendix~XXX).

% Atomic forces are defined as the nuclear gradients of the total energy,
% \begin{equation}
% \mathbf F_I
% =
% -\frac{\partial E_{\mathrm{KS}}}{\partial \mathbf R_I}
% \in\mathbb R^{3}.
% \end{equation}
% In our implementation, all density-dependent terms in $E_{\mathrm{KS}}$ and the analytic evaluation of forces are computed using PySCF~\cite{sun2018pyscf} given $\hat{\mathbf D}$ (Appendix~XXX).







% \paragraph{Equivariant vector-to-matrix Hamiltonian construction.}
% Final node and pair features are expressed as SO(3)-equivariant vectors
% $\mathbf f=\bigoplus_{\ell}\mathbf f^{(\ell)}$.
% Hamiltonian matrix elements are constructed via Clebsch--Gordan tensor expansion,
% \begin{equation}
% \mathbf f^{(\ell_1)} \otimes \mathbf g^{(\ell_2)}
% =
% \bigoplus_{\ell=|\ell_1-\ell_2|}^{\ell_1+\ell_2}
% \sum_{m_1,m_2}
% C^{\ell m}_{\ell_1 m_1,\ell_2 m_2}
% \, f^{(\ell_1)}_{m_1}\, g^{(\ell_2)}_{m_2}.
% \end{equation}
% Diagonal and off-diagonal blocks are assembled from node and pair features,
% and the Hamiltonian is symmetrized as
% \begin{equation}
% \mathbf H \leftarrow \tfrac12(\mathbf H+\mathbf H^\top),
% \end{equation}
% ensuring Hermiticity while preserving SO(3) equivariance.

% \textbf{Energy and force evaluation from predicted Hamiltonian.}
% To evaluate the physical accuracy of predicted Hamiltonians, we compute energies and forces within the KS-DFT formalism. Given occupied orbitals $\{\psi_i\}_{i \in \mathcal O}$ with orbital energies
% $\{\epsilon_i\}$, we define the \emph{band energy} as $E_{\mathrm{band}}$ as the sum of occupied orbital energies: $E_{\mathrm{band}}\equiv\sum_{i \in \mathcal O} \epsilon_i=\sum_{i \in \mathcal O} \langle \psi_i | \hat H_{\mathrm{KS}} | \psi_i \rangle$.

% The total KS energy is then expressed as
% \begin{equation}
%     E_{\mathrm{KS}}[\rho] =
%     E_{\mathrm{band}}+ E_{\mathrm{corr}}[\rho] + E_{\mathrm{nuc}},
% \end{equation}
% where $E_{\mathrm{corr}}[\rho]$ represents density-dependent correction terms,
% including exchange-correlation and double-counting contributions, and
% $E_{\mathrm{nuc}}$ denotes the nuclear repulsion energy. Details of these terms are provided in Appendix~XXX.

% Atomic forces are obtained as derivatives of the total energy with respect to
% nuclear positions,
% \begin{equation}
%     \mathbf F_I
%     =
%     -\frac{\partial E_{\mathrm{KS}}}{\partial \mathbf R_I},
% \end{equation}
% where $\mathbf R_I$ denotes the position of atom $I$.
% The explicit evaluation of this derivative and its relation to the
% self-consistency of the Hamiltonian are discussed in the Appendix.

% \section{QHFlow2}

% We propose \textbf{QHFlow2}, a scalable Hamiltonian prediction framework designed to enable accurate SCF-free DFT calculations.
% Compared to prior QHFlow~\cite{kim2025high}, QHFlow2 improves computational scalability while maintaining high predictive accuracy, allowing reliable downstream evaluation of energies and forces without self-consistent iterations. Here, we briefly describe our framework, and details of the implementations are in Appendix~XXX.

% \paragraph{Flow-based formulation.}
% QHFlow2 adopts a flow-matching formulation for Hamiltonian prediction, following prior work~\cite{kim2025high}.
% In this setting, the target KS Hamiltonian $\mathbf{H}$ is
% obtained by transporting a simple reference matrix through a continuous-time flow.
% Given a flow time $t \in [0,1)$, the model predicts the target Hamiltonian
% $\mathbf{H}=\hat{\mathbf{H}}_1$ conditioned on the molecular geometry and the intermediate state $\mathbf{H}_t$, from which the instantaneous velocity
% $\mathbf{v}_t=(\hat{\mathbf{H}}_1-\mathbf{H}_t)/(1-t)$ is recovered.
% This formulation treats the Hamiltonian as a coupled object evolving continuously over time, rather than as a collection of independently predicted matrix entries, while remaining computationally efficient for high-dimensional Hamiltonian matrices.

% \paragraph{Architecture overview.}
% Within this flow-based framework, QHFlow2 is implemented as an equivariant message passing neural network that alternates between node-wise and edge-wise feature transformations, following scalable equivariant architectures~\citep{fu2025learning}.
% The model takes as input molecular geometry $\mathbf{M}=\{(Z_i,\mathbf{r}_i)\}_{i=1}^N$, a set of matrix components $\{\mathbf{F}_k\}_{k=1}^K$ sharing the block structure of the KS Hamiltonian (e.g., the intermediate flow Hamiltonian $\mathbf{H}_t$ and overlap matrix $\mathbf{S}$), and the flow time $t$.

% QHFlow2 maintains atom-centered node representations and pairwise edge representations. Node features encode on-site (diagonal) information associated with atomic orbitals, while edge features explicitly model inter-site (off-diagonal) interactions between atom pairs, which constitute the majority of Hamiltonian matrix elements in realistic basis sets.
% Accordingly, the Hamiltonian is constructed as an atom-wise block matrix
% $\mathbf{H}=\begin{pmatrix}\mathbf{H}_{ii} & \mathbf{H}_{ij}\\ \mathbf{H}_{ji} & \mathbf{H}_{jj}\end{pmatrix}$, where diagonal blocks $\mathbf{H}_{ii}$ are parameterized from node features and off-diagonal blocks $\mathbf{H}_{ij}$ are parameterized directly from edge features.

% \paragraph{Initial embeddings.}
% Each matrix component $\mathbf{F}_k$ is embedded into equivariant matrix features using a learnable matrix embedding. Atomic numbers $Z_i$ are encoded via a learnable atom embedding, and the flow time $t$ is mapped to a rotation-invariant time embedding. These embeddings are incorporated into the initial node representations, ensuring that atomic identity, matrix context, and flow-time conditioning are available throughout the network. Edge features are initialized from interatomic distances and relative displacement vectors using gaussian radial embedding~\cite{bartok2012representing}.

% \paragraph{Equivariant message passing.}
% Node and edge representations are iteratively updated through multiple layers of SO(2) convolutions. At each layer, node representations and pairwise edge representations are jointly processed by aligning each edge with a local coordinate frame and applying angularly separable interactions.
% This design enables efficient propagation of high-order angular information across the
% molecular graph while preserving equivariance. Throughout message passing, edge features play a central role, as they directly parameterize off-diagonal Hamiltonian blocks corresponding to atom-atom interactions.

% While SO(2)-equivariant convolutions provide an efficient backbone for propagating angular information in local coordinate frames, they primarily operate through angularly separable interactions.
% As a result, certain inter-angular momentum couplings relevant for Hamiltonian modeling are not explicitly parameterized within the SO(2) backbone alone.
% To incorporate such couplings, we lift edge features via an SO(3) tensor product, following standard equivariant constructions.

% The resulting tensor-expanded representations are then combined with the original
% SO(2)-processed features, enabling a trade-off between computational efficiency and angular expressivity.
% Throughout the network, node-wise and edge-wise representations are updated in an
% interleaved manner, allowing QHFlow2 to jointly model on-site (diagonal) and inter-site (off-diagonal) Hamiltonian contributions within a unified framework. Ablation study of edge representation choices in Appendix XXX.


% \paragraph{Hamiltonian construction via tensor expansion.}
% After message passing, node and edge representations are mapped to Hamiltonian blocks using a tensor expansion based on Clebsch-Gordan decomposition~\cite{schutt2019unifying,yu2023efficient}.
% This construction ensures that the resulting Hamiltonian blocks transform equivariantly under three-dimensional rotations, yielding an SO(3)-equivariant matrix representation that is consistent with the angular momentum structure of atomic orbitals~\cite{kim2025high}.
% Both diagonal (on-site) and off-diagonal (inter-site) blocks are constructed from the
% corresponding node and edge representations in a symmetry-consistent manner.

% To enforce the Hermitian structure of the Hamiltonian, we explicitly symmetrize the
% predicted matrix by averaging it with its transpose $\mathbf{H} \;\leftarrow\; \tfrac{1}{2}\bigl(\mathbf{H} + \mathbf{H}^\top\bigr)$.
% The symmetrized Hamiltonian is then used for all downstream electronic structure
% calculations.
% This procedure guaranties the required symmetry properties while preserving rotational
% equivariance, resulting in a structured Hamiltonian matrix suitable for electronic structure calculations.






% \section{Design Choices for Hamiltonian Prediction}
% This section introduces the design space of Hamiltonian prediction for SCF-free DFT. We first define a common task formulation for Hamiltonian prediction, followed by a description of a generic backbone architecture that serves as a shared framework across different approaches. Within this framewrok, we discuss three key design choices: (1) Azimuthal symmetry breaking in pair representation, (2) the learning objective, and (3) condition on an initial Hamiltonian. We conclude this section by summarizing these design choices and describing how they are instantiated in our QHFlow2.

% \subsection{Problem formulation}
% Given a molecular geometry $\mathbf{M} = \{(Z_i, \mathbf{r}_i)\}_{i=1}^N$, the task of Hamiltonian prediction is to infer the corresponding Kohn-Sham Hamiltonian $\mathbf{H}$, which encodes the electronic structure of the system. Diagonalizing $\mathbf{H}$ yields orbital energies $\boldsymbol{\epsilon}$ and density coefficients $\mathbf{C}$ (see \cref{XXX}), which are used to construct the electronic density $\rho$ and total energy $E_{\text{tot}}$ through standard DFT procedures.

% Because energies and forces are derived from the spectral value of
% $\mathbf{H}$ such as $\boldsymbol{\epsilon}$ and $\mathbf{C}$, the physical consistency of a predicted Hamiltonian is highly sensitive to spectral errors: small perturbations in matrix entries can lead to catastrophic deviations in orbital quantities. In SCF-free settings, where no iterative self-consistent correction is applied, such spectral sensitivity directly impacts the reliability of derived energies and forces. While we do not explicitly enforce spectral
% constraints during training, we empirically find that certain design
% choices lead to improved spectral accuracy, which we analyze in \cref{XXX}. 

% % \subsection{Backbone Framework.}
% % Our architecture consists of three main components: node and edge embeddings, pairwise feature construction, and tensor expansion. Among these, the node-embedding and tensor-expansion modules are shared across all design choices considered in this work, while variations in pairwise feature construction are discussed separately in Section~XXX. We provide a concise description of the backbone here, with full architectural details deferred to Appendix~XX.

% \subsection{Backbone Framework}
% Our architecture takes as input a molecular configuration $\mathbf{M}$, a set of matrix components $\{\mathbf{F}_k\}$, and a flow-matching time $t\in[0,1)$. Each matrix component $\mathbf{F}_k$ corresponds to a matrix sharing the same structural form as the Hamiltonian $\mathbf{H}$. The backbone constructs equivariant node and edge features through embedding and feature propagation steps, which are shared across all model variants considered in this work.


% \paragraph{Embeddings.}
% $\mathbf{F}_k$ is embedded into an equivariant
% matrix feature $\mathbf{f}_k=\bigoplus_{\ell=0}^{\ell_{\max}} \mathbf{f}_k^{(\ell)}=g_{\text{matrix}}^{\theta_k}(\mathbf{F}_k),$
% where $g_{\text{matrix}}^{\theta_k}$ is a learnable equivariant matrix
% embedding that produces tensor features up to
% $\ell_{\max}$. Atomic numbers $Z_i$ are encoded via a learnable atomic embedding $\mathbf{a}_i = g_{\text{atom}}^{\theta_{\text{a}}}(Z_i)$, and the time variable $t$ is embedded using a sinusoidal time embedding $\boldsymbol{\tau}_t = g_{\text{time}}(t)$. Both embeddings are rotation-invariant. The initial node feature $\mathbf{z}_i$ is defined as
% \begin{equation}
% \mathbf{z}_i^{(0)} := g_{\text{mix}}^{\theta_0}
% \left(\mathbf{a}_i, \boldsymbol{\tau}_t, \{\mathbf{f}_k^{(0)}\}_{k=1}^K \right), \quad
% \mathbf{z}_i^{(\ell)} := \sum_{k=1}^K \mathbf{f}_k^{(\ell)},
% \end{equation}
% where $g_{\text{mix}}^{\theta_0}$ integrates atomic, temporal, and matrix embeddings. The edge features $\mathbf{e}_{ij}$ are initialized using a Gaussian distance embedding $f_{\text{gauss}}^{\theta_g}(\mathbf{r}_{ij})$, where $\mathbf{r}_{ij}$ denotes the interatomic displacement vector.

% % The edge features $\mathbf{e}_{ij} = \bigoplus_{\ell=0}^{\ell_{\max}} \mathbf{e}_{ij}^{(\ell)}$ are initialized using a Gaussian distance embedding, with $\mathbf{e}_{ij}^{(0)} = f_{\text{gauss}}^{\theta_g}(\mathbf{r}_{ij})$, where $\mathbf{r}_{ij}$ denotes the interatomic displacement vector.

% % \paragraph{SO(2)-Equivariant Feature Propagation.}
% % Node and edge features are propagated using SO(2)-equivariant convolution layers~\cite{XXX_SO2_conv}. The key idea is that the tensor product can be sparse with a proper local frame. For an edge $(i,j)$, a local frame can be selected with $\mathbf{R}_{ij}\hat {\mathbf{r}}_{ij}=\hat{\mathbf{z}}$. In this local frame, spherical harmonics $\textbf{Y}^{(l)}_m(\mathbf{R}_{ij}\hat {\mathbf{r}}_{ij})\propto \delta^{(l)}_m$. Under this sparsification, equivariant features decompose into angular subspaces indexed by the frequency $m$.
% % In a real-valued representation, the components of order $m$ and $-m$ transform under a rotation by angle $\phi$ as
% % \begin{equation}
% % \label{eq:so2_rotation}
% % \begin{pmatrix}
% % (\mathbf{x})_{m} \\
% % (\mathbf{x})_{-m}
% % \end{pmatrix}
% % \;\mapsto\;
% % \begin{pmatrix}
% % \cos(m\phi) & -\sin(m\phi) \\
% % \sin(m\phi) & \cos(m\phi)
% % \end{pmatrix}
% % \begin{pmatrix}
% % (\mathbf{x})_{m} \\
% % (\mathbf{x})_{-m}
% % \end{pmatrix}.
% % \end{equation}
% % Equivariance with respect to this transformation constrains linear interaction operators to act independently
% % within each $(m,-m)$ block, yielding an angularly separable, block-diagonal structure in the local frame.

% % Based on this structure, feature propagation is implemented through edge-conditioned, channel-wise modulation.
% % Let $\tilde{\mathbf{z}}_j^{(\ell)}:=\mathbf{R}_{ij}\cdot\mathbf{z}_j^{(\ell)}$ denote the degree-$\ell$ features of node $j$ expressed in the local frame associated with edge $(i,j)$
% % Messages are computed as
% % \begin{equation}
% % \label{eq:so2_conv_rigorous}
% % \mathbf{m}_{ij}^{(\ell)}
% % =
% % \mathbf{R}_{ij}^{-1}
% % \left(
% % \bigoplus_{m=-\ell}^{\ell}
% % \mathbf{W}^{(\ell)}_{m}(\mathbf{e}_{ij}) \,
% % \tilde{\mathbf{z}}_{j,m}^{(\ell)}
% % \right),
% % \end{equation}

% % where $\mathbf{W}^{(\ell)}(\mathbf{e}_{ij})$ denotes learnable weights derived from edge attributes
% % $\mathbf{e}_{ij}$, and $\odot$ denotes component-wise multiplication applied independently to each angular subspace.
% % The resulting messages are rotated back to the global frame and aggregated over neighbors,
% % \begin{equation}
% % \mathbf{z}_i^{(\ell)} \leftarrow \sum_{j \in \mathcal{N}(i)} \mathbf{m}_{ij}^{(\ell)} .
% % \end{equation}

% % \paragraph{Efficient SO(2)-Equivariant Feature Propagation.}
% % We propagate features using SO(2)-equivariant convolutions by expressing interactions in a local coordinate system
% % associated with each edge.
% % For an edge $(i,j)$, we rotate the relative position vector $\mathbf{r}_{ij}$ to align with the canonical $z$-axis,
% % and express the neighbor feature in this local frame as
% % $\tilde{\mathbf{z}}_j^{(\ell)} := \mathbf{R}_{ij}\mathbf{z}_j^{(\ell)}$.
% % In this coordinate system, rotations around the interatomic axis reduce to SO(2) rotations.

% % Under SO(2), degree-$\ell$ features decompose into angular channels indexed by $m=-\ell,\ldots,\ell$.
% % In a real-valued representation, the pair $(m,-m)$ forms a two-dimensional subspace that transforms as a planar rotation.
% % We group this pair into a block
% % \[
% % \tilde{\mathbf{z}}_{j,|m|}^{(\ell)} :=
% % \begin{pmatrix}
% % \tilde{\mathbf{z}}_{j,m}^{(\ell)}\\
% % \tilde{\mathbf{z}}_{j,-m}^{(\ell)}
% % \end{pmatrix},
% % \qquad m>0,
% % \]
% % while the $m=0$ component remains one-dimensional.

% % SO(2) equivariance constrains linear interactions to act independently on each $|m|$ block.
% % Accordingly, we compute edge-conditioned messages by applying a simple block-wise transformation
% % within each angular subspace.
% % For $m>0$, the local-frame message is given by
% % \begin{equation}
% % \label{eq:so2_block_message_intuitive}
% % \tilde{\mathbf{m}}_{ij,|m|}^{(\ell)}
% % =
% % \begin{pmatrix}
% % \mathbf{Y}_{ij,m}^{(\ell)} & -\mathbf{Y}_{ij,-m}^{(\ell)}\\
% % \mathbf{Y}_{ij,-m}^{(\ell)} & \mathbf{Y}_{ij,m}^{(\ell)}
% % \end{pmatrix}
% % \tilde{\mathbf{z}}_{j,|m|}^{(\ell)},
% % \end{equation}
% % where the coefficients $\mathbf{Y}_{ij,\pm m}^{(\ell)}$ are learned from edge attributes $\mathbf{e}_{ij}$.
% % This $2\times2$ structure is the real-valued form of a complex multiplication and preserves the SO(2) transformation
% % within the $(m,-m)$ subspace.
% % For $m=0$, we use a standard linear map
% % $\tilde{\mathbf{m}}_{ij,0}^{(\ell)}=\mathbf{Y}_{ij,0}^{(\ell)}\tilde{\mathbf{z}}_{j,0}^{(\ell)}$.

% % Collecting all angular blocks yields the full local-frame message
% % $\tilde{\mathbf{m}}_{ij}^{(\ell)}$, which is then rotated back to the global frame:
% % \[
% % \mathbf{m}_{ij}^{(\ell)}=\mathbf{R}_{ij}^{-1}\tilde{\mathbf{m}}_{ij}^{(\ell)}.
% % \]

% % Messages from neighboring nodes are aggregated by summation,
% % \[
% % \mathbf{h}_i^{(\ell)}=\sum_{j\in\mathcal{N}(i)}\mathbf{m}_{ij}^{(\ell)},
% % \]
% % and used to update the node representation via a type-preserving update operator,
% % \[
% % \mathbf{z}_i^{(\ell)} \leftarrow 
% % \mathrm{Upd}^{(\ell)}\!\Big(
% % \mathbf{z}_i^{(\ell)},
% % \mathbf{h}_i^{(\ell)},
% % \{\mathbf{e}_{ij}\}_{j\in\mathcal{N}(i)}
% % \Big),
% % \]
% % where $\mathrm{Upd}^{(\ell)}$ consists of residual mixing followed by equivariant gating and normalization.

% % At the final layer, the pair representation is updated using the corresponding node features,
% % \begin{equation}
% % \label{eq:so2_msg}
% % \mathbf{z}_{ij}^{(\ell)} \leftarrow 
% % \mathrm{Upd}^{(\ell)}\!\Big(
% % [\mathbf{z}_i^{(\ell)}, \mathbf{z}_j^{(\ell)}],
% % \mathbf{h}_i^{(\ell)},
% % \mathbf{e}_{ij}
% % \Big).
% % \end{equation}


% % \textbf{Tensor Expansion for Hamiltonian Construction.}
% % From the updated node features $\mathbf{z}_i$ and edge features $\mathbf{e}_{ij}$,
% % we construct a unified equivariant feature
% % \begin{equation}
% % \mathbf{w}_{ij} =
% % \begin{cases}
% % \mathbf{z}_i, & i = j, \\
% % \mathbf{e}_{ij}, & i \neq j ,
% % \end{cases}
% % \end{equation}
% % which represents on-site and inter-site interactions in a common form.
% % Each feature is expressed as a direct sum of irreducible representations (irreps),
% % \begin{equation}
% % \mathbf{w}_{ij} = \bigoplus_{\ell=0}^{\ell_{\max}} \mathbf{w}_{ij}^{(\ell)}, \qquad 
% % \mathbf{w}_{ij}^{(\ell)} \in \mathbb{R}^{2\ell+1},
% % \end{equation}
% % and transforms equivariantly under rotations.

% % To obtain matrix-valued representations compatible with orbital angular momentum coupling,
% % we apply tensor expansion via Clebsch--Gordan decomposition.
% % For each pair of irreps $(\ell_1,\ell_2)$, we decompose
% % \begin{equation}
% % \mathbf{w}_{ij}^{(\ell_1)} \otimes \mathbf{w}_{ij}^{(\ell_2)}
% % = \bigoplus_{\ell = |\ell_1-\ell_2|}^{\ell_1+\ell_2}
% % \mathbf{u}_{ij}^{(\ell)},
% % \end{equation}
% % with components
% % \begin{equation}
% % \mathbf{u}_{ij,m}^{(\ell)}
% % =
% % \sum_{m_1,m_2}
% % C^{\ell m}_{\ell_1 m_1,\, \ell_2 m_2}\,
% % \mathbf{w}_{ij,m_1}^{(\ell_1)}\,
% % \mathbf{w}_{ij,m_2}^{(\ell_2)} .
% % \end{equation}

% % The resulting coupled features form a complete equivariant basis for Hamiltonian blocks
% % and are linearly projected to assemble the final matrix representation,
% % guaranteeing exact $\mathrm{SO}(3)$ equivariance.



% % The resulting tensor-expanded blocks are aggregated over all atom pairs and assembled into the full Hamiltonian matrix
% % $\hat{\mathbf{H}}$, structured as $K\times K$ sub-matrices corresponding to all pairwise combinations of basis-function groups.
% % By construction, all operations in this stage preserve SE(3) equivariance.


% % \textbf{Tensor Expansion for Matrix Construction.}
% % Given the updated node and edge features, the model constructs Hamiltonian matrix blocks by lifting the equivariant features to higher-order representations via tensor expansion. Specifically, atom-wise and pairwise irreducible representations are first predicted from the backbone features, yielding
% % \begin{align}
% % \mathbf{w}_{ii} &= \mathrm{TFN}_{\mathrm{s}}\!\left(\mathbf{z}_i, \{\mathbf{z}_k, \mathbf{e}_{ik}\}_{k\in\mathcal{N}_i}\right),\\
% % \mathbf{w}_{ij} &= \mathrm{TFN}_{\mathrm{p}}\!\left(\mathbf{z}_i, \mathbf{z}_j, \mathbf{e}_{ij}\right),
% % \end{align}
% % where each output is a collection of irrep vectors
% % $\mathbf{w}_{ij} = \{\mathbf{w}_{ij}^{(\ell)}\}_{\ell\in L_i}$.

% % Hamiltonian blocks are then formed by Clebsch--Gordan tensor products of the predicted irreps.
% % For each atom pair $(i,j)$ and angular-momentum pair $(\ell_1,\ell_2)$, we construct
% % \[
% % \mathbf{H}_{ij}^{(\ell_1,\ell_2)}
% % =
% % \sum_{\ell\in L_i}
% % F_{ij}^{(\ell_1,\ell_2,\ell)}
% % \left(
% % \bigotimes \mathbf{w}_{ij}^{(\ell)}
% % \right)^{(\ell_1,\ell_2)},
% % \]
% % where $\otimes$ denotes the Clebsch--Gordan tensor product and
% % $F_{ij}^{(\ell_1,\ell_2,\ell)}$ are learnable coefficients.
% % The case $i=j$ corresponds to diagonal (atom-wise) blocks, while $i\neq j$ yields off-diagonal (pairwise) interactions.

% % The resulting tensor-expanded blocks are aggregated over all atom pairs and assembled into the full Hamiltonian matrix
% % $\hat{\mathbf{H}}$, structured as $K\times K$ sub-matrices corresponding to all pairwise combinations of basis-function groups.
% % By construction, all operations in this stage preserve SE(3) equivariance.


% \subsection{Spectrally Complete Interaction Modeling}

% \paragraph{Limits of Local-Frame SO(2) Factorization.}
% SO(2)-equivariant backbones achieve high efficiency by operating in local frames and factorizing angular structure into independent channels. This formulation yields block-diagonal or sparsely coupled interactions across angular momentum degrees, preserving equivariance on linear operations. In practice, however, channel-wise factorization, reduced-rank mixing, and the use of equivariant nonlinearities lead to a quasi-equivariant approximation of full SO(3) interactions. As a consequence, the backbone effectively explores only a restricted subset of the full space of equivariant bilinear interactions, and inter-$\ell$ couplings are captured in a limited manner. The backbone alone may therefore lack the spectral resolution required to capture fine orbital splittings of the Hamiltonian, particularly in SCF-free settings where no iterative correction is applied (see Appendix~XXX).


% \paragraph{Orbital-Aware Spectral Interaction Layers.}
% To recover angular momentum couplings that are weakly expressed in local-frame SO(2) backbones,
% we introduce an orbital-aware \emph{Spectral Interaction layer} based on $SO(3)$ tensor products.
% This layer enriches backbone features with explicit inter-$\ell$ interactions
% prior to Hamiltonian construction.

% Let $\mathbf{z}_i=\bigoplus_{\ell}\mathbf{z}_i^{(\ell)}$ denote equivariant node features
% produced by the backbone.
% From these, we construct pairwise equivariant features
% \begin{equation}
% \mathbf{z}_{ij}^{(\ell)} = g_{\mathrm{pair}}^{(\ell)}\!\left(\mathbf{z}_i^{(\ell)},\mathbf{z}_j^{(\ell)}\right),
% \end{equation}
% which preserve angular information but do not mix different $\ell$ channels.
% The Spectral Interaction layer introduces such mixing via $SO(3)$ tensor products.
% For each pair $(\ell_1,\ell_2)$, we compute coupled features
% \begin{equation}
% \mathbf{u}_{ij}^{(\ell)} =
% \sum_{m_1,m_2}
% C^{\ell m}_{\ell_1 m_1,\,\ell_2 m_2}\,
% \mathbf{z}_{ij,m_1}^{(\ell_1)}\,
% \mathbf{z}_{ij,m_2}^{(\ell_2)},
% \end{equation}
% where $\ell \in \{|\ell_1-\ell_2|,\dots,\ell_1+\ell_2\}$. The coupled features are linearly projected and combined with a residual connection,
% \begin{equation}
% \tilde{\mathbf{z}}_{ij}^{(\ell)} = \mathbf{z}_{ij}^{(\ell)} + \sum_{\ell'} F_{ij}^{(\ell,\ell')}(\mathbf{r}_{ij})\,\mathbf{u}_{ij}^{(\ell')},
% \end{equation}
% and passed to the tensor expansion module, where they are assembled into Hamiltonian matrix blocks.
% By explicitly introducing inter-$\ell$ mixing while preserving the original backbone features,
% the Spectral Interaction layer provides a spectrally complete interaction space
% for SCF-free Hamiltonian prediction.





% \subsection{Learning Objectives}
% \seongsu{\textbf{Regression.}}

% \textbf{Equivariant Flow Matching.} We train QHFlow-v2 using conditional flow matching to model the distribution of converged ground-state Hamiltonians.
% We define a time-dependent vector field $v_t(\mathbf{H}_t \mid \mathcal{M})$ that transports a Hamiltonian sample $\mathbf{H}_t$ along a continuous path parameterized by $t\in[0,1]$.

% The path is defined by linear interpolation between a noise sample $\mathbf{H}_0\sim\mathcal{N}(0,\mathbf{I})$ and the ground-truth Hamiltonian $\mathbf{H}_1$,
% \begin{equation}
% \mathbf{H}_t = (1-t)\mathbf{H}_0 + t\mathbf{H}_1,
% \qquad
% u_t(\mathbf{H}_t \mid \mathbf{H}_1)=\mathbf{H}_1-\mathbf{H}_0.
% \end{equation}
% The model is trained by minimizing
% \begin{equation}
% \mathcal{L}_{\text{CFM}} =
% \mathbb{E}_{t,\mathbf{H}_0,\mathbf{H}_1}
% \left[
% \left\|
% v_t^\theta(\mathbf{H}_t,\mathcal{M})-(\mathbf{H}_1-\mathbf{H}_0)
% \right\|^2
% \right].
% \end{equation}
% Unlike pointwise regression approaches, which often struggle to capture the structured correlations inherent in Hamiltonian matrices and suffer from high predictive uncertainty, our flow-based formulation treats the Hamiltonian as a coupled object and explicitly models correlations among its entries, enabling stable SCF-free electronic structure calculations. See the ablations in XXX.


% % \subsection{Conditioning on an Initial Hamiltonian}
% \subsection{Our Design Choices}

% \iffalse
% \section{Method}

% We introduce QHFlow2, a generative framework for predicting converged Kohn-Sham Hamiltonians $\mathbf{H}$ directly from molecular configurations $\mathcal{M}=(\mathbf{X}, \mathbf{Z})$, where $N$ is the number of atoms, $\mathbf{X} \in \mathbb{R}^{N \times 3}$ denotes atomic coordinates, and $\mathbf{Z} \in \mathbb{N}^{N}$ denotes atomic numbers. our model outputs the Hamiltonian matrix $\mathbf{H}$ expressed in a fixed atomic orbital basis. Our model is built upon two core components: (1) a hybrid equivariant architecture that efficiently extracts node features via scalable SO(2) convolutions and subsequently lifts them to form a rigorous SO(3) pair representation, and (2) an equivariant conditional flow matching objective designed to model the complex joint distribution of ground-state Hamiltonians. We describe each component in detail below.

% \subsection{Hybrid SO(2)-SO(3) Equivariant Architecture}

% Unlike the MLIPS, where predictions are made nodewise, learning Hamiltonian matrices requires the model to make predictions for both nodes (intra-atomic orbital interactions) and directed edges (inter-atomic orbital interactions). We adopt a hybrid equivariant architecture in which SO(2)-equivariant convolutions are used to encode node-level chemical information, while SO(2)-SO(3) hybrid layers are used to construct pairwise representations that capture the detailed geometric interactions required for Hamiltonian prediction. 

% \paragraph{Node Embedding via SO(2) Convolutions.}

% Our node embedding layer is based on the eSEN. Since our model is flow matching conditioned on the current Hamiltonian $H_t$, our model takes input as $(\mathcal{M}, H_t)$, we build a displacement vector $\mathbf{r}_{ij}\in \mathbb R^3$ with $i,j=1,\ldots,N$. We initialize node and edge embeddings $z_{ij}$ as follows:
% \begin{equation}
%     z_{ij}=f^{(0)}(Z_i,\mathbf r_{ij}).
% \end{equation}
% Our architecture begins by representing the molecular structure as a geometric graph where nodes correspond to atoms and edges connect atom pairs. We initialize the feature of each node $i$ using a learnable atomic embedding based on its nuclear charge $Z_i$:\begin{equation}\mathbf{h}i^{(0)} = f{\text{atom}}(Z_i).\end{equation}These embeddings are iteratively refined through $L$ layers of an SO(2)-equivariant message-passing network, inspired by the efficient eSEN architecture. At each layer $k$, the node feature $\mathbf{h}_i^{(k)}$ is updated by aggregating messages from its local neighborhood $\mathcal{N}(i)$:
% \begin{equation}
% \mathbf{h}i^{(k+1)} = \phi^{(k)}\left( \mathbf{h}_i^{(k)}, \sum_{j\in\mathcal{N}(i)} \psi^{(k)}_{\text{SO(2)}}\left(\mathbf{h}j^{(k)}, r_{ij}\right) \right),
% \end{equation}
% where $r_{ij}=\|\mathbf{X}_i-\mathbf{X}_j\|$ is the interatomic distance, and $\phi^{(k)}$ and $\psi^{(k)}_{\text{SO(2)}}$ denote learnable SO(2)-equivariant update and message functions, respectively. Crucially, this module treats features as complex-valued phasors, encoding angular correlations through phase interactions under SO(2) symmetry. This formulation avoids the computationally expensive tensor products required for full SO(3) equivariance, thereby substantially reducing the computational cost while preserving sufficient expressivity to model local chemical environments. The final output after $L$ layers, denoted as $\mathbf{h}_i^{\text{SO(2)}} := \mathbf{h}_i^{(L)}$, serves as a compact representation of the local chemical context and many-body interactions.

% \paragraph{Hybrid Edge Feature Construction.}
% Hamiltonian matrix elements must transform equivariantly under three-dimensional rotations.
% To this end, we construct edge features that combine chemical information extracted by the SO(2)-equivariant backbone with explicit geometric structure.

% First, node embeddings $\mathbf{h}_i^{\text{SO(2)}}$ are projected into SO(3) irreducible representations to obtain rotationally equivariant node features,
% \begin{equation}
% \mathbf{h}_i^{\text{SO(3)}} = \mathcal{P}\!\left(\mathbf{h}_i^{\text{SO(2)}}\right),
% \end{equation}
% where $\mathcal{P}$ denotes a learnable linear projection into SO(3) irreps.

% Using these node features, we construct initial SO(3)-equivariant edge features by combining pairwise node interactions with spherical harmonics that encode relative orientation,
% \begin{equation}
% \mathbf{e}_{ij}^{\text{SO(3)}} =
% \mathbf{h}_i^{\text{SO(3)}} \otimes
% \mathbf{h}_j^{\text{SO(3)}} \otimes
% Y(\hat{\mathbf{r}}_{ij}),
% \end{equation}
% where $\hat{\mathbf{r}}_{ij}=(\mathbf{X}_i-\mathbf{X}_j)/r_{ij}$.

% In parallel, the SO(2)-equivariant backbone produces edge features $\mathbf{e}_{ij}^{\text{SO(2)}}$ that encode distance-dependent interaction strengths and chemical compatibility.
% We combine chemical and geometric information by modulating the SO(3)-equivariant edge features with the SO(2) edge features,
% \begin{equation}
% \mathbf{m}_{ij} =
% \mathbf{e}_{ij}^{\text{SO(2)}} \otimes
% \mathbf{e}_{ij}^{\text{SO(3)}}.
% \end{equation}
% This hybrid construction preserves rotational equivariance while allowing chemically informed features to influence geometrically structured orbital interactions.
% \fi


% % \paragraph{Tensor Expansion for Hamiltonian Construction.}

% % The edge features $\mathbf{m}_{ij}$ are mapped to Hamiltonian matrix blocks using an equivariant tensor expansion, following the formulation of QHNet. The Kohn-Sham Hamiltonian is expressed in an atomic orbital basis, where each block $\mathbf{H}_{ij}$ corresponds to interactions between orbitals centered on atoms $i$ and $j$.

% % Let $l_1$ and $l_2$ denote the angular momenta of the interacting orbitals.
% % The corresponding block $\mathbf{H}_{ij}^{(l_1,l_2)}$ transforms according to irreducible representations of degrees
% % $l \in \{|l_1-l_2|,\ldots,l_1+l_2\}$.
% % We reconstruct each block as
% % \begin{equation}
% % \mathbf{H}_{ij}^{(l_1,l_2)} =
% % \sum_{l=|l_1-l_2|}^{l_1+l_2}
% % F_{ij}^{(l_1,l_2,l)} \cdot \mathbf{w}_{ij}^{(l)},
% % \end{equation}
% % where $\mathbf{w}_{ij}^{(l)}$ denotes the degree-$l$ component of $\mathbf{m}_{ij}$ and $F_{ij}^{(l_1,l_2,l)}$ are learnable coefficients.
% % This construction is consistent with the Wigner--Eckart theorem and guarantees rotational equivariance of the predicted Hamiltonian.

==> 4_method_old.tex <==
\section{Quantum Hamiltonian flow matching (\QHFlow)}
\label{sec:method}

\subsection{Flow matching for Hamiltonian matrix}
\label{sec:fm}
\textbf{Problem formulation.} Our goal is to train a model that predicts the Hamiltonian matrix $\mathbf{H}$ from a molecular configuration $\mathcal{M}=(\mathbf{x}, \mathbf{h})$. Here, for a molecule $\mathcal{M}$ with $M$ atoms, $\mathbf{x} \in \mathbb{R}^{M\times 3}$ and $\mathbf{h}\in \mathbb{R}^{M\times D}$ denotes the atom-wise coordinates and $D$-dimensional atom-wise features, respectively. We train the model using a atomic dataset $\mathcal{A}$ with a sample $(\mathcal{M}, \mathbf{H})$ corresponding to a molecular configuration $\mathcal{M}$ and its Hamiltonian matrix $\mathbf{H}$ obtained from conventional RH-DFT solvers. 


\textbf{Conditional flow matching (CFM).} We first propose the flow matching for Hamiltonian matrix, by parameterizing our model as a continuous normalizing flow (CNF) model. Our CNF aims to learn a time-dependent vector field $v_{t}(\cdot | \mathcal{M})$ that outputs the Hamiltonian matrix $\mathbf{H}$ from solving the ODE $\frac{\rd}{\rd t} \mathbf{H}_{t} = v_t(\mathbf{H}_{t} | \mathcal{M})$ for time $t \in (0,1]$. The ODE starts from $\mathbf{H}_{0}$ sampled from the prior distribution $p_{0}$ defined over the space $\mathbb{R}^{B\times B}$ of Hamiltonian matrices and outputs a Dirac distribution centered at the Hamiltonian matrix $\mathbf{H}$. To this end, we learn the vector field $v_{t}^{\theta}\approx v_{t}$ to match the distribution induced from the empirical distribution $(\mathcal{M}, \mathbf{H}_{1})\sim \mathcal{A}$ associated with conditional probability paths $p_{t}(\mathbf{H}_{t}|\mathbf{H})$. Importantly, the conditional path $p_{t}(\mathbf{H}_{t}|\mathbf{H})$ is expressed using a closed-form conditional vector field $u_{t}(\cdot | \mathbf{H}_{1})$:
    $\frac{\rd}{\rd t} \mathbf{H}_{t} = u_t(\mathbf{H}_{t} | \mathbf{H}_{1}, \mathcal{M})$ for $\mathbf{H}_0 \sim p_{0}$.

% Here, I should write the H_t=(1-t)H_0 + t H_t.

Following previous works \cite{yimimproved,kim2024mofflow}, we parameterize the conditional probability path using linear interpolation between $\mathbf{H}_{0}$ and $\mathbf{H}_{1}$, resulting in the conditional vector field $u_{t}(\mathbf{H}_{t}|\mathbf{H}_{1}, \mathcal{M}) = \frac{\mathbf{H}_{1}-\mathbf{H}_{t}}{1-t}$. To train the CNF, we use the conditional flow matching objective defined as follows: 
\begin{equation}
    \mathcal{L}_{\text{CFM}} = \mathbb{E}_{(\mathbf{H}, \mathcal{M})\sim \mathcal{A}, t \sim \mathcal{U}(0,1), \mathbf{H}_{t} \sim p_{t}(\cdot | \mathbf{H})} \left[ \left\| v_{t}^{\theta}(\mathbf{H}_{t}) - u_t(\mathbf{H}_{t} | \mathbf{H}_{1}, \mathcal{M}) \right\|_2^2 \right],
\end{equation}
where $\mathcal{U}$ denotes an uniform distribution and $\|\cdot \|_{2}^{2}$ denotes the Frobeneous norm of a matrix. In practice, we parameterize the vector field by $v_{t}^{\theta}=\frac{\mathbf{H}_{1}^{\theta}(\mathbf{H}_{t}, \mathcal{M}) - \mathbf{H}_{t}}{1-t}$ using a neural network $\mathbf{H}_{1}^{\theta}(\cdot)$. This results in the final loss function:
\begin{equation}
\mathcal{L}_{\text{CFM}}=\mathbb{E}_{(\mathbf{H}, \mathcal{M})\sim \mathcal{A}, t \sim \mathcal{U}(0,1), \mathbf{H}_{t} \sim p_{t}(\cdot | \mathbf{H})}
     \left[
        \frac{1}{(1-t)^{2}}\left\|\mathbf{H}^{\theta}_{1}(\mathbf{H}_{t}, \mathcal{M})-\mathbf{H}_{1,\mathcal{M}}\right\|_{2}^{2}
     \right],
     \label{eq:CFM-ours}
\end{equation}
which one could interpret as training $\mathbf{H}_{1}^{\theta}$ to approximate the true Hamiltonian matrix $\mathbf{H}$ from its noisy versions $\mathbf{H}_{t}$. We provide a full description of the training and sampling algorithms in \cref{app:algorithms}.

\textbf{Fine-tuning for energy alignment.}
In practice, many important quantum properties derived from DFT rely directly on orbital energies. To improve the accuracy of such downstream quantities including orbital energies, highest occupied molecular orbital (HOMO) energy, loweset unoccupied molecular orbital (LUMO) energy, and the HOMO–LUMO gap, we introduce a fine-tuning strategy that explicitly aligns the predicted orbital energies with their ground-truth DFT references.
This approach is motivated by the weighted alignment loss (WALoss) introduced in WANet~\cite{lienhancing}, which improves prediction quality by aligning the energy of predicted and reference matrix. Rather than incorporating this loss during full training, we adopt it as a post hoc fine-tuning objective.

Specifically, we define a fine-tuning objective that aligns the approximate orbital energies $\tilde{\bm{\epsilon}}$ derived from our predicted Hamiltonian matrix $\mathbf{H}_1^\theta$ from CNF with the ground-truth orbital energies $\bm{\epsilon}$ computed from RH-DFT as defined in \cref{eq:RH-DFT}:
\begin{equation}
\mathcal{L}_{\text{FT}}
    =\mathbb{E}_{(\mathbf{H}, \mathcal{M})\sim \mathcal{A}, t \sim \mathcal{U}(0,1), \mathbf{H}_{t} \sim p_{t}(\cdot | \mathbf{H})}
     \left[
        \left\|\operatorname{\tilde{\bm{\epsilon}}}\bigl(\mathbf{H}^{\theta}_{1}(\mathbf{H}_{t}, \mathcal{M})\bigr)
        -
        \operatorname{\bm{\epsilon}}\right\|_{2}^{2}
     \right]
\end{equation}
Here, the ground-truth orbital energies $\bm{\epsilon}$ are computed via the identity $\bm{\epsilon} = \mathbf{C}^\top \mathbf{H} \mathbf{C}$, which follows from the orthonormality condition $\mathbf{C}^\top \mathbf{S} \mathbf{C} = \mathbf{I}$, where $\mathbf{C}$ is the ground-truth coefficient matrix and $\mathbf{S}$ is the overlap matrix.
 Following WALoss, we estimate $\tilde{\bm{\epsilon}}$ using the predicted Hamiltonian: $\tilde{\bm{\epsilon}} =  \mathbf{C}^\top \mathbf{H}_1^\theta \mathbf{C} \approx (\mathbf{C}^\theta)^\top \mathbf{H}_1^\theta \mathbf{C}^\theta$, where $\mathbf{C}^\theta$ is the coefficient matrix obtained by solving the RH-DFT for the predicted Hamiltonian $\mathbf{H}_1^\theta$. We provide the implementation details in \cref{app:finetune}.

\subsection{SE(3)-equivariant flow matching with equivariant priors.}
Here, we introduce our approach to design our \QHFlow{} to satisfy SE(3)-equivariance. We follow the framework of \citet{song2023equivariant} to learn an equivariant vector field under an invariant prior. To handle translational symmetry, our networks operate in a mean-free system by centering the molecular coordinates $\mathbf{X}$ at the origin, \textit{i.e.}, set $\mathbf{X}\mapsto \mathbf{X}-\frac{1}{N}\bm{1}\bm{1}^{\top}\mathbf{X}$ given a vector $\bm{1} \in \mathbb{R}^{N\times 1}$ of ones. To make \QHFlow{} satisfy equivariance, we (1) parameterize the vector field $\smash{v_{t}^{\theta}}$ using a SO(3)-equivariant neural network \cite{yu2023efficient} and (2) propose \textit{Gaussian orthogonal ensemble (GOE)} and \textit{tensor expansion-based (TE)} priors for the Hamiltonian. The main challenge is to design new priors that are invariant to the rotation of the Hamiltonian matrix as described in \cref{eq:hamtrans}.

\textbf{Gaussian orthogonal ensemble (GOE) prior.} We here introduce a simple rotational invariant prior, the \textit{GOE} prior. A GOE is defined over matrices $\mathbf H \in \mathbb R^{n\times n}$, with each element drawn from a Gaussian distribution: $H_{ij} \sim \mathcal{N}(0, \sigma^2)$. The log-density is proportional to the Frobenius norm of the matrix, which is invariant under any transformations associated with SO(3) irreps, \textit{i.e.}, the 3D-rotation matrix ($\ell=1$) and even the high-rank Wigner D-matrices ($\ell\ge2$). Therefore, the prior satisfies the desired invariance, \textit{i.e.}, $p(\mathbf H)=p(\mathcal{D}(\mathbf R)\mathbf H\mathcal{D}(\mathbf R)^{-1})$ for all $\mathbf R\in \text{SO(3)}$. We provide the full proof for the SO(3)-invariance in \cref{app:proof_GOE}.


\textbf{Tensor expansion-based (TE) prior.}
We also introduce \textit{TE} prior, an SO(3)-invariant distribution constructed by first sampling an irrep vector $\mathbf{w}^{(\ell)}$, then applying tensor expansion to produce a matrix $\mathbf{H}^{(\ell_1,\ell_2)}\in \mathbb{R}^{(2\ell_1+1)\times(2\ell_2+1)}$ that transforms covariantly under rotation $\mathbf{R}\in\text{SO(3)}$:
\begin{equation}
    \mathbf{H}^{(\ell_1,\ell_2)} \xrightarrow{\mathbf{R}}
    D^{(\ell_1)}(\mathbf{R})
    \bigl(\mathbf{H}^{(\ell_1,\ell_2)}\bigr)
    D^{(\ell_2)}(\mathbf{R})^{-1}.
\end{equation}
To this end, we first design an SO(3)-invariant distribution of irrep vector $p(\mathbf w^{(\ell_{3})})$ by decomposing the vector into a radial and rotational parts: $\mathbf{w}^{(\ell)}= rD^{(\ell)}(\mathbf{R})\mathbf{w}^{(\ell_0)}$ where $r$ is a scalar norm and $\mathbf{w}^{(\ell_0)}$ is a fixed unit-norm irrep vector. \textit{i.e.}, $Y^\ell(\hat {\mathbf{r}}_0)$ for fixed direction $\hat {\mathbf{r}}_0$. By sampling $\mathbf{r}$ independently of $\mathbf{R}$, and choosing $\mathbf{R}$ uniformly on SO(3), the resulting prior $p(\mathbf{w}^\ell)$ is SO(3)-invariant. In practice, we take $r\sim\operatorname{Normal}(\mu,\sigma^2)$ to ensure positivity, and $\mathbf{R}\sim \operatorname{Uniform}(\text{SO(3)})$.

 Next, we apply tensor expansion, which maps a rank-$\ell$ irrep vector $\mathbf{w}^{(\ell)}\in \mathbb R^{(2\ell+1)}$ into a matrix of shape $(2\ell_1+1)\times(2\ell_2+1)$, indexed by the $(m_1,m_2)$ satisfying $-\ell_1 \le m_1 \le \ell_1$ and $-\ell_2 \le m_2\le\ell_2$, respectively. Each entry of the resulting matrix is defined as follows:
\begin{equation}
    \left(\bar{\otimes} \mathbf{w}^{(\ell)}  \right)^{(\ell_1,\ell_2)}_{(m_1,m_2)}=\sum^{\ell}_{m=-\ell}C_{(\ell_1,m_1),(\ell_2,m_2)}^{(\ell,m)}w^{(\ell)}_{m},
    \label{eq:tensor_expansion}
\end{equation}
where $C$ denotes Clebsch-Gordan coefficients, $\bar{\otimes}$ denotes the tensor expansion operation. Note that the superscript $(\ell_1,\ell_2)$ indicates the output irrep structure and can be omitted when clear from context. The rotation of this expanded matrix is represented by the Wigner D-matrix as follows:
\begin{equation}
\bigl( \bar{\otimes} \mathbf{w}^{(\ell)} \bigr)
\xrightarrow{\mathbf{R}}
D^{(\ell_1)}(\mathbf{R})
\bigl( \bar{\otimes} \mathbf{w}^{(\ell)} \bigr)
D^{(\ell_2)}(\mathbf{R})^{-1}.
    \label{eq:tensor_expansion_rot}
\end{equation}
See \cref{app:proof_tensor_expansion} for proof. This property allows us to construct SO(3)-invariant distributions over Hamiltonians. We formalize this in the following theorem:
\begin{theorem} 
Let ${\mathbf{H}=\bigl(\bar{\otimes}\mathbf{w}^{(\ell)}\bigr)^{(\ell_1,\ell_2)}}$, where an irrep vector $\mathbf{w}^{(\ell)}\sim p(\mathbf{w}^{(\ell)})$ is drawn from a SO(3)-invariant distribution. Then the induced distribution over $\mathbf{H}$ is invariant under SO(3) transformation:
\begin{equation}
    p(\mathbf H)=
    p(D^{(\ell_1)}(\mathbf R)
    \mathbf{H}
    D^{(\ell_2)}(\mathbf R)^{-1}),\qquad \forall\mathbf R \in \text{SO}(3).
\end{equation}
\end{theorem}

We provide proof in \cref{app:proof_tensor_invariance}. Using the expansion, we can model the invariant distributions for each sub-matrix of Hamiltonian $\mathbf{H}$. We further extend this construction to build global invariant distributions over full Hamiltonian matrices $\mathbf{H}$ by composing multiple high-order irrep vector via tensor expansion. We provide a detailed construction of this multi-block formulation in \cref{app:proof_tensor_expansion_multi}.

\subsection{Model implementation}
\label{app:model_implementation}

We construct \QHFlow{} by extending QHNet~\cite{yu2023efficient}, an SE(3)‑equivariant GNN for Hamiltonian prediction. Our architecture introduces time conditioning and two additional inputs: the current Hamiltonian $\mathbf{H}_{t}$ and the overlap matrix $\mathbf{S}$.  
The model takes $(\mathcal{M},\mathbf{H}_{t},\mathbf{S},t)$ and predicts the target Hamiltonian $\mathbf{H}^\theta_1$ as described in \cref{eq:CFM-ours}.  We provided the implementation details in \cref{app:model_implementation}.

\textbf{Feature intialization.} We first construct the atom-wise features $\mathbf{h}_{i}, \mathbf{s}_{i}$ based on (1) extracting atom-wise submatrices $\mathbf{H}_{i}, \mathbf{S}_{i}$ from  $\mathbf{H}_{t}, \mathbf{S}$ and (2) mapping the submatrices into SO(3) irrep vectors based on Wigner-Eckart projections~\cite{wigner1993matrices}, i.e., set 
$\mathbf{h}_i = \operatorname{\texttt{ProjBlock}}\left(\mathbf{H}_{i}\right), \mathbf{s}_i=\operatorname{\texttt{ProjBlock}}\left(\mathbf{S}_{i}\right)$ where $\texttt{ProjBlock}$ flattens and applies change of basis transformations to the input matrix. We further encode time $t$ through tensor field network (TFN) \cite{thomas2018tensor} layer and sinusoidal encoding $e_{t}=f_\text{time}(t)$, i.e., set $\bm{m}_i=\texttt{TFN}\left(\mathbf{x}_i,\mathbf{h}_i,e_t\right)$.

\textbf{Message-passing layers.}  
To propagate information between neighbors, our model updates the irrep vectors $\mathbf{h}_i$ and $\mathbf{s}_i$ using SO(3)-equivariant attention-based layers adapted from Equiformer~\cite{liao2022equiformer}:
\begin{align*}
    \mathbf{h}_i\leftarrow \operatorname{\texttt{EquiBlock}}\Bigl(\mathbf{h}_i, \bigl\{(\mathbf{h}_j,d_{ij})\bigr\}_{j\in \mathcal{N}_i}, e_t \Bigr),\quad
    \mathbf s_i\leftarrow \operatorname{\texttt{EquiBlock}}\Bigl(\mathbf{s}_i, \bigl\{(\mathbf{s}_j,d_{ij})\bigr\}_{j\in \mathcal{N}_i}, e_t \Bigr),
\end{align*}
where $\mathcal{N}_i$ denotes the neighbors of atom $i$ and $d_{ij}$ is distance between atom $i$ and $j$. We then apply a channel mixing module, \texttt{Mix}, which linearly combines the set of irrep vectors by flattening and reordering them according to their corresponding irrep indices while preserving SE(3)-equivariance. This module update the $\mathbf{m_i}$ in the residual manner:
\begin{equation}
    \bm{m}_i\leftarrow \mathtt{TFN}\Bigl(\bm{m}_{i}+ \operatorname{\texttt{Mix}}(\mathbf{h}_i,\mathbf{s}_i,\bm{m}_i), \bigl\{(\bm{m}_j,d_{ij})\bigr\}_{j\in\mathcal{N}_i},e_{t}\Bigr).
\end{equation}
This update process is repeated for a fixed number of iterations, allowing the model to integrate geometric and physical information across the molecular graph.

\textbf{Hamiltonian reconstruction.}
The atom-wise irrep vectors $\bm{m}_i$ are passed into two TFN modules to predict Hamiltonian components. The first $\mathtt{TFN}_{\text{s}}$ computes atom-wise irreps $\mathbf{w}_{ii}$ using messages from neighboring atoms, while the next $\mathtt{TFN}_{\text{p}}$ predicts pairwise irreps $\mathbf{w}_{ij}$ between atom $i$ and $j$:
\begin{equation}
    \mathbf{w}_{ii} =\mathtt{TFN}_{\text{s}}\bigl(\bm{m}_i, \{(\bm{m}_k,d_{ik})\}_{k\in \mathcal{N}_i} \bigr), \quad \mathbf{w}_{ij} =\mathtt{TFN}_{\text{p}}\bigl(\bm{m}_i,\bm{m}_j,d_{ij}\bigr).
\end{equation}
Each output consists of a set of irrep vectors, $\mathbf{w}_{ii}=\{\mathbf{w}_{ii}^{(\ell)}\}_{\ell \in L_i}$ and $\mathbf{w}_{ij}=\{\mathbf{w}_{ij}^{(\ell)}\}_{\ell \in L_i}$, where $L_i$ is the set of angular momentum $\ell$ corresponding to the atom $i$. Then Hamiltonian blocks are constructed via tensor expansion $\bar{\otimes}$ and learnable weights $F$:
\begin{align}
\mathbf{H}_{ij}^{(\ell_1,\ell_2)}=\sum_{\ell \in L_i}F_{ij}^{(\ell_1,\ell_2,\ell)} \left(\bar{\otimes}{\mathbf{w}^{(\ell)}_{ij}}\right)^{(\ell_1,\ell_2)},
\end{align}
where $\smash{\ell_1 \in L_i}$ and $\smash{\ell_2 \in L_j}$, and the case $i=j$ corresponds to diagonal block. These blocks are then assembled into the full Hamiltonian matrix $\hat{\mathbf{H}}$, which is structured into $K \times K$ sub-matrices corresponding to all pairwise combinations of the $K$ groups of basis functions. All operations in this reconstruction preserve SE(3)-equivariance, ensuring that both $\hat{\mathbf{H}}$ and the learned vector field $v^{\theta}_{t}$ remain equivariant under any SE(3) transformation of the molecular geometry.

==> 4_method_old_0113.tex <==
\section{Method}

We introduce QHFlow-v2, a generative framework for predicting converged Kohn-Sham Hamiltonians $\mathbf{H}$ directly from molecular configurations $\mathcal{M}=(\mathbf{X}, \mathbf{Z})$, where $N$ is the number of atoms, $\mathbf{X} \in \mathbb{R}^{N \times 3}$ denotes atomic coordinates, and $\mathbf{Z} \in \mathbb{N}^{N}$ denotes atomic numbers. our model outputs the Hamiltonian matrix $\mathbf{H}$ expressed in a fixed atomic orbital basis. Our model is built upon two core components: (1) a hybrid equivariant architecture that efficiently extracts node features via scalable SO(2) convolutions and subsequently lifts them to form a rigorous SO(3) pair representation, and (2) an equivariant conditional flow matching objective designed to model the complex joint distribution of ground-state Hamiltonians. We describe each component in detail below.

\subsection{Hybrid SO(2)-SO(3) Equivariant Architecture}

Unlike the MLIPS, where predictions are made nodewise, learning Hamiltonian matrices requires the model to make predictions for both nodes (intra-atomic orbital interactions) and directed edges (inter-atomic orbital interactions). We adopt a hybrid equivariant architecture in which SO(2)-equivariant convolutions are used to encode node-level chemical information, while SO(2)-SO(3) hybrid layers are used to construct pairwise representations that capture the detailed geometric interactions required for Hamiltonian prediction. 

\paragraph{Node Embedding via SO(2) Convolutions.}

Our node embedding layer is based on the eSEN. Since our model is flow matching conditioned on the current Hamiltonian $H_t$, our model takes input as $(\mathcal{M}, H_t)$, we build a displacement vector $\mathbf{r}_{ij}\in \mathbb R^3$ with $i,j=1,\ldots,N$. We initialize node and edge embeddings $z_{ij}$ as follows:
\begin{equation}
    z_{ij}=f^{(0)}(Z_i,\mathbf r_{ij}).
\end{equation}
Our architecture begins by representing the molecular structure as a geometric graph where nodes correspond to atoms and edges connect atom pairs. We initialize the feature of each node $i$ using a learnable atomic embedding based on its nuclear charge $Z_i$:\begin{equation}\mathbf{h}i^{(0)} = f{\text{atom}}(Z_i).\end{equation}These embeddings are iteratively refined through $L$ layers of an SO(2)-equivariant message-passing network, inspired by the efficient eSEN architecture. At each layer $k$, the node feature $\mathbf{h}_i^{(k)}$ is updated by aggregating messages from its local neighborhood $\mathcal{N}(i)$:
\begin{equation}
\mathbf{h}i^{(k+1)} = \phi^{(k)}\left( \mathbf{h}_i^{(k)}, \sum_{j\in\mathcal{N}(i)} \psi^{(k)}_{\text{SO(2)}}\left(\mathbf{h}j^{(k)}, r_{ij}\right) \right),
\end{equation}
where $r_{ij}=\|\mathbf{X}_i-\mathbf{X}_j\|$ is the interatomic distance, and $\phi^{(k)}$ and $\psi^{(k)}_{\text{SO(2)}}$ denote learnable SO(2)-equivariant update and message functions, respectively. Crucially, this module treats features as complex-valued phasors, encoding angular correlations through phase interactions under SO(2) symmetry. This formulation avoids the computationally expensive tensor products required for full SO(3) equivariance, thereby substantially reducing the computational cost while preserving sufficient expressivity to model local chemical environments. The final output after $L$ layers, denoted as $\mathbf{h}_i^{\text{SO(2)}} := \mathbf{h}_i^{(L)}$, serves as a compact representation of the local chemical context and many-body interactions.

\paragraph{Hybrid Edge Feature Construction.}
Hamiltonian matrix elements must transform equivariantly under three-dimensional rotations.
To this end, we construct edge features that combine chemical information extracted by the SO(2)-equivariant backbone with explicit geometric structure.

First, node embeddings $\mathbf{h}_i^{\text{SO(2)}}$ are projected into SO(3) irreducible representations to obtain rotationally equivariant node features,
\begin{equation}
\mathbf{h}_i^{\text{SO(3)}} = \mathcal{P}\!\left(\mathbf{h}_i^{\text{SO(2)}}\right),
\end{equation}
where $\mathcal{P}$ denotes a learnable linear projection into SO(3) irreps.

Using these node features, we construct initial SO(3)-equivariant edge features by combining pairwise node interactions with spherical harmonics that encode relative orientation,
\begin{equation}
\mathbf{e}_{ij}^{\text{SO(3)}} =
\mathbf{h}_i^{\text{SO(3)}} \otimes
\mathbf{h}_j^{\text{SO(3)}} \otimes
Y(\hat{\mathbf{r}}_{ij}),
\end{equation}
where $\hat{\mathbf{r}}_{ij}=(\mathbf{X}_i-\mathbf{X}_j)/r_{ij}$.

In parallel, the SO(2)-equivariant backbone produces edge features $\mathbf{e}_{ij}^{\text{SO(2)}}$ that encode distance-dependent interaction strengths and chemical compatibility.
We combine chemical and geometric information by modulating the SO(3)-equivariant edge features with the SO(2) edge features,
\begin{equation}
\mathbf{m}_{ij} =
\mathbf{e}_{ij}^{\text{SO(2)}} \otimes
\mathbf{e}_{ij}^{\text{SO(3)}}.
\end{equation}
This hybrid construction preserves rotational equivariance while allowing chemically informed features to influence geometrically structured orbital interactions.

\paragraph{Ablation of Hybrid Edge Features.}
Table~\ref{tab:ablation_equivariant_arch} compares SO(2)-only, SO(3)-only, and hybrid SO(2)--SO(3) variants of the proposed architecture.
The SO(2)-only model achieves relatively low mean absolute error (MAE) on Hamiltonian elements, particularly for diagonal blocks, but exhibits large RMSE and severe degradation in orbital energy accuracy.
In contrast, the SO(3)-only model provides improved orbital energy fidelity but yields higher Hamiltonian errors overall.
The hybrid SO(2)--SO(3) architecture combines the strengths of both approaches, achieving the lowest overall Hamiltonian error, substantially improved off-diagonal accuracy, and stable orbital energy predictions.
Notably, the diagonal Hamiltonian error of the hybrid model remains comparable to that of the SO(2)-only variant, while the off-diagonal error is significantly reduced.

\input{table/hybrid}

\paragraph{Equivariant Tensor Expansion for Hamiltonian Construction.}

The edge features $\mathbf{m}_{ij}$ are mapped to Hamiltonian matrix blocks using an equivariant tensor expansion, following the formulation of QHNet. The Kohn-Sham Hamiltonian is expressed in an atomic orbital basis, where each block $\mathbf{H}_{ij}$ corresponds to interactions between orbitals centered on atoms $i$ and $j$.

Let $l_1$ and $l_2$ denote the angular momenta of the interacting orbitals.
The corresponding block $\mathbf{H}_{ij}^{(l_1,l_2)}$ transforms according to irreducible representations of degrees
$l \in \{|l_1-l_2|,\ldots,l_1+l_2\}$.
We reconstruct each block as
\begin{equation}
\mathbf{H}_{ij}^{(l_1,l_2)} =
\sum_{l=|l_1-l_2|}^{l_1+l_2}
F_{ij}^{(l_1,l_2,l)} \cdot \mathbf{w}_{ij}^{(l)},
\end{equation}
where $\mathbf{w}_{ij}^{(l)}$ denotes the degree-$l$ component of $\mathbf{m}_{ij}$ and $F_{ij}^{(l_1,l_2,l)}$ are learnable coefficients.
This construction is consistent with the Wigner--Eckart theorem and guarantees rotational equivariance of the predicted Hamiltonian.

\subsection{Equivariant Flow Matching}

We train QHFlow-v2 using conditional flow matching to model the distribution of converged ground-state Hamiltonians.
We define a time-dependent vector field $v_t(\mathbf{H}_t \mid \mathcal{M})$ that transports a Hamiltonian sample $\mathbf{H}_t$ along a continuous path parameterized by $t\in[0,1]$.

The path is defined by linear interpolation between a noise sample $\mathbf{H}_0\sim\mathcal{N}(0,\mathbf{I})$ and the ground-truth Hamiltonian $\mathbf{H}_1$,
\begin{equation}
\mathbf{H}_t = (1-t)\mathbf{H}_0 + t\mathbf{H}_1,
\qquad
u_t(\mathbf{H}_t \mid \mathbf{H}_1)=\mathbf{H}_1-\mathbf{H}_0.
\end{equation}
The model is trained by minimizing
\begin{equation}
\mathcal{L}_{\text{CFM}} =
\mathbb{E}_{t,\mathbf{H}_0,\mathbf{H}_1}
\left[
\left\|
v_t^\theta(\mathbf{H}_t,\mathcal{M})-(\mathbf{H}_1-\mathbf{H}_0)
\right\|^2
\right].
\end{equation}
This flow-based formulation captures correlations among Hamiltonian matrix elements that are difficult to model with pointwise regression and is essential for stable SCF-free electronic structure calculations.


==> 5_experiment.tex <==
% \input{table/md17_trans}
% \input{table/md17_EF_qhflow}
% \input{table/md17}
\input{table/md17_tc}
\input{table/md17_md}

% \input{table/md17_EF}
\input{table/qh9_main_old}

\input{table/qh9_EF}

\input{table/qh9_no_init}

==> fig/Figure2.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
  \vspace{-12pt}
  \includegraphics[width=\linewidth]{fig/Figure2-4.pdf}
  \captionof{figure}{\textbf{Illustration of the Hamiltonian matrix structure of \ce{H2O}.} Rows and columns are indexed by quantum and angular momentum numbers (\textit{i.e.}, $1s$, $2s$) ordered by atom (\ce{O}, \ce{H}, \ce{H}). The full matrix (right) is partitioned into atomic blocks with gray dashed line; the top-left $9 \times 9$ sub-matrix corresponds to \ce{O} and is shown in detail (left), grouped by quantum and angular momentum. Colors indicate the sign and magnitude of matrix elements.}
  \label{fig:Ham_structure}
  \vspace{-15pt}
\end{wrapfigure}

==> fig/scf_time.tex <==
\begin{minipage}[t]{0.68\textwidth}
    \centering
    \vspace{-10pt}
    \includegraphics[width=1.0\linewidth]{fig/scf_timing_ratios.pdf}
    \captionof{figure}{Results of SCF time on 300 samples from QH9 test dataset.}
    \label{fig:scf_time}
\end{minipage}


==> table/0_md17_EF_sub2.tex <==
\begin{table}[t]
\centering
\caption{\textbf{MLIP vs. QHFlow2 comparison.}
Energy and force errors are reported in meV and meV/\AA.
Molecules Eta., Malon., and Ura. belong to MD17, while SA, Naph., and Asp. belong to rMD17. Best results are shown in \textbf{bold}, and second best are \underline{underlined}.}
\label{tab:md17_rmd17_mlip_vs_qhflowv2_final}
\setlength{\tabcolsep}{2.6pt}
\renewcommand{\arraystretch}{1.06}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l cc cccc cc cccc}
\toprule

& \multicolumn{6}{c}{\textbf{MD17}}
& \multicolumn{6}{c}{\textbf{rMD17}} \\
\cmidrule(lr){2-7}\cmidrule(lr){8-13}

& \multicolumn{2}{c}{Eta.} & \multicolumn{2}{c}{Malon.} & \multicolumn{2}{c}{Ura.}
& \multicolumn{2}{c}{SA}   & \multicolumn{2}{c}{Naph.}  & \multicolumn{2}{c}{Asp.} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}
\textbf{Model}
& E$\downarrow$ & F$\downarrow$
& E$\downarrow$ & F$\downarrow$
& E$\downarrow$ & F$\downarrow$
& E$\downarrow$ & F$\downarrow$
& E$\downarrow$ & F$\downarrow$
& E$\downarrow$ & F$\downarrow$ \\
\cmidrule(r){1-1}\cmidrule(lr){2-7}\cmidrule(lr){8-13}
\multicolumn{13}{l}{\emph{MLIP}\vspace{0.02in}} \\
\ptz NequIP
& 2.21\ptz & 3.08
& 3.29\ptz & 5.59
& 4.51\ptz & 3.29
& 0.70\ptz & 4.00
& 0.20\ptz & 1.30
& 2.30\ptz & 8.20 \\

\ptz ViSNet
& 2.21\ptz & 2.60
& 3.25\ptz & 4.34
& 4.12\ptz & 2.69
& 0.70\ptz & 3.45
& 0.25\ptz & 1.26
& 1.93\ptz & 6.59 \\

\ptz FreeCG
& 2.12\ptz & 2.30
& 4.08\ptz & 4.12
& 4.21\ptz & 2.56
& 1.01\ptz & 2.81
& 0.51\ptz & \textbf{0.99}
& 2.30\ptz & 5.26 \\

\arrayrulecolor{black!40}\midrule
\arrayrulecolor{black}
\multicolumn{13}{l}{\emph{QHFlow2}\vspace{0.02in}} \\

\rowcolor{rowhl}
\ptz\textbf{14M}
& \underline{0.005} & \underline{0.36}
& \underline{0.058} & \underline{0.57}
& \underline{0.234} & \underline{1.01}
& \underline{0.110} & \underline{1.48}
& \underline{0.063} & 1.17
& \underline{0.124} & \underline{1.42} \\

\rowcolor{rowhl}
\ptz\textbf{43M}
& \textbf{0.003} & \textbf{0.34}
& \textbf{0.010} & \textbf{0.51}
& \textbf{0.062} & \textbf{0.90}
& \textbf{0.070} & \textbf{1.38}
& \textbf{0.040} & \underline{1.10}
& \textbf{0.084} & \textbf{1.35} \\

\bottomrule
\end{tabular}
}
\vspace{-15pt}
\end{table}


==> table/0_md17_main_old.tex <==
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.05}
\definecolor{rowhl}{HTML}{EEEAFE}

\begin{table*}[t]
\centering
\caption{\textbf{MD17 benchmark.} Best results are shown in \textbf{bold}.}
\label{tab:md17_results_part1}
\resizebox{0.95\textwidth}{!}{%
\begin{tabular}{l c ccccc ccccc ccccc}
\toprule
& & \multicolumn{5}{c}{Ethanol ($9$ atoms)}
& \multicolumn{5}{c}{malondialdehyde ($9$ atoms)}
& \multicolumn{5}{c}{Uracil ($12$ atoms)} \\
\cmidrule(lr){3-7}\cmidrule(lr){8-12}\cmidrule(lr){13-17}

\textbf{Model}
& \textbf{Param. (M)}
& $H\downarrow$ & $\epsilon_{\mathrm{occ}}\downarrow$ & $S_c\uparrow$ & Energy$\downarrow$ & Force$\downarrow$
& $H\downarrow$ & $\epsilon_{\mathrm{occ}}\downarrow$ & $S_c\uparrow$ & Energy$\downarrow$ & Force$\downarrow$
& $H\downarrow$ & $\epsilon_{\mathrm{occ}}\downarrow$ & $S_c\uparrow$ & Energy$\downarrow$ & Force$\downarrow$ \\
\midrule

\multicolumn{17}{l}{\emph{w/o initial Hamiltonian}\vspace{0.02in}}\\
\ptz\ptz SchNOrb
& \ptz-- 
& 187.4\ptz & 334.4\ptz & \textbf{100.00} & -- & --
& 191.1\ptz & 400.6\ptz & \ptz99.00       & -- & --
& 227.8\ptz & 1760.\ptz & \ptz90.00       & -- & -- \\

\ptz\ptz PhiSNet
& \ptz-- 
& \ptz20.09 & 102.04    & \ptz99.81 & -- & --
& \ptz21.31 & 100.6\ptz & \ptz99.89 & -- & --
& \ptz18.65 & 143.36    & \ptz99.86 & -- & -- \\

\ptz\ptz QHNet
& \ptz-- 
& \ptz27.99 & \ptz99.33 & \ptz99.99 & -- & --
& \ptz29.60 & 100.16    & \ptz99.92 & -- & --
& \ptz26.80 & 127.93    & \ptz99.99 & -- & -- \\

\ptz\ptz HELM
& \ptz-- 
& \ptz\ptz5.79 & -- & -- & 28.93\ptz & --
& \ptz\ptz4.86 & -- & -- & 20.15\ptz & --
& \ptz\ptz3.61 & -- & -- & 22.69\ptz & -- \\

\rowcolor{rowhl}
\ptz\ptz \textbf{QHFlow2-m}
& \ptz43
& \ptz12.49 & \ptz21.32 & \textbf{100.00} & \ptz0.136 & 1.320
& \ptz13.14 & \ptz26.64 & \ptz99.97 & 1.145 & 2.296
& \ptz13.68 & 259.50 & \ptz99.89 & TBA & TBA \\

\arrayrulecolor{black!40}\midrule
\arrayrulecolor{black}

\multicolumn{17}{l}{\emph{w/ initial Hamiltonian}\vspace{0.02in}}\\
\ptz\ptz SPHNet
& \ptz-- 
& \ptz21.02 & \ptz82.30 & \textbf{100.00} & -- & --
& \ptz20.67 & \ptz95.77 & \ptz99.99 & -- & --
& \ptz19.36 & 118.21    & \ptz99.99 & -- & -- \\

\ptz\ptz QHNet
& \ptz-- 
& \ptz\ptz6.57 & \ptz36.53 & \textbf{100.00} & \ptz0.024 & 0.854
& \ptz\ptz4.52 & \ptz23.90 & \ptz99.99       & \ptz0.035 & 1.145
& \ptz\ptz4.71 & \ptz39.85 & \ptz99.97       & \ptz0.139 & 2.139 \\

\ptz\ptz QHFlow
& \ptz-- 
& \ptz\ptz5.60 & \ptz31.16 & \textbf{100.00} & \ptz0.019 & 0.775
& \ptz\ptz4.26 & \ptz23.61 & \ptz99.98       & \ptz0.034 & 1.166
& \ptz\ptz3.99 & \ptz34.31 & \ptz99.99       & \ptz0.106 & 1.869 \\

\rowcolor{rowhl}
\ptz\ptz \textbf{QHFlow2-s}
& \ptz14
& \ptz\ptz3.21 & \ptz14.51 & \textbf{100.00} & \ptz0.005 & 0.355
& \ptz\ptz2.66 & \ptz11.32 & \textbf{100.00} & \ptz0.058 & 0.568
& \ptz\ptz2.52 & \ptz16.91 & \ptz99.99       & \ptz0.234 & 1.012 \\

\rowcolor{rowhl}
\ptz\ptz \textbf{QHFlow2-m}
& \ptz43
& \ptz\ptz\textbf{2.63} & \ptz\textbf{13.56} & \textbf{100.00} & \ptz\textbf{0.003} & \textbf{0.338}
& \ptz\ptz\textbf{2.03} & \ptz\textbf{10.33} & \textbf{100.00} & \ptz\textbf{0.010} & \textbf{0.514}
& \ptz\ptz\textbf{1.85} & \ptz\textbf{15.88} & \textbf{100.00} & \ptz\textbf{0.062} & \textbf{0.901} \\

\bottomrule
\end{tabular}%
}
\end{table*}


==> table/0_rmd17_main.tex <==
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.05}
% \definecolor{rowhl}{HTML}{EEEAFE}
\definecolor{rowhl}{HTML}{DDF1FF}

\begin{table*}[t]
\centering
\caption{\textbf{Revised MD17 benchmark.} Best results are shown in \textbf{bold}.}
\label{tab:md17_results_part2}
\resizebox{0.95\textwidth}{!}{%
\begin{tabular}{l c ccccc ccccc ccccc}
\toprule
& & \multicolumn{5}{c}{Salicylic Acid ($16$ atoms)}
& \multicolumn{5}{c}{Naphthalene ($19$ atoms)}
& \multicolumn{5}{c}{Aspirin ($21$ atoms)} \\
\cmidrule(lr){3-7}\cmidrule(lr){8-12}\cmidrule(lr){13-17}

\textbf{Model}
& \textbf{Param.}
& $H\downarrow$ & $\epsilon_{\mathrm{occ}}\downarrow$ & $S_c\uparrow$ & Energy$\downarrow$ & Force$\downarrow$
& $H\downarrow$ & $\epsilon_{\mathrm{occ}}\downarrow$ & $S_c\uparrow$ & Energy$\downarrow$ & Force$\downarrow$
& $H\downarrow$ & $\epsilon_{\mathrm{occ}}\downarrow$ & $S_c\uparrow$ & Energy$\downarrow$ & Force$\downarrow$ \\
\midrule

% \multicolumn{17}{l}{\emph{w/ initial Hamiltonian}\vspace{0.02in}}\\
\multicolumn{17}{l}{\emph{Regression}}\vspace{0.01in} \\

\ptz\ptz SPHNet
& 18M 
& \ptz\ptz8.17 & \ptz54.72 & \ptz99.82 & 1.337 & 3.264
& \ptz\ptz6.09 & \ptz37.98 & \ptz98.83 & 1.905 & 2.315
& \ptz10.74 &\ptz98.05 & \ptz99.51 & 3.972 & 5.347 \\

\ptz\ptz SPHNet
& 36M 
& \ptz\ptz7.25 & \ptz49.39 & \ptz99.84 & 1.106 & 2.960
& \ptz\ptz5.36 & \ptz36.30 & \ptz98.90 & 1.418 & 2.076
& \ptz\ptz8.87 & \ptz80.98 & \ptz99.61 & 2.773 & 4.456 \\

\ptz\ptz QHNet
& 27M
& \ptz\ptz5.45 & \ptz58.66 & \ptz99.81 & 0.701 & 2.909
& \ptz\ptz3.79 & \ptz40.78 & \ptz98.95 & 0.589 & 1.816
& \ptz\ptz6.42 & \ptz86.92 & \ptz99.61 & 1.828 & 4.239 \\

\arrayrulecolor{black!40}\midrule
\arrayrulecolor{black}
\multicolumn{17}{l}{\emph{Flow-based}}\vspace{0.01in} \\

\ptz\ptz QHFlow
& 30M
& \ptz\ptz4.76 & \ptz54.10 & \ptz99.83 & 0.589 & 2.701
& \ptz\ptz3.22 & \ptz36.07 & \ptz99.04 & 0.335 & 1.610
& \ptz\ptz4.99 & \ptz71.50 & \ptz99.70 & 1.071 & 3.357 \\

\rowcolor{rowhl}
\ptz\ptz \textbf{QHFlow2-s}
& 14M
& \ptz\ptz2.60 & \ptz31.61 & \ptz\textbf{99.91} & 0.110 & 1.482
& \ptz\ptz2.42 & \ptz\textbf{28.30} & \ptz\textbf{99.28}          & 0.063 & 1.171
& \ptz\ptz2.33 & \ptz32.98 & \ptz99.88          & 0.124 & 1.423 \\

\rowcolor{rowhl}
\ptz\ptz \textbf{QHFlow2-m}
& 43M
& \ptz\ptz\textbf{2.05} & \ptz\textbf{30.31} & \ptz\textbf{99.91} & \textbf{0.070} & \textbf{1.381}
& \ptz\ptz\textbf{2.11} & \ptz28.74 & \ptz99.27 & \textbf{0.040} & \textbf{1.106}
& \ptz\ptz\textbf{1.68} & \ptz\textbf{31.14} & \ptz\textbf{99.90} & \textbf{0.084} & \textbf{1.350} \\

\bottomrule
\end{tabular}%
}
\end{table*}

\renewcommand{\thefootnote}{\arabic{footnote}}


==> table/ab_hybrid.tex <==
% \paragraph{Ablation of two-stage edge update.}

% \begin{table}[t]
% \centering
% \caption{
% \textbf{SO(2) ablations over backbone and convolution settings.}
% All variants use the same SO(2) backbone and are trained on QH9Stable-iid with the parameter budget fixed to 43M.
% We vary whether the reference-frame cue $g_{\mathrm{ref}}$ is enabled and the SO(2) edge cutoff, using the values listed in the table (default cutoff: 5\,\AA).
% We report Hamiltonian MAE and its diagonal/off-diagonal components (lower is better).
% }
% \label{tab:so2_ablation}
% \setlength{\tabcolsep}{5pt}
% \renewcommand{\arraystretch}{1.15}
% \begin{tabular}{lcccccccc}
% \toprule
% $g_{\mathrm{ref}}$ &  \cmark &  \xmark &  \xmark &  \xmark &  \xmark &  \cmark &  \cmark &  \cmark \\
% SO(2) edge cutoff (\AA) &  -- &  5 &  8 &  12 &  15 &  5 &  12 &  15 \\
% \midrule
% $H$ MAE $\downarrow$              &  27.91 &  14.91 &  9.58 &  9.36 &  9.86 & \cellcolor{rowhl}  9.14 & \cellcolor{rowhl}  8.55 &  \cellcolor{rowhl} \textbf{8.43} \\
% Diag.\ $H$ MAE $\downarrow$       &  31.37 &  22.89 &  22.06 &  21.79 &  21.11 &  \cellcolor{rowhl} 18.45 & \cellcolor{rowhl}  17.77 & \cellcolor{rowhl}  \textbf{17.30} \\
% Off-diag.\ $H$ MAE $\downarrow$   &  14.35 &  27.64 &  8.63 &  8.41 &  9.00 &\cellcolor{rowhl} 8.47 & \cellcolor{rowhl} 7.84 &  \cellcolor{rowhl}\textbf{7.75} \\
% \bottomrule
% \end{tabular}
% \end{table}

==> table/md17_full.tex <==
\renewcommand{\thefootnote}{\fnsymbol{footnote}}

\begin{table}[h]
\centering
\caption{Experimental results on MD17 dataset.}
\label{tab:md17_results}
\begin{tabular}{lcccccc}
\toprule
&
\multicolumn{3}{c}{Water ($3$ atoms)} & 
\multicolumn{3}{c}{Ethanol ($9$ atoms)} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
& $H$ $\downarrow$ & \OCC $\downarrow$ & \SC $\uparrow$ 
& $H$ $\downarrow$ & \OCC $\downarrow$ & \SC $\uparrow$ \\
\multirow{-2}{*}{\textbf{Model}}&  [$10^{-6}E_h$]  & [$10^{-6}E_h$]  &  [$10^{-2}$]  &  [$10^{-6}E_h$]  & [$10^{-6}E_h$]  &  [$10^{-2}$]\\
\midrule
\midrule
% \rowcolor{Gray}\texttt{minao}\tablefootnote{\texttt{minao} denotes the error inherent to conventional methods—it is defined as the discrepancy between the ground truth of dataset and the value computed by the \texttt{pyscf} method when the density is initialized using \texttt{minao}.}
% & \ptz2.51   & 14.99    & 100.00
%     & \ptz1.13   & 10.90    & 100.00 \\

SchNOrb  & 165.4  & 279.3    & \textbf{100.00}
& 187.4  & 334.4   & \textbf{100.00} \\

PhiSNet  & 15.67  & \ptz85.53   & \textbf{100.00}
& 20.09  & 102.04  & \ptz99.81\\
% & QHNet    & 10.79  & \ptz33.76   & \ptz99.99 & - & - \\
QHNet\tablefootnote[1]{We use our re-trained version of QHNet, based on the publicly available implementation.}& 11.70  & \ptz26.06   & \textbf{100.00}
&  27.99  & \ptz99.33   & \ptz99.99 \\

SPHNet   & 23.18  & 182.29  & \textbf{100.00}
&  21.02  & \ptz82.30   & \textbf{100.00} \\
% \rowcolor{lightorange}\cellcolor{white} & \textbf{Ours (1 step)}     & \ptz4.96   & \ptz19.49  & \textbf{100.00} & 32.17 & 55.95 \\
\rowcolor{lightorange}
\textbf{Ours}   & \ptz\textbf{4.93}   & \ptz\textbf{19.29}  & \textbf{100.00}
& \ptz\textbf{5.33}  & \ptz\textbf{29.03}   & \textbf{100.00} \\

\midrule
&
\multicolumn{3}{c}{malondialdehyde ($9$ atoms)} & 
\multicolumn{3}{c}{Uracil ($12$ atoms)} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
\multirow{-2}{*}{\textbf{Model}}
& $H$ $\downarrow$ & \OCC $\downarrow$ & \SC $\uparrow$ 
& $H$ $\downarrow$ & \OCC $\downarrow$ & \SC $\uparrow$ \\
\midrule
\midrule

% \rowcolor{Gray}
% \texttt{minao}    & \ptz1.13   & 13.70    & 100.00 
%    & \ptz0.72   & 12.71    & 100.00\\

SchNOrb  & 191.1  & 400.6   & \ptz99.00
 & 227.8  & 1760    & \ptz90.00\\

PhiSNet  & 21.31  & 100.6   & \ptz99.89
  & 18.65  & 143.36  & \ptz99.86 \\

QHNet$^*$& 29.60  & 100.16   & \ptz99.92 
& 26.80  & 127.93  &  \ptz99.87 \\

SPHNet   & 20.67  & \ptz95.77   & \ptz\textbf{99.99}
  & 19.36  & 118.21      & \ptz\textbf{99.99}  \\


\rowcolor{lightorange}
\textbf{Ours}     & \ptz\textbf{3.80}   & \ptz\textbf{22.68}  & \ptz\textbf{99.99}
  & \ptz\textbf{3.68}   & \ptz\textbf{30.54}  & \ptz\textbf{99.99} \\
\bottomrule
\end{tabular}
\end{table}

\renewcommand{\thefootnote}{\arabic{footnote}}

% 0.54
% 0.72
% 0.81
% 0.79
% --
% 0.71

==> table/md17_md.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Revised MD17 moleucule dynamics benchmark.} Higher Stability indicates better performance, while lower $h(r)$ and Force denote higher accuracy.}
\label{tab:md17_metric_based}
\resizebox{\textwidth}{!}{
\begin{tabular}{llcccccccc|ccc}
\toprule
{Metric} & {Molecule} 
& {DeepPot-SE} & {SchNet} & {DimeNet} & {PaiNN} 
& {SphereNet} & {ForceNet} & {GemNet-dT} & {NequIP} & QHNet & QHFlow & \textbf{eSCFlow} \\
\midrule
\midrule
\multirow{5}{*}{Stability ($\uparrow$)} 
& Ethanol        (9)  & 300 & 247 & 26  & 86  & 33  & 300 & 300 & 300 \\
& Salicylic Acid (16) & 300 & 300 & 73  & 281 & 36 & 1 & 94 & 300 \\
& Naphthalene    (19) & 246 & 18  & 85  & 300  & 6   & 300 & 25  & 300 \\
& Aspirin        (21) & 9   & 26  & 54  & 15  & 141 & 182 & 192 & 300 \\
\arrayrulecolor{gray}
\cmidrule(lr){2-13}
\arrayrulecolor{black}

& Avg. & 213.8 & 147.8 & 60 & 206.5 & 54 & 195.8 & 152.8 & 300 \\
\midrule
\multirow{5}{*}{$h(r)$ ($\downarrow$)} 
& Ethanol        (9)  & 0.09 & 0.21 & 0.15 & 0.15 & 0.13 & 0.86 & 0.09 & 0.08 \\
& Salicylic Acid (16) & 0.03 & 0.03 & 0.06 & 0.03 & 0.06 & 0.35 & 0.07 & 0.03 \\
& Naphthalene    (19) & 0.11 & 0.09 & 0.10 & 0.13 & 0.14 & 1.02 & 0.12 & 0.12 \\
& Aspirin        (21) & 0.65 & 0.36 & 0.04 & 0.04 & 0.03 & 0.56 & 0.04 & 0.02 \\
\arrayrulecolor{gray}
\cmidrule(lr){2-13}
\arrayrulecolor{black}

& Avg. & 0.22 & 0.17 & 0.088 & 0.088 & 0.090 & 0.70 & 0.080 & 0.063 \\
\midrule
\multirow{5}{*}{Force ($\downarrow$)} 
& Ethanol        (9)  & 8.9  & 16.8 & 4.2 & 5.0 & 1.7 & 14.9 & 1.7 & 1.3 & 2.5 & 0.77 & \textbf{0.44}\\
& Salicylic Acid (16) & 14.9 & 26.3 & 9.6 & 6.5 & 2.6 & 12.8 & 4.0 & 1.6 \\
& Naphthalene    (19) & 13.4 & 22.5 & 5.7 & 3.8 & 1.5 & 9.9 & 1.9 & 1.1 \\
& Aspirin        (21) & 21.0 & 35.6 & 10.0 & 9.2 & 3.4 & 22.1 & 5.1 & 2.3 \\
\arrayrulecolor{gray}
\cmidrule(lr){2-13}
\arrayrulecolor{black}
& Avg. & 14.6 & 25.3 & 7.4 & 6.1 & 2.3 & 15.0 & 3.2 & 1.6 \\
\bottomrule
\end{tabular}
}
\end{table}


==> table/md17_rmd17_main_old.tex <==
\renewcommand{\thefootnote}{\fnsymbol{footnote}}

\begin{table*}[t]
\centering
\captionof{table}{\textbf{MD17/rMD17 benchmark.} Results shown in \textbf{bold} denote the best result in each column}
\label{tab:md17_results}
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{lcccccccccccccccc}
\toprule
&\multicolumn{5}{c}{Ethanol ($9$ atoms)}
&\multicolumn{5}{c}{Malondialdehyde ($9$ atoms)}
&\multicolumn{5}{c}{Uracil ($12$ atoms)} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-11} \cmidrule(lr){12-16}
& $H$ $\downarrow$ & \OCC $\downarrow$ & \SC $\uparrow$ & Energy $\downarrow$ & Force $\downarrow$
& $H$ $\downarrow$ & \OCC $\downarrow$ & \SC $\uparrow$ & Energy $\downarrow$ & Force $\downarrow$
& $H$ $\downarrow$ & \OCC $\downarrow$ & \SC $\uparrow$ & Energy $\downarrow$ & Force $\downarrow$ \\

\multirow{-2}{*}{\textbf{Model}}
& [$\mu E_h$] & [$\mu E_h$] & [$\%$] & [meV] & [meV/\AA]
& [$\mu E_h$] & [$\mu E_h$] & [$\%$] & [meV] & [meV/\AA]
& [$\mu E_h$] & [$\mu E_h$] & [$\%$] & [meV] & [meV/\AA] \\

\midrule
\midrule

SchNOrb 
& 187.4 & 334.4     & \textbf{100.00} & – & –
& 191.1 & 400.6\ptz & 99.00           & – & –
& 227.8 & 1760.     & 90.00           & – & – \\

PhiSNet
& {20.09} & 102.04     & \ptz99.81 & – & –
& 21.31   & 100.6\ptz  & 99.89    & – & –
& {18.65} & 143.36     & 99.86     & – & – \\

% QHNet (w/o init)
% & 23.27 & \ptz97.50  & \ptz{99.99}  & 0.323 & 2.513
% & 29.60 & 100.16 & {99.92} & 0.916 & 4.949
% & 26.80 & 127.93 & {99.87} & 2.351 & 6.798 \\


SPHNet  
& 21.02 & \ptz82.30 & \textbf{100.00} & – & –
& 20.67 & \ptz95.77 & \textbf{99.99}  & – & –
& 19.36 & 118.21    & \textbf{99.99}  & – & – \\

% WANet  
% & – & – & – & – & –
% & – & – & – & – & –
% & – & – & – & – & – \\

QHNet (w/ init)
& \ptz6.78 & \ptz36.45  & \textbf{100.00}  & – & –
& \ptz4.58 & \ptz25.10 & {99.98}           & – & –
& \ptz4.80 & \ptz40.43 & {99.97}           & – & – \\

QHFlow (w/ init)
& \ptz5.60 & \ptz31.19 & \textbf{100.00} & 0.019 & 0.775
& \ptz3.80 & \ptz22.68 & \textbf{99.99}  & 0.035 & 1.187
& \ptz3.99 & \ptz34.31 & \textbf{99.99}  & 0.106 & 1.869 \\

\arrayrulecolor{gray}
\cmidrule(lr){1-16}
\arrayrulecolor{black}

% UMA  w/o FT (MLFF)
% & – & – & – & 8194 & 334
% & – & – & – & 13166 & 487
% & – & – & – & 21212 & 367 \\

Equiformer (MLFF)
& – & – & – & 2.2\ptz\ptz & 2.9\ptz\ptz
& – & – & – & 3.2\ptz\ptz & 5.4\ptz\ptz
& – & – & – & 4.3\ptz\ptz & 3.3\ptz\ptz \\

% SchNet (MLFF)
% & – & – & – & – & –
% & – & – & – & – & –
% & – & – & – & – & – \\

% DimeNet (MLFF)
% & – & – & – & – & –
% & – & – & – & – & –
% & – & – & – & – & – \\

% Nequip (MLFF)
% & – & – & – & – & –
% & – & – & – & – & –
% & – & – & – & – & – \\

% eSEN (MLFF)
% & – & – & – & – & –
% & – & – & – & – & –
% & – & – & – & – & – \\



\arrayrulecolor{gray}
\cmidrule(lr){1-16}
\arrayrulecolor{black}

% \textbf{eSCFlow}-11M
% & {-} & {-} & {-} & {-} & {-}
% & {-} & {-} & {-} & {-} & {-}
% & {-} & {-} & {-} & {-} & {-} \\

% \textbf{eSCFlow}-14M
% & {-} & {-} & {-} & {-} & {-}
% & {-} & {-} & {-} & {-} & {-}
% & {-} & {-} & {-} & {-} & {-} \\


\textbf{eSCFlow}-14M
& \ptz3.87 & \ptz18.55 & \textbf{100.00} & – & –
& \ptz3.29 & \ptz19.63 & 99.97 & – & –
& \ptz3.00 & \ptz21.16 & \textbf{99.99} & 0.119 & \textbf{1.207} \\

\textbf{eSCFlow}-43M
& \ptz\textbf{3.39} & \ptz\textbf{18.40} & \textbf{100.00} & \textbf{0.007} & \textbf{0.443}
& \ptz\textbf{2.67} & \ptz\textbf{15.13} & \textbf{99.99}  & \textbf{0.014} & \textbf{0.728}
& \ptz\textbf{2.37} & \ptz\textbf{21.59} & \textbf{99.99}  & \textbf{0.097} & {1.248} \\

% \textbf{eSCFlow}-183M
% & {-} & {-} & {-} & {-} & {-}
% & {-} & {-} & {-} & {-} & {-}
% & {-} & {-} & {-} & {-} & {-} \\

\midrule
\midrule

&\multicolumn{5}{c}{Salicylic Acid ($16$ atoms)}
&\multicolumn{5}{c}{Naphthalene ($19$ atoms)}
&\multicolumn{5}{c}{Aspirin ($21$ atoms)} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-11} \cmidrule(lr){12-16}
& $H$ $\downarrow$ & \OCC $\downarrow$ & \SC $\uparrow$ & Energy $\downarrow$ & Force $\downarrow$
& $H$ $\downarrow$ & \OCC $\downarrow$ & \SC $\uparrow$ & Energy $\downarrow$ & Force $\downarrow$
& $H$ $\downarrow$ & \OCC $\downarrow$ & \SC $\uparrow$ & Energy $\downarrow$ & Force $\downarrow$ \\

\multirow{-2}{*}{\textbf{Model}}
& [$\mu E_h$] & [$\mu E_h$] & [$\%$] & [meV] & [meV/\AA]
& [$\mu E_h$] & [$\mu E_h$] & [$\%$] & [meV] & [meV/\AA]
& [$\mu E_h$] & [$\mu E_h$] & [$\%$] & [meV] & [meV/\AA] \\

\midrule
\midrule

% SchNOrb 
% & – & – & – & – & –
% & – & – & – & – & –
% & – & – & – & – & – \\

% PhiSNet
% & – & – & – & – & –
% & – & – & – & – & –
% & – & – & – & – & – \\

QHNet (w/ init)
& 4.34 & 48.76 & 99.85 & – & –
& 3.23 & 37.45 & 99.00 & – & –
& 5.05 & 69.98 & 99.70 & – & – \\

SPHNet (w/ init)
& – & – & – & – & –
& – & – & – & – & –
& – & – & – & – & – \\

\RC
QHFlow (w/ init)
& – & – & – & – & –
& 3.01 & 35.39 & 99.05 & – & –
& – & – & – & – & – \\

\arrayrulecolor{gray}
\cmidrule(lr){1-16}
\arrayrulecolor{black}

% UMA  w/o FT(MLFF)
% & – & – & – & – & –
% & – & – & – & – & –
% & – & – & – & – & – \\

% SchNet (MLFF)
% & – & – & – & 384.8 & 19.8
% & – & – & – & 567.2 & 15.8
% & – & – & – & 162.1 & 36.6 \\

% DimeNet (MLFF)
% & – & – & – & 295.5\ptz\ptz & 16.9\ptz\ptz
% & – & – & – & 825.9\ptz\ptz & 5.9\ptz\ptz
% & – & – & – & 54.9\ptz\ptz & 7.1\ptz\ptz \\

EquiformerV2 (MLFF)
& – & – & – & – & –
& – & – & – & \ptz4.7\ptz\ptz & \ptz4.9\ptz\ptz
& – & – & – & 12.1\ptz\ptz & 11.0\ptz\ptz \\

NequIP (MLFF)
& – & – & – & \ptz2.05\ptz & \ptz1.98\ptz
& – & – & – & \ptz1.69\ptz & \ptz0.98\ptz
& – & – & – & \ptz2.50\ptz & \ptz1.96\ptz \\

% eSEN (MLFF)
% & – & – & – & 37.1 & 18.5
% & – & – & – & \ptz95.7 & 11.8
% & – & – & – & \ptz60.0 & 17.2 \\

\arrayrulecolor{gray}
\cmidrule(lr){1-16}
\arrayrulecolor{black}

\textbf{eSCFlow}-14M
& {2.95} & {35.40} & \textbf{99.90} & \ptz0.148 & \ptz1.652
& {2.59} & {30.55} & {99.18} & \ptz0.077 & \ptz1.257
& 2.63 & 39.14 & 99.86 & \ptz0.170 & \ptz1.670 \\

\textbf{eSCFlow}-43M
& \textbf{2.37} & \textbf{34.24} & \textbf{99.90} & \ptz\textbf{0.108} & \ptz\textbf{1.563}
& \textbf{2.14} & \textbf{29.15} & \textbf{99.25} & \ptz\textbf{0.052} & \ptz\textbf{1.173}
& \textbf{2.03} & \textbf{37.58} & \textbf{99.87} & \ptz\textbf{0.136} & \ptz\textbf{1.630} \\

\bottomrule
\end{tabular}
    }
\vspace{-10pt}
\end{table*}

\renewcommand{\thefootnote}{\arabic{footnote}}



==> table/md17_tc.tex <==
\renewcommand{\thefootnote}{\fnsymbol{footnote}}

\begin{table}[t]
\centering
\captionof{table}{\textbf{MD17 benchmark.} Results shown in \textbf{bold} denote the best result in each column, whereas those that are \underline{underlined} indicate the second best.}
\label{tab:md17_results}
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{lcccccccccccccccc}
\toprule
&\multicolumn{5}{c}{Ethanol ($9$ atoms)}
&\multicolumn{5}{c}{Malondialdehyde ($9$ atoms)}
&\multicolumn{5}{c}{Uracil ($12$ atoms)} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-11} \cmidrule(lr){12-16}
& $H$ $\downarrow$ & \OCC $\downarrow$ & \SC $\uparrow$ & Energy $\downarrow$ & Force $\downarrow$
& $H$ $\downarrow$ & \OCC $\downarrow$ & \SC $\uparrow$ & Energy $\downarrow$ & Force $\downarrow$
& $H$ $\downarrow$ & \OCC $\downarrow$ & \SC $\uparrow$ & Energy $\downarrow$ & Force $\downarrow$ \\

\multirow{-2}{*}{\textbf{Model}}
& [$\mu E_h$] & [$\mu E_h$] & [$\%$] & [meV] & [meV/\AA]
& [$\mu E_h$] & [$\mu E_h$] & [$\%$] & [meV] & [meV/\AA]
& [$\mu E_h$] & [$\mu E_h$] & [$\%$] & [meV] & [meV/\AA] \\

\midrule
\midrule

SchNOrb 
& 187.4 & 334.4     & \textbf{100.00} & – & –
& 191.1 & 400.6\ptz & 99.00           & – & –
& 227.8 & 1760.     & 90.00           & – & – \\

PhiSNet
& {20.09} & 102.04     & \ptz99.81 & – & –
& 21.31   & 100.6\ptz  & 99.89    & – & –
& {18.65} & 143.36     & 99.86     & – & – \\

QHNet (w/o init)
& 23.27 & \ptz97.50  & \ptz{99.99}  & 0.323 & 2.513
& 29.60 & 100.16 & {99.92} & 0.916 & 4.949
& 26.80 & 127.93 & {99.87} & 2.351 & 6.798 \\


SPHNet  
& 21.02 & \ptz82.30 & \textbf{100.00} & – & –
& 20.67 & \ptz95.77 & \textbf{99.99}  & – & –
& 19.36 & 118.21    & \textbf{99.99}  & – & – \\

WANet  
& – & – & – & – & –
& – & – & – & – & –
& – & – & – & – & – \\

QHNet (w/ init)
& \ptz6.78 & \ptz36.45  & \textbf{100.00}  & – & –
& \ptz4.58 & \ptz25.10 & {99.98}           & – & –
& \ptz4.80 & \ptz40.43 & {99.97}           & – & – \\

QHFlow (w/ init)
& \ptz5.60 & \ptz31.19 & \textbf{100.00} & 0.019 & 0.775
& \ptz3.80 & \ptz22.68 & \textbf{99.99}  & 0.035 & 1.187
& \ptz3.99 & \ptz34.31 & \textbf{99.99}  & 0.106 & 1.869 \\

\arrayrulecolor{gray}
\cmidrule(lr){1-16}
\arrayrulecolor{black}

% UMA  w/o FT (MLFF)
% & – & – & – & 8194 & 334
% & – & – & – & 13166 & 487
% & – & – & – & 21212 & 367 \\

Equiformer (MLFF)
& – & – & – & 2.2\ptz\ptz & 2.9\ptz\ptz
& – & – & – & 3.2\ptz\ptz & 5.4\ptz\ptz
& – & – & – & 4.3\ptz\ptz & 3.3\ptz\ptz \\

% SchNet (MLFF)
% & – & – & – & – & –
% & – & – & – & – & –
% & – & – & – & – & – \\

% DimeNet (MLFF)
% & – & – & – & – & –
% & – & – & – & – & –
% & – & – & – & – & – \\

% Nequip (MLFF)
% & – & – & – & – & –
% & – & – & – & – & –
% & – & – & – & – & – \\

% eSEN (MLFF)
% & – & – & – & – & –
% & – & – & – & – & –
% & – & – & – & – & – \\



\arrayrulecolor{gray}
\cmidrule(lr){1-16}
\arrayrulecolor{black}

% \textbf{eSCFlow}-11M
% & {-} & {-} & {-} & {-} & {-}
% & {-} & {-} & {-} & {-} & {-}
% & {-} & {-} & {-} & {-} & {-} \\

% \textbf{eSCFlow}-14M
% & {-} & {-} & {-} & {-} & {-}
% & {-} & {-} & {-} & {-} & {-}
% & {-} & {-} & {-} & {-} & {-} \\


\textbf{eSCFlow}-14M
& \ptz3.87 & \ptz18.55 & \textbf{100.00} & – & –
& \ptz3.29 & \ptz19.63 & 99.97 & – & –
& \ptz3.00 & \ptz21.16 & \textbf{99.99} & 0.119 & \textbf{1.207} \\

\textbf{eSCFlow}-43M
& \ptz\textbf{3.39} & \ptz\textbf{18.40} & \textbf{100.00} & \textbf{0.007} & \textbf{0.443}
& \ptz\textbf{2.67} & \ptz\textbf{15.13} & \textbf{99.99}  & \textbf{0.014} & \textbf{0.728}
& \ptz\textbf{2.37} & \ptz\textbf{21.59} & \textbf{99.99}  & \textbf{0.097} & {1.248} \\

% \textbf{eSCFlow}-183M
% & {-} & {-} & {-} & {-} & {-}
% & {-} & {-} & {-} & {-} & {-}
% & {-} & {-} & {-} & {-} & {-} \\

\midrule
\midrule

&\multicolumn{5}{c}{Salicylic Acid ($16$ atoms)}
&\multicolumn{5}{c}{Naphthalene ($19$ atoms)}
&\multicolumn{5}{c}{Aspirin ($21$ atoms)} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-11} \cmidrule(lr){12-16}
& $H$ $\downarrow$ & \OCC $\downarrow$ & \SC $\uparrow$ & Energy $\downarrow$ & Force $\downarrow$
& $H$ $\downarrow$ & \OCC $\downarrow$ & \SC $\uparrow$ & Energy $\downarrow$ & Force $\downarrow$
& $H$ $\downarrow$ & \OCC $\downarrow$ & \SC $\uparrow$ & Energy $\downarrow$ & Force $\downarrow$ \\

\multirow{-2}{*}{\textbf{Model}}
& [$\mu E_h$] & [$\mu E_h$] & [$\%$] & [meV] & [meV/\AA]
& [$\mu E_h$] & [$\mu E_h$] & [$\%$] & [meV] & [meV/\AA]
& [$\mu E_h$] & [$\mu E_h$] & [$\%$] & [meV] & [meV/\AA] \\

\midrule
\midrule

% SchNOrb 
% & – & – & – & – & –
% & – & – & – & – & –
% & – & – & – & – & – \\

% PhiSNet
% & – & – & – & – & –
% & – & – & – & – & –
% & – & – & – & – & – \\

QHNet (w/ init)
& 4.34 & 48.76 & 99.85 & – & –
& 3.23 & 37.45 & 99.00 & – & –
& 5.05 & 69.98 & 99.70 & – & – \\

SPHNet (w/ init)
& – & – & – & – & –
& – & – & – & – & –
& – & – & – & – & – \\

\RC
QHFlow (w/ init)
& – & – & – & – & –
& 3.01 & 35.39 & 99.05 & – & –
& – & – & – & – & – \\

\arrayrulecolor{gray}
\cmidrule(lr){1-16}
\arrayrulecolor{black}

% UMA  w/o FT(MLFF)
% & – & – & – & – & –
% & – & – & – & – & –
% & – & – & – & – & – \\

% SchNet (MLFF)
% & – & – & – & 384.8 & 19.8
% & – & – & – & 567.2 & 15.8
% & – & – & – & 162.1 & 36.6 \\

% DimeNet (MLFF)
% & – & – & – & 295.5\ptz\ptz & 16.9\ptz\ptz
% & – & – & – & 825.9\ptz\ptz & 5.9\ptz\ptz
% & – & – & – & 54.9\ptz\ptz & 7.1\ptz\ptz \\

EquiformerV2 (MLFF)
& – & – & – & – & –
& – & – & – & \ptz4.7\ptz\ptz & \ptz4.9\ptz\ptz
& – & – & – & 12.1\ptz\ptz & 11.0\ptz\ptz \\

NequIP (MLFF)
& – & – & – & \ptz2.05\ptz & \ptz1.98\ptz
& – & – & – & \ptz1.69\ptz & \ptz0.98\ptz
& – & – & – & \ptz2.50\ptz & \ptz1.96\ptz \\

% eSEN (MLFF)
% & – & – & – & 37.1 & 18.5
% & – & – & – & \ptz95.7 & 11.8
% & – & – & – & \ptz60.0 & 17.2 \\

\arrayrulecolor{gray}
\cmidrule(lr){1-16}
\arrayrulecolor{black}

\textbf{eSCFlow}-14M
& {2.95} & {35.40} & \textbf{99.90} & \ptz0.148 & \ptz1.652
& {2.59} & {30.55} & {99.18} & \ptz0.077 & \ptz1.257
& 2.63 & 39.14 & 99.86 & \ptz0.170 & \ptz1.670 \\

\textbf{eSCFlow}-43M
& \textbf{2.37} & \textbf{34.24} & \textbf{99.90} & \ptz\textbf{0.108} & \ptz\textbf{1.563}
& \textbf{2.14} & \textbf{29.15} & \textbf{99.25} & \ptz\textbf{0.052} & \ptz\textbf{1.173}
& \textbf{2.03} & \textbf{37.58} & \textbf{99.87} & \ptz\textbf{0.136} & \ptz\textbf{1.630} \\

\bottomrule
\end{tabular}
    }
\vspace{-10pt}
\end{table}

\renewcommand{\thefootnote}{\arabic{footnote}}

==> table/qh9_EF.tex <==
% 문서 상단(Preamble)에 이 패키지를 추가하세요
% \usepackage{siunitx}
% \usepackage{multirow}
% \usepackage{booktabs}
% \usepackage[table]{xcolor} % \cellcolor를 위해

\begin{table*}[t]
\centering
\caption{\textbf{QH9 Energy \& Force benchmark.} Results shown in \textbf{bold} denote the best in each column, and the \underline{underlined} ones indicate the second best. Only (Pred $-$ Targ) metrics are reported.}
\label{tab:md17_results_predtarg}
% 테이블 너비 조정
\resizebox{\textwidth}{!}{
\sisetup{detect-all=true}
% 컬럼 정의 수정: Reduction 컬럼 삭제로 S 컬럼이 6개 -> 3개로 감소
% 남은 컬럼: Molecule, Metric, Hamiltonian, Energy, E/atoms, Force
\begin{tabular}{ll S[table-format=3.2] S[table-format=4.2] S[table-format=3.2] S[table-format=3.2]}
\toprule
\arrayrulecolor{gray}
\multirow{2}{*}{\textbf{Molecule}} & 
\multirow{2}{*}{\textbf{Metric (MAE)}} &
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Hamiltonian (meV)}}} &
% \multicolumn 범위를 6에서 3으로 수정 (Energy, E/atoms, Force)
\multicolumn{3}{c}{\textbf{(Pred $-$ Targ)}} \\
% \cmidrule 범위를 4-9에서 4-6으로 수정
\cmidrule(lr){4-6}
 & & & \multicolumn{1}{c}{\textbf{Energy (meV)}} & \multicolumn{1}{c}{\textbf{E/atoms (meV/atom)}} & \multicolumn{1}{c}{\textbf{Force (meV/\AA)}} \\
\midrule

\multirow{10}{*}{\shortstack{QH9-stable \\ (\texttt{id})}} 
 % & DFT-variance & {-} & 0.00008 & {-} & 0.0491 \\
 & UMA-omol (MLFF) & {-} & 7839.93 & 185.17 & 462.77 \\
 & Equiformer{\color{red}$^\dagger$} (MLFF) & {-} & \color{red} 6.59 & {-} & {-} \\
 & EquiformerV2{\color{red}$^\dagger$} (MLFF) & {-} & \color{red} 6.17 & {-} & {-} \\
 & eSEN-5M (MLFF) & {-} & 1449.61 & 83.22 & 7.03 \\
 & eSEN-50M (MLFF) & {-} & 816.29 & 47.00 & 4.18 \\
\arrayrulecolor{lightgray}
\cmidrule(lr){2-6}
\arrayrulecolor{gray}
 & QHNet (DFT) & 77.72 & 434.63 & 27.73 & 2868.26 \\ 
 & QHFlow (DFT) & 22.95 & 2.37 & 0.14 & 4.71 \\
\arrayrulecolor{lightgray}
\cmidrule(lr){2-6}
\arrayrulecolor{gray}
 & \textbf{eSCFlow}-12M (DFT) & 16.29 & 1.42 & 0.08 & 3.12 \\
 & \textbf{eSCFlow}-183M (DFT) & 5.93 & 0.32 & 0.02 & 1.44 \\
 & \textbf{eSCFlow}-990M (DFT) & \bfseries 4.58 & \bfseries 0.21 & \bfseries 0.01 & \bfseries 1.21 \\
\midrule

\multirow{7}{*}{Stable-ood} 
 % & DFT-variance & {-} & 0.0002 & {-} & 0.088 \\
 & UMA-omol (MLFF) & {-} & 6232.34 & 151.97 & 264.55 \\
 & QHNet (DFT) & 69.69 & {-} & {-} & {-} \\
 & QHFlow (DFT) & 20.01 & 8.78 & 0.21 & 0.38 \\
 & \textbf{eSCFlow}-12M (DFT) & 12.52 & {-} & {-} & {-} \\
 & \textbf{eSCFlow}-183M (DFT) & 5.18 & {-} & {-} & {-} \\
 & \textbf{eSCFlow}-990M (DFT) & \bfseries 4.14 & \bfseries 0.20 & \bfseries 0.01 & \bfseries 0.28 \\
\midrule

\multirow{7}{*}{Dynamic-geo} 
 % & DFT-variance & {-} & 0.0004 & {-} & 0.1469 \\
 & UMA-omol (MLFF) & {-} & 7957.00 & 183.16 & 459.39 \\
 & QHNet (DFT) & 88.36 & {-} & {-} & {-} \\
 & QHFlow (DFT) & 25.94 & {-} & {-} & {-} \\
 & \textbf{eSCFlow}-12M (DFT) & 15.44 & {-} & {-} & {-} \\
 & \textbf{eSCFlow}-183M (DFT) & 5.25 & 0.33 & 0.01 & 0.02 \\
 & \textbf{eSCFlow}-990M (DFT) & \bfseries 3.74 & \bfseries 0.15 & \bfseries 0.01 & \bfseries 0.88 \\
\midrule

\multirow{7}{*}{Dynamic-mol} 
 % & DFT-variance & {-} & 0.0004 & {-} & 0.2955 \\
 & UMA-omol (MLFF) & {-} & 7790.00 & 186.76 & 450.00 \\
 & QHNet (DFT) & 121.39 & {-} & {-} & {-} \\
 & QHFlow (DFT) & 45.91 & {-} & {-} & {-} \\
 & \textbf{eSCFlow}-12M (DFT) & 29.68 & {-} & {-} & {-} \\
 & \textbf{eSCFlow}-183M (DFT) & 17.54 & 7.94 & 0.19 & 0.51 \\
 & \textbf{eSCFlow}-990M (DFT) & \bfseries 15.90 & \bfseries 1.66 & \bfseries 0.12 & \bfseries 6.45 \\
% \midrule

% \multirow{7}{*}{\textbf{Average}} 
%  & UMA-omol (MLFF) & {-} & {-} & {-} & {-} \\
%  & Equiformer (MLFF) & {-} & {-} & {-} & {-} \\
%  & QHNet (DFT) & {-} & {-} & {-} & {-} \\ 
%  & QHFlow (DFT) & {-} & {-} & {-} & {-} \\
%  & \textbf{eSCFlow}-12M (DFT) & {-} & {-} & {-} & {-} \\
%  & \textbf{eSCFlow}-183M (DFT) & {-} & {-} & {-} & {-} \\
%  & \textbf{eSCFlow}-990M (DFT) & {-} & {-} & {-} & {-} \\
\bottomrule
\end{tabular}
}
\end{table*}

==> table/qh9_finetuning.tex <==
% \NewTableCommand\SCC[2]{\SetCell{bg=#1, fg=#2}}
% \NewTableCommand\cco{\SetCell{bg=lightorange}}
% \newcolumntype{s}{>{\columncolor{white}} c}
% \newcommand{\RC}{\rowcolor{lightorange}\cellcolor{white}}

% \rowcolor{lightorange}

\begin{table}[t]
\centering
\caption{Ablation experimental results on QH9 dataset Finetuning. Results shown in \textbf{bold} denote the best result in each column, whereas those that are \underline{underlined} indicate the second best.}
\label{tab:qh9_finetunes}
\resizebox{\textwidth}{!}{
\begin{tabular}{clcccccc}
\toprule
\textbf{Dataset} & \textbf{Type} & $H$ [$\mu E_h$] $\downarrow$  &  \OCC~[$\mu E_h$] $\downarrow$ & \SC~[$\%$] $\uparrow$ & \LUMO~[$\mu E_h$] $\downarrow$  & \HOMO~[$\mu E_h$] $\downarrow$ & \GAP~[$\mu E_h$] $\downarrow$  \\
\midrule\midrule
 & WA-Full &
 \ptz{62.69}\ptp{0.001}  & {153.82}\ptp{0.001}  & {98.96}\ptp{0.001} & \ptz\underline{240.07}\ptp{0.001} & \underline{117.26}\ptp{0.001} & \underline{251.81}\ptp{0.001} \\
 & w/o-FT &
\ptz\textbf{22.95}\tp{0.001}  & \underline{119.67}\tp{0.211}  & \underline{99.51}\tp{0.001} & \ptz{437.96}\tp{7.452} & {179.48}\tp{0.098} & {553.87}\tp{7.454}  \\
 \multirow{-3}{*}{\shortstack{QH9-stable \\ (\texttt{id})}}
 & WA-FT  &
\ptz\underline{23.85}\tp{0.003}  &  \textbf{101.92}\tp{0.279}  &   \textbf{99.56}\tp{0.002} & \ptz\textbf{187.48}\tp{6.434} & \ptz\textbf{92.22}\tp{0.234}  & \textbf{206.15}\tp{6.197} \\
 % & (3) WA + Init  &
 % {21.23}  & \ptz{71.75}  & {99.65} & {135.08} & \ptz70.50 & \ptz{148.34} \\
 % \multirow{-5}{*}{\shortstack{QH9-stable \\ (id)}}
 % & (4) DWA  &
 % \textbf{20.28}  & {103.56}  & {99.64} & {121.14} & \ptz66.01 & \ptz{134.72} \\

 
\midrule
 & WA-Full &
 \ptz57.11\ptp{0.001}  & {110.34}\ptp{0.001}  & 98.12\ptp{0.001} & \ptz416.08\ptp{0.001} & \underline{113.55}\ptp{0.001} & \underline{387.83}\ptp{0.001} \\
 & w/o-FT &
\ptz\textbf{20.01}\tp{0.001}  & \ptz\underline{84.54}\tp{0.007}  & \underline{99.04}\tp{0.003} & \ptz\underline{321.20}\tp{1.497} & {130.74}\tp{0.043} & {395.83}\tp{1.510} \\
 \multirow{-3}{*}{\shortstack{QH9-stable \\ (\texttt{ood})}}
 & WA-FT  &
\ptz\underline{20.55}\tp{0.002}  & \ptz\textbf{72.64}\tp{0.018}  & \textbf{99.16}\tp{0.006} & \ptz\textbf{171.24}\tp{0.273} & \ptz\textbf{77.96}\tp{0.095} & \textbf{179.57}\tp{0.271} \\
 % & (3) WA + Init  &
 % 20.36  & \ptz70.30  & 99.19 & \textbf{177.67} & \ptz74.92 & \textbf{184.86} \\
 % \multirow{-5}{*}{\shortstack{QH9-stable \\ (ood)}}
 % & (4) DWA  &
 % 20.12  & 109.82  & 99.17 & 178.46 & \ptz\textbf{72.88} & 188.07 \\

 
 \midrule
  & WA-Full &
 \ptz75.38\ptp{0.001}  & {108.96}\ptp{0.001}  & 98.77\ptp{0.001} & \ptz\underline{231.63}\ptp{0.001} & \underline{114.14}\ptp{0.001} & \underline{219.20}\ptp{0.001} \\
 & w/o-FT &
\ptz\textbf{25.94}\tp{0.001}  & \underline{103.11}\tp{0.031}  & \underline{99.59}\tp{0.001} & \ptz{425.18}\tp{1.119} & {175.18}\tp{0.255} & {547.33}\tp{1.168}\\
 \multirow{-3}{*}{\shortstack{QH9-dynamic \\ (300k-\texttt{geo})}}
 & WA-FT  &
\ptz\underline{27.12}\tp{0.002}  & \ptz\textbf{89.03}\tp{0.213}  & \textbf{99.65}\tp{0.001} & \ptz\textbf{136.63}\tp{4.661} & \ptz\textbf{84.17}\tp{0.211} & \textbf{154.68}\tp{4.449}  \\
 % & (3) WA + Init  &
 % 25.71  & \ptz79.55  & \textbf{99.68} & 123.68 & \ptz75.53 & 138.56 \\
 % \multirow{-5}{*}{\shortstack{QH9-dynamic \\ (300k-geo)}}
 % & (4) DWA  &
 % \textbf{24.40}  & 122.98  & 99.66 & 121.45 & \ptz\textbf{70.66} & \textbf{132.82} \\

 \midrule
  & WA-Full &
 103.47\ptp{0.001}  & 692.17\ptp{0.001}  & 97.02\ptp{0.001} & \underline{1046.21}\ptp{0.001} & 760.85\ptp{0.001} & \underline{1408.36}\ptp{0.001} \\
 & w/o-FT &
\ptz\textbf{45.91}\tp{0.001}  & \underline{442.56}\tp{0.171}  & \underline{98.65}\tp{0.001} & {1344.68}\tp{2.338} & \underline{479.71}\tp{0.150} & {1605.03}\tp{2.286}  \\
 \multirow{-3}{*}{\shortstack{QH9-dynamic \\ (300k-\texttt{mol})}}
 & WA-FT  &
\ptz\underline{46.60}\tp{0.003}  & \textbf{424.75}\tp{0.324}  & \textbf{98.74}\tp{0.001} & \ptz\textbf{912.10}\tp{2.941} & \textbf{403.51}\tp{1.861} & \textbf{1047.88}\tp{2.683} \\
 % & (3) WA + Init  &
 % 25.64  & \textbf{111.21}  & 99.27 & 212.36 & 118.53 & \ptz218.32 \\
 % \multirow{-5}{*}{\shortstack{QH9-dynamic \\ (300k-mol)}}
 % & (4) DWA  &
 % \textbf{24.14}  & 127.29  & 99.24 & \textbf{173.32} & \textbf{105.18} & \ptz\textbf{181.78} \\

\bottomrule
\end{tabular}}
\end{table}


==> table/qh9_finetuning_old.tex <==
\begin{table}[h]
\centering
\caption{{\color{myblue}Experimental results on QH9 dataset Finetuning.}}
\label{tab:qh9_finetunes}
\resizebox{\textwidth}{!}{
\begin{tabular}{clcccccc}
\toprule
 & & $H \downarrow$  & \OCC $\downarrow$  & \SC $\uparrow$ & \LUMO $\downarrow$ & \HOMO $\downarrow$ & \GAP $\downarrow$  \\
\textbf{Dataset} & \textbf{Type} & [$10^{-6}E_h$] &  [$10^{-6}E_h$] &  [$10^{-2}$] &  [$10^{-6}E_h$]  &  [$10^{-6}E_h$] &  [$10^{-6}E_h$]  \\
\midrule\midrule
 & w/o-FT &
22.81  & 103.73  & 99.53 & 426.89 & 163.69 & \ptz543.69 \\
 & (1) WA-Full &
 {47.62}  & \ptz58.41  & {99.34} & {131.82} & \ptz\textbf{65.29} & \ptz{135.78} \\
 & (2) WA  &
 {21.21}  & \ptz\textbf{71.37}  & \textbf{99.66} & \textbf{118.73} & \ptz70.11 & \ptz\textbf{134.37} \\
 & (3) WA + Init  &
 {21.23}  & \ptz{71.75}  & {99.65} & {135.08} & \ptz70.50 & \ptz{148.34} \\
 \multirow{-5}{*}{\shortstack{QH9-stable \\ (id)}}
 & (4) DWA  &
 \textbf{20.28}  & {103.56}  & {99.64} & {121.14} & \ptz66.01 & \ptz{134.72} \\
 
\midrule
 & w/o-FT &
 \textbf{20.00}  & \ptz84.53  & 99.04 & 321.96 & 130.80 & 396.56 \\
 & (1) WA-Full &
 50.32  & \ptz\textbf{68.98}  & 99.02 & 254.28 & \ptz76.11 & 240.84 \\
 & (2) WA  &
 20.38  & \ptz70.67  & 99.20 & 187.42 & \ptz74.80 & 192.16 \\
 & (3) WA + Init  &
 20.36  & \ptz70.30  & 99.19 & \textbf{177.67} & \ptz74.92 & \textbf{184.86} \\
 \multirow{-5}{*}{\shortstack{QH9-stable \\ (ood)}}
 & (4) DWA  &
 20.12  & 109.82  & 99.17 & 178.46 & \ptz\textbf{72.88} & 188.07 \\

 
 \midrule
 & w/o-FT &
 26.15  & 107.80  & 99.59 & 398.36 & 165.77 & 519.93 \\
 & (1) WA-Full &
 54.70  & \ptz64.51  & 99.26 & 151.92 & \ptz65.31 & 147.70 \\
 & (2) WA  &
 25.70  & \ptz\textbf{78.96}  & \textbf{99.68} & \textbf{119.76} & \ptz74.41 & 134.53 \\
 & (3) WA + Init  &
 25.71  & \ptz79.55  & \textbf{99.68} & 123.68 & \ptz75.53 & 138.56 \\
 \multirow{-5}{*}{\shortstack{QH9-dynamic \\ (300k-geo)}}
 & (4) DWA  &
 \textbf{24.40}  & 122.98  & 99.66 & 121.45 & \ptz\textbf{70.66} & \textbf{132.82} \\


 \midrule
 & w/o-FT &
 36.90  & 278.88  & 98.87 & 1167.50 & 317.42 & 1250.70 \\
 & (1) WA-Full &
 00.00  & \ptz00.00  & 00.00 & \ptz000.00 & \ptz00.00 & \ptz000.00 \\
 & (2) WA  &
 25.63  & 111.38  & \textbf{99.28} & 205.43 & 118.67 & \ptz215.65 \\
 & (3) WA + Init  &
 25.64  & \textbf{111.21}  & 99.27 & 212.36 & 118.53 & \ptz218.32 \\
 \multirow{-5}{*}{\shortstack{QH9-dynamic \\ (300k-mol)}}
 & (4) DWA  &
 \textbf{24.14}  & 127.29  & 99.24 & \textbf{173.32} & \textbf{105.18} & \ptz\textbf{181.78} \\

\bottomrule
\end{tabular}}
\end{table}

==> table/qh9_main_0127.tex <==
% ---------- spacing tuning ----------
\setlength{\tabcolsep}{3.2pt}
\renewcommand{\arraystretch}{1.05}
% \definecolor{rowhl}{HTML}{EEEAFE}
\definecolor{rowhl}{HTML}{DDF1FF}


\begin{table*}[t]
\centering
\caption{
\textbf{Hamiltonian prediction model performance on QH9 benchmark.}
Comparison of Hamiltonian prediction methods across QH9-Stable (id/ood) and QH9-Dynamic (geo/mol) splits.
Reported metrics include Hamiltonian MAE $H$ ($\mu$Ha), occupied orbital energy MAE $\epsilon_{\mathrm{occ}}$ ($\mu$Ha),
coefficient similarity $S_c$ (\%), and orbital errors for HOMO, LUMO, and the HOMO--LUMO gap (all in $\mu$Ha),
as well as total-energy and force MAE ($E$ in meV; $F$ in meV/\AA) computed from each predicted Hamiltonian.
QHFlow2 rows are highlighted with \hlc{rowhl}{100}{skyblue}, and the best result in each column is shown in \textbf{bold}. Size suffixes {-s}/{-m}/{-l}/{-xl} denote increasing model capacity.
}

\label{tab:qh9_ham}

\resizebox{\textwidth}{!}{%
\begin{tabular}{l r *{9}{c} @{\hspace{6pt}} *{9}{c}}
\toprule
& &
\multicolumn{9}{c}{\textbf{QH9-stable-id}} &
\multicolumn{9}{c}{\textbf{QH9-stable-ood}} \\
\cmidrule(lr){3-11} \cmidrule(lr){12-20}


\textbf{Model} & \textbf{Param.}
& $H(\downarrow)$ & $\epsilon_{\mathrm{occ}}(\downarrow)$ & $S_c(\uparrow)$
& HOMO$(\downarrow)$ & LUMO$(\downarrow)$ & GAP$(\downarrow)$
& Energy$(\downarrow)$ & E/atom$(\downarrow)$ & Force$(\downarrow)$
& $H(\downarrow)$ & $\epsilon_{\mathrm{occ}}(\downarrow)$ & $S_c(\uparrow)$
& HOMO$(\downarrow)$ & LUMO$(\downarrow)$ & GAP$(\downarrow)$
& Energy$(\downarrow)$ & E/atom$(\downarrow)$ & Force$(\downarrow)$ \\
\cmidrule(r){1-2} \cmidrule(lr){3-11} \cmidrule(lr){12-20}

\multicolumn{20}{l}{\emph{Regression}}\vspace{0.02in}\\
\ptz\ptz QHNet (w/o init) & \ptz20M
& \ptz77.72 & \ptz963.45 & 94.80
& \ptz1546.27 & 18257.34 & 17822.62
& 434.63 & 27.73 & 2868.26
& \ptz69.69 & \ptz884.97 & 93.01
& \ptz1045.99 & 25848.83 & 25370.10
& 427.22 & 17.79 & \ptz\ptz66.13 \\

\ptz\ptz QHNet & \ptz20M
& \ptz46.03 & \ptz459.64 & 98.29
& \ptz\ptz470.63 & \ptz2781.15 & \ptz2967.87
& \ptz36.92 & \ptz2.27 & \ptz\ptz16.26
& \ptz38.13 & \ptz170.45 & 97.77 
& \ptz\ptz255.58 & \ptz1326.76 & \ptz1359.88
& \ptz13.18 & \ptz0.56 & \ptz\ptz\ptz6.31 \\

\ptz\ptz WANet & \ptz29M
& \ptz80.00 & \ptz833.62 & 96.86
& -- & -- & --
& -- & -- & --
& -- & -- & --
& -- & -- & --
& -- & -- & -- \\

\ptz\ptz SPHNet & \ptz30M
& \ptz45.48 & \ptz334.28 & 97.75
& -- & -- & --
& -- & -- & --
& \ptz43.33 & \ptz186.40 & 98.16
& -- & -- & --
& -- & -- & -- \\

\arrayrulecolor{black!40}\midrule
\arrayrulecolor{black}
\multicolumn{20}{l}{\emph{Flow-based}}\vspace{0.02in} \\

\ptz\ptz QHFlow & \ptz28M
& \ptz22.95 & \ptz119.67 & 99.51
& \ptz\ptz179.48 & \ptz\ptz437.96 & \ptz\ptz553.87
& \ptz\ptz2.37 & \ptz0.14 & \ptz\ptz\ptz4.71
& \ptz20.01 & \ptz\ptz84.54 & 99.04
& \ptz\ptz130.74 & \ptz\ptz321.20 & \ptz\ptz395.83
& \ptz\ptz8.78 & \ptz0.38 & \ptz\ptz\ptz3.25 \\

\rowcolor{rowhl}
\ptz\ptz \textbf{QHFlow2-s} & \ptz12M
& \ptz16.29 & \ptz\ptz94.89 & 99.63
& \ptz\ptz148.42 & \ptz\ptz304.69 & \ptz\ptz411.41
& \ptz\ptz1.42 & \ptz0.08 & \ptz\ptz\ptz3.12
& \ptz12.52 & \ptz\ptz54.56 & 99.37
& \ptz\ptz\ptz72.78 & \ptz\ptz182.94 & \ptz\ptz200.18
& \ptz\ptz0.97 & \ptz0.04 & \ptz\ptz\ptz1.59 \\

\rowcolor{rowhl}
\ptz\ptz \textbf{QHFlow2-m} & \ptz43M
& \ptz\ptz9.18 & \ptz\ptz59.23 & 99.73
& \ptz\ptz\ptz77.67 & \ptz\ptz175.68 & \ptz\ptz215.99
& \ptz\ptz0.69 & \ptz0.04 & \ptz\ptz\ptz2.07
& \ptz\ptz7.84 & \ptz\ptz42.11 & 99.53
& \ptz\ptz\ptz49.54 & \ptz\ptz134.83 & \ptz\ptz147.30
& \ptz\ptz0.51 & \ptz0.03 & \ptz\ptz\ptz1.68 \\

\rowcolor{rowhl}
\ptz\ptz \textbf{QHFlow2-l} & 183M
& \ptz\ptz5.93 & \ptz\ptz45.73 & 99.81
& \ptz\ptz\ptz50.50 & \ptz\ptz103.32 & \ptz\ptz119.62
& \ptz\ptz0.32 & \ptz0.02 & \ptz\ptz\ptz1.44
& \ptz\ptz5.18 & \ptz\ptz31.86 & 99.65
& \ptz\ptz\ptz33.69 & \ptz\ptz\ptz98.98 & \ptz\ptz105.87
& \ptz\ptz0.30 & \ptz\textbf{0.01} & \ptz\ptz\ptz0.81 \\

\rowcolor{rowhl}
\ptz\ptz \textbf{QHFlow2-xl} & 990M
& \textbf{\ptz\ptz4.58} & \textbf{\ptz\ptz39.36} & \textbf{99.84}
& \textbf{\ptz\ptz\ptz40.30} & \textbf{\ptz\ptz\ptz73.19} & \textbf{\ptz\ptz\ptz87.74}
& \textbf{\ptz\ptz0.21} & \textbf{\ptz0.01} & \textbf{\ptz\ptz\ptz1.21}
& \textbf{\ptz\ptz4.14} & \textbf{\ptz\ptz26.77} & \textbf{99.71}
& \textbf{\ptz\ptz\ptz28.75} & \textbf{\ptz\ptz\ptz97.83} & \textbf{\ptz\ptz105.72}
& \textbf{\ptz\ptz0.20} & \textbf{\ptz0.01} & \textbf{\ptz\ptz\ptz0.68} \\

\midrule

& &
\multicolumn{9}{c}{\textbf{QH9-dynamic-geo}} &
\multicolumn{9}{c}{\textbf{QH9-dynamic-mol}} \\
\cmidrule(r){1-2} \cmidrule(lr){3-11} \cmidrule(lr){12-20}

\multicolumn{20}{l}{\emph{Regression}}\vspace{0.02in} \\
\ptz\ptz QHNet (w/o init) & \ptz20M
& \ptz88.36 & 1170.50 & 93.65
& \ptz2040.06 & 23269.41 & 22407.96
& 448.63 & 26.87 & 119.25
& \ptz121.39 & 5554.36 & 86.02
& \ptz4352.76 & 53505.09 & 50424.86
& 841.74 & 49.43 & 206.47 \\

\ptz\ptz WANet & \ptz29M
& \ptz74.74 & \ptz416.57 & 99.68
& -- & -- & --
& -- & -- & --
& -- & -- & --
& -- & -- & --
& -- & -- & -- \\

\ptz\ptz SPHNet & \ptz30M
& \ptz52.18 & \ptz100.88 & 99.12
& -- & -- & --
& -- & -- & --
& \ptz108.19 & 1724.10 & 91.49
& -- & -- & --
& -- & -- & -- \\

\arrayrulecolor{black!40}\midrule
\arrayrulecolor{black}
\multicolumn{20}{l}{\emph{Flow-based}}\vspace{0.02in} \\

\ptz\ptz QHFlow & \ptz28M
& \ptz25.94 & \ptz103.11 & 99.59
& \ptz\ptz175.18 & \ptz\ptz425.18 & \ptz\ptz547.33
& \ptz\ptz4.28 & \ptz0.24 & \ptz\ptz\ptz5.24
& \ptz\ptz45.91 & \ptz442.56 & 98.65
& \ptz\ptz479.71 & \ptz1344.68 & \ptz1605.03
& \ptz\ptz8.93 & \ptz0.54 & \ptz\ptz11.42 \\

\rowcolor{rowhl}
\ptz\ptz \textbf{QHFlow2-s} & \ptz12M
& \ptz15.44 & \ptz\ptz53.82 & 99.72
& \ptz\ptz\ptz67.27 & \ptz\ptz430.13 & \ptz\ptz447.54
& \ptz\ptz1.34 & \ptz0.08 & \ptz\ptz\ptz2.85
& \ptz\ptz29.68 & \ptz261.32 & 99.22
& \ptz\ptz263.24 & \ptz\ptz644.01 & \ptz\ptz772.89
& \ptz\ptz4.29 & \ptz0.28 & \ptz\ptz\ptz9.03 \\

\rowcolor{rowhl}
\ptz\ptz \textbf{QHFlow2-m} & \ptz43M
& \ptz\ptz8.70 & \ptz\ptz42.51 & 99.89
& \ptz\ptz\ptz51.80 & \ptz\ptz113.54 & \ptz\ptz143.97
& \ptz\ptz0.51 & \ptz0.03 & \ptz\ptz\ptz1.68
& \ptz\ptz21.99 & \ptz240.09 & 99.39
& \ptz\ptz207.16 & \ptz\ptz378.78 & \ptz\ptz468.62
& \ptz\ptz2.51 & \ptz0.17 & \ptz\ptz\ptz8.07 \\

\rowcolor{rowhl}
\ptz\ptz \textbf{QHFlow2-l} & 183M
& \ptz\ptz5.25 & \ptz\ptz28.19 & 99.94
& \ptz\ptz\ptz30.58 & \ptz\ptz\ptz88.76 & \ptz\ptz101.68
& \ptz\ptz0.22 & \ptz\textbf{0.01} & \ptz\ptz\ptz1.08
& \ptz\ptz17.54 & \ptz214.51 & 99.52
& \ptz\ptz179.23 & \ptz\ptz261.68 & \ptz\ptz324.99
& \ptz\ptz1.85 & \ptz0.13 & \ptz\ptz\ptz6.98 \\

\rowcolor{rowhl}
\ptz\ptz \textbf{QHFlow2-xl} & 990M
& \textbf{\ptz\ptz3.74} & \textbf{\ptz\ptz22.84} & \textbf{99.96}
& \textbf{\ptz\ptz\ptz21.01} & \textbf{\ptz\ptz\ptz44.35} & \textbf{\ptz\ptz\ptz50.57}
& \textbf{\ptz\ptz0.15} & \textbf{\ptz0.01} & \textbf{\ptz\ptz\ptz0.88}
& \textbf{\ptz\ptz15.90} & \textbf{\ptz202.32} & \textbf{99.55}
& \textbf{\ptz\ptz167.38} & \textbf{\ptz\ptz219.52} & \textbf{\ptz\ptz278.06}
& \textbf{\ptz\ptz1.66} & \textbf{\ptz0.12} & \textbf{\ptz\ptz\ptz6.45} \\

\bottomrule
\end{tabular}
}
\vspace{-10pt}
\end{table*}


==> table/qh9_main_old.tex <==
% ---------- spacing tuning (same style) ----------
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.05}
\definecolor{rowhl}{HTML}{EEEAFE}

\begin{table*}[!h]
\centering
\caption{\textbf{QH9 benchmark.}
Comparison of regression-based and flow-based models on QH9 across
in-distribution (iid), and dynamic (geo) splits. Reported metrics include Hamiltonian and orbital errors, as well as derived energy and force errors. Best results in each column are highlighted in \textbf{bold}. ood and mol splits are in the appendix.}
\label{tab:qh9_results}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c l r c c c c c c c c c}
\toprule
\textbf{Dataset} & \textbf{Model} & \textbf{Param.}
& $H\downarrow$ & $\epsilon_{\mathrm{occ}}\downarrow$ & $S_c\uparrow$
& LUMO$\downarrow$ & HOMO$\downarrow$ & GAP$\downarrow$
& Energy$\downarrow$ & Energy/atom$\downarrow$ & Force$\downarrow$ \\
\midrule

% ===================== QH9-stable (id) =====================

\multirow{4}{*}{\shortstack{\textbf{QM9}$^\dagger$}}
& \multicolumn{11}{l}{\emph{MLIP}} \\
& \ptz\ptz Equiformer & \ptz4M
& - & - & -
& 551.24 & 514.49 & 1102.48
& 6.59 & - & - \\
& \ptz\ptz MACE & -
& - & - & -
& 808.48 & 698.24 & 1543.47
& 4.1 & - & - \\
& \ptz\ptz EquiformerV2 & \ptz11M
& - & - & -
& 514.49 & 477.74 & 1065.73
& 6.17 & - & -\\

\midrule

\multirow{12}{*}{\shortstack{\textbf{QH9-stable}\\(\texttt{id})}}
& \multicolumn{11}{l}{\emph{Regression}} \\
& \ptz\ptz QHNet (w/o init) & \ptz20M
& 77.72 & 963.45 & 94.80
& 18257.34 & 1546.27 & 17822.62
& 434.63 & 27.73 & 2868.26 \\
& \ptz\ptz QHNet (w/ init) & \ptz20M
& 46.03 & 459.64 & 98.29
& 2781.15 & 470.63 & 2967.87
& 36.92 & 2.27 & 16.26 \\
& \ptz\ptz WANet & \ptz29M
& 80.00 & 833.62 & 96.86
& -- & -- & --
& -- & -- & -- \\
& \ptz\ptz SPHNet & \ptz30M
& 45.48 & 334.28 & 97.75
& -- & -- & --
& -- & -- & -- \\

\arrayrulecolor{lightgray}
\cmidrule(l{2pt}r{2pt}){2-12}
\arrayrulecolor{black}

& \multicolumn{11}{l}{\emph{Flow-based}} \\
& \ptz\ptz QHFlow & \ptz28M
& 22.95 & 119.67 & 99.51
& 437.96 & 179.48 & 553.87
& 2.37 & 0.14 & 4.71 \\

\rowcolor{rowhl}
\cellcolor{white!0}& \ptz\ptz \textbf{QHFlow-v2-s} & \ptz12M
& 16.29 & 94.89 & 99.63
& 304.69 & 148.42 & 411.41
& 1.42 & 0.08 & 3.12 \\

\rowcolor{rowhl}
\cellcolor{white!0}& \ptz\ptz \textbf{QHFlow-v2-m} & \ptz43M
& 9.18 & 59.23 & 99.73
& 175.68 & 77.67 & 215.99
& 0.69 & 0.04 & 2.07 \\

\rowcolor{rowhl}
\cellcolor{white!0}& \ptz\ptz \textbf{QHFlow-v2-l} & 183M
& 5.93 & 45.73 & 99.81
& 103.32 & 50.50 & 119.62
& 0.32 & 0.02 & 1.44 \\

\rowcolor{rowhl}
\cellcolor{white!0}& \ptz\ptz \textbf{QHFlow-v2-x} & 990M
& \textbf{4.58} & \textbf{39.36} & \textbf{99.84}
& \textbf{73.19} & \textbf{40.30} & \textbf{87.74}
& \textbf{0.21} & \textbf{0.01} & \textbf{1.21} \\

\midrule

% % ===================== QH9-stable (ood) =====================
& \multicolumn{11}{l}{\emph{Flow-based}} \\
& \ptz\ptz QHFlow & \ptz28M
& 20.01 & 84.54 & 99.04
& 321.20 & 130.74 & 395.83
& 8.78 & 0.38 & 3.25 \\

\rowcolor{rowhl}
\cellcolor{white!0}& \ptz\ptz \textbf{QHFlow-v2-s} & \ptz12M
& 12.52 & 54.56 & 99.37
& 182.94 & 72.78 & 200.18
& 0.97 & 0.04 & 1.59 \\

\rowcolor{rowhl}
\cellcolor{white!0}& \ptz\ptz \textbf{QHFlow-v2-m} & \ptz43M
& 7.84 & 42.11 & 99.53
& 134.83 & 49.54 & 147.30
& 0.51 & 0.03 & 1.68 \\

\rowcolor{rowhl}
\cellcolor{white!0}& \ptz\ptz \textbf{QHFlow-v2-l} & 183M
& 5.18 & 31.86 & 99.65
& 98.98 & 33.69 & 105.87
& 0.30 & 0.01 & 0.81 \\

\rowcolor{rowhl}
\cellcolor{white!0}& \ptz\ptz \textbf{QHFlow-v2-x} & 990M
& \textbf{4.14} & \textbf{26.77} & \textbf{99.71}
& \textbf{97.83} & \textbf{28.75} & \textbf{105.72}
& \textbf{0.20} & \textbf{0.01} & \textbf{0.68} \\

\midrule

% ===================== QH9-dynamic (300k-geo) =====================
\multirow{11}{*}{\shortstack{\textbf{QH9-dynamic}\\(300k-\texttt{geo})}}
& \multicolumn{11}{l}{\emph{Regression}} \\
& \ptz\ptz QHNet (w/o init) & \ptz20M
& 88.36 & 1170.50 & 93.65
& 23269.41 & 2040.06 & 22407.96
& TBA & TBA & TBA \\
& \ptz\ptz WANet & \ptz29M
& 74.74 & 416.57 & 99.68
& -- & -- & --
& -- & -- & -- \\
& \ptz\ptz SPHNet & \ptz30M
& 52.18 & 100.88 & 99.12
& -- & -- & --
& -- & -- & -- \\

\arrayrulecolor{lightgray}
\cmidrule(l{2pt}r{2pt}){2-12}
\arrayrulecolor{black}

& \multicolumn{11}{l}{\emph{Flow-based}} \\
& \ptz\ptz QHFlow & \ptz28M
& 25.94 & 103.11 & 99.59
& 425.18 & 175.18 & 547.33
& 4.28 & 0.24 & 5.24 \\

\rowcolor{rowhl}
\cellcolor{white!0}& \ptz\ptz \textbf{QHFlow-v2-s} & \ptz12M
& 15.44 & 53.82 & 99.72
& 430.13 & 67.27 & 447.54
& 1.34 & 0.08 & 2.85 \\

\rowcolor{rowhl}
\cellcolor{white!0}& \ptz\ptz \textbf{QHFlow-v2-m} & \ptz43M
& 8.70 & 42.51 & 99.89
& 113.54 & 51.80 & 143.97
& 0.51 & 0.03 & 1.68 \\

\rowcolor{rowhl}
\cellcolor{white!0}& \ptz\ptz \textbf{QHFlow-v2-l} & 183M
& 5.25 & 28.19 & 99.94
& 88.76 & 30.58 & 101.68
& 0.22 & 0.01 & 1.08 \\

\rowcolor{rowhl}
\cellcolor{white!0}& \ptz\ptz \textbf{QHFlow-v2-x} & 990M
& \textbf{3.74} & \textbf{22.84} & \textbf{99.96}
& \textbf{44.35} & \textbf{21.01} & \textbf{50.57}
& \textbf{0.15} & \textbf{0.01} & \textbf{0.88} \\

\midrule

% % % ===================== QH9-dynamic (300k-mol) =====================
% \multirow{10}{*}{\shortstack{\textbf{QH9-dynamic}\\(300k-\texttt{mol})}}
& \multicolumn{11}{l}{\emph{Regression}} \\
& \ptz\ptz QHNet (w/o init) & \ptz20M
& 121.39 & 5554.36 & 86.02
& 53505.09 & 4352.76 & 50424.86
& -- & -- & -- \\
& \ptz\ptz SPHNet & \ptz30M
& 108.19 & 1724.10 & 91.49
& -- & -- & --
& -- & -- & -- \\

\arrayrulecolor{lightgray}
\cmidrule(l{2pt}r{2pt}){2-12}
\arrayrulecolor{black}

& \multicolumn{11}{l}{\emph{Flow-based}} \\
& \ptz\ptz QHFlow & \ptz28M
& 45.91 & 442.56 & 98.65
& 1344.68 & 479.71 & 1605.03
& -- & -- & -- \\

\rowcolor{rowhl}
\cellcolor{white!0}& \ptz\ptz \textbf{QHFlow-v2-s} & \ptz12M
& 29.68 & 261.32 & 99.22
& 644.01 & 263.24 & 772.89
& 4.29 & 0.28 & 9.03 \\

\rowcolor{rowhl}
\cellcolor{white!0}& \ptz\ptz \textbf{QHFlow-v2-m} & \ptz43M
& 21.99 & 240.09 & 99.39
& 378.78 & 207.16 & 468.62
& 2.51 & 0.17 & 8.07 \\

\rowcolor{rowhl}
\cellcolor{white!0}& \ptz\ptz \textbf{QHFlow-v2-l} & 183M
& 17.54 & 214.51 & 99.52
& 261.68 & 179.23 & 324.99
& 1.85 & 0.13 & 6.98 \\

\rowcolor{rowhl}
\cellcolor{white!0}
\multirow{-9}{*}{\shortstack{\textbf{QH9-dynamic}\\(300k-\texttt{mol})}}
& \ptz\ptz \textbf{QHFlow-v2-x} & 990M
& \textbf{15.90} & \textbf{202.32} & \textbf{99.55}
& \textbf{219.52} & \textbf{167.38} & \textbf{278.06}
& \textbf{1.66} & \textbf{0.12} & \textbf{6.45} \\

\arrayrulecolor{black}
\bottomrule
\end{tabular}%
}
\vspace{-10pt}
\end{table*}


==> table/qh9_runtime.tex <==
\begin{table}[t]
\centering
\caption{
\textbf{Inference runtime and memory on QH9.}
We report inference speed (samples/s) and peak GPU memory (GB) for the forward pass that outputs $\hat{\mathbf H}$ on an NVIDIA RTX A6000 (48GB) with batch size 32.
Higher speed and lower memory are better; best speed is in \textbf{bold}.}
\label{tab:qh9_runtime_inf}

\resizebox{0.4\columnwidth}{!}{%
\begin{tabular}{lrrr}
\toprule
\textbf{Model} & Params. (M) & Mem$\downarrow$ (GB) & Speed$\uparrow$ (samp./s) \\
\midrule
QHNet  & 20  & 11.33 & 34.9 \\
QHFlow & 28  & 10.37 & 27.7 \\
QHFlow & 60  & 13.00 & 18.8 \\
\rowcolor{rowhl}
QHFlow2-s  & 12  & \textbf{9.32}  & \textbf{78.4} \\
\rowcolor{rowhl}
QHFlow2-m  & 43  & 12.09 & 43.7 \\
\rowcolor{rowhl}
QHFlow2-l  & 183 & 31.37 & 21.6 \\
\rowcolor{rowhl}
QHFlow2-xl & 990 & 37.99 & 7.2 \\
\bottomrule
\end{tabular}%
}
\end{table}

==> table/rmd17_md_main.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Revised MD17 molecule dynamics benchmark.} Higher Stability indicates better performance, while lower $h(r)$ and Force denote higher accuracy.}
\label{tab:md17_metric_based}
\resizebox{0.49\textwidth}{!}{
\begin{tabular}{llccccc}
\toprule
{Metric} & {Molecule} 
& {GemNet-dT} & {NequIP} & {QHNet} & {QHFlow} & {\textbf{SCFlow}} \\
\midrule
\midrule
\multirow{4}{*}{Stability ($\uparrow$)} 
& Salicylic Acid (16) & 94  & 300 & TBA & TBA & \textbf{TBA} \\
& Naphthalene    (19) & 25  & 300 & TBA & TBA & \textbf{TBA} \\
& Aspirin        (21) & 192 & 300 & TBA & TBA & \textbf{TBA} \\
\arrayrulecolor{gray}
\cmidrule(lr){2-7}
\arrayrulecolor{black}
& Avg. & 103.7 & 300 & TBA & TBA & \textbf{TBA} \\
\midrule
\multirow{4}{*}{$h(r)$ ($\downarrow$)} 
& Salicylic Acid (16) & 0.07 & 0.03 & TBA & TBA & \textbf{TBA} \\
& Naphthalene    (19) & 0.12 & 0.12 & TBA & TBA & \textbf{TBA} \\
& Aspirin        (21) & 0.04 & 0.02 & TBA & TBA & \textbf{TBA} \\
\arrayrulecolor{gray}
\cmidrule(lr){2-7}
\arrayrulecolor{black}
& Avg. & 0.077 & 0.057 & TBA & TBA & \textbf{TBA} \\
\midrule
\multirow{4}{*}{Force ($\downarrow$)} 
& Salicylic Acid (16) & 4.0 & 1.6 & TBA & TBA & \textbf{TBA} \\
& Naphthalene    (19) & 1.9 & 1.1 & TBA & TBA & \textbf{TBA} \\
& Aspirin        (21) & 5.1 & 2.3 & TBA & TBA & \textbf{TBA} \\
\arrayrulecolor{gray}
\cmidrule(lr){2-7}
\arrayrulecolor{black}
& Avg. & 3.67 & 1.67 & TBA & TBA & \textbf{TBA} \\
\bottomrule
\end{tabular}
}
\end{table}


==> table/size_extra.tex <==
\begin{table}[h]
\centering
\caption{\textbf{Size extrapolation to large molecular systems.}
Performance of QHFlow-v2 on molecules larger than those seen during training.
Overall reports the average across all size bins.}
\label{tab:extrap_size_compact}
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{lcc}
\toprule
\textbf{System Size}
& {H MAE ($\mu$ H)} $\downarrow$
& {E MAE (eV/atom)} $\downarrow$ \\
\midrule
40--80 atoms   & \ptz96.8 & \ptz31.1 \\
80--120 atoms  & \ptz83.1 & 281.3 \\
120--160 atoms & 121.0 & 209.4 \\
\midrule
Overall        & \ptz96.9 & 135.9 \\
\bottomrule
\end{tabular}
}
\end{table}


==> table/unuse/md17.tex <==
\renewcommand{\thefootnote}{\fnsymbol{footnote}}

\begin{table}[t]
\centering
\captionof{table}{\textbf{MD17 benchmark.} Results shown in \textbf{bold} denote the best result in each column, whereas those that are \underline{underlined} indicate the second best.}
\label{tab:md17_results}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccccccccccc}
\toprule
&\multicolumn{3}{c}{Ethanol ($9$ atoms)}
&\multicolumn{3}{c}{Malondialdehyde ($9$ atoms)}
&\multicolumn{3}{c}{Uracil ($12$ atoms)}
&\multicolumn{3}{c}{Salicylic Acid ($16$ atoms)}
&\multicolumn{3}{c}{Naphthalene ($19$ atoms)}
&\multicolumn{3}{c}{Aspirin ($21$ atoms)} \\

\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
\cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19}
& $H$ $\downarrow$ & \OCC $\downarrow$ & \SC $\uparrow$ 
& $H$ $\downarrow$ & \OCC $\downarrow$ & \SC $\uparrow$
& $H$ $\downarrow$ & \OCC $\downarrow$ & \SC $\uparrow$
& $H$ $\downarrow$ & \OCC $\downarrow$ & \SC $\uparrow$
& $H$ $\downarrow$ & \OCC $\downarrow$ & \SC $\uparrow$
& $H$ $\downarrow$ & \OCC $\downarrow$ & \SC $\uparrow$ \\

\multirow{-2}{*}{\textbf{Model}}
& [$\mu E_h$]  & [$\mu E_h$]  &  [$\%$]
& [$\mu E_h$]  & [$\mu E_h$]  &  [$\%$]
& [$\mu E_h$]  & [$\mu E_h$]  &  [$\%$]
& [$\mu E_h$]  & [$\mu E_h$]  &  [$\%$]
& [$\mu E_h$]  & [$\mu E_h$]  &  [$\%$]
& [$\mu E_h$]  & [$\mu E_h$]  &  [$\%$] \\

\midrule
\midrule

SchNOrb 
& 187.4 & 334.4 & \textbf{100.00}
& 191.1 & 400.6 & 99.00
& 227.8 & 1760. & 90.00
& 240.5 & 2100. & 88.50
& 265.3 & 2350. & 87.20
& 280.1 & 2600. & 86.40 \\

PhiSNet
& \underline{20.09} & 102.04 & 99.81
& 21.31 & 100.6 & 99.89
& \underline{18.65} & 143.36 & 99.86
& 20.01 & 185.42 & 99.84
& 22.37 & 210.16 & 99.80
& 24.90 & 230.25 & 99.77 \\

QHNet\footnotemark[1]
& 27.99 & 99.33 & \underline{99.99}
& 29.60 & 100.16 & \underline{99.92}
& 26.80 & 127.93 & \underline{99.87}
& 25.75 & 156.30 & \underline{99.85}
& 28.45 & 182.47 & \underline{99.82}
& 30.12 & 198.64 & \underline{99.80} \\

SPHNet  
& 21.02 & 82.30 & \textbf{100.00}
& \underline{20.67} & 95.77 & \textbf{99.99}
& 19.36 & 118.21 & \textbf{99.99}
& 19.80 & 140.52 & \textbf{99.98}
& 21.45 & 165.32 & \textbf{99.98}
& 23.12 & 180.47 & \textbf{99.97} \\

\RC
QHFlow
& 5.33 & 29.03 & 100.00
& 3.80 & 22.68 & 99.99
& 3.68 & 30.54 & 99.99
& 3.55 & 31.62 & 99.99
& 3.42 & 33.80 & 99.99
& 3.35 & 34.75 & 99.99 \\

\arrayrulecolor{gray}
\cmidrule(lr){1-19}
\arrayrulecolor{black}

\textbf{QHFlow-v3}
& \textbf{5.33} & \textbf{29.03} & \textbf{100.00}
& \textbf{3.80} & \textbf{22.68} & \textbf{99.99}
& \textbf{3.68} & \textbf{30.54} & \textbf{99.99}
& \textbf{3.55} & \textbf{31.62} & \textbf{99.99}
& \textbf{3.42} & \textbf{33.80} & \textbf{99.99}
& \textbf{3.35} & \textbf{34.75} & \textbf{99.99} \\

\bottomrule
\end{tabular}
}
\vspace{-10pt}
\end{table}

\renewcommand{\thefootnote}{\arabic{footnote}}

==> table/unuse/md17_EF.tex <==
% 문서 상단(Preamble)에 이 패키지를 추가하세요
% \usepackage{siunitx}
% \usepackage{multirow}
% \usepackage{booktabs}
% \usepackage[table]{xcolor} % \cellcolor를 위해

\begin{table*}[t]
\centering
\caption{\textbf{MD17 benchmark.} Results shown in \textbf{bold} denote the best in each column, and the \underline{underlined} ones indicate the second best. Only (Pred $-$ Targ) metrics are reported.}
\label{tab:md17_results_predtarg}
% 테이블이 넓어졌으므로 \textwidth로 조정
\resizebox{\textwidth}{!}{
\sisetup{detect-all=true}
% S 컬럼 순서 변경 및 Reduction %를 위해 table-format=+3.1 (예: +106.0) 추가
\begin{tabular}{ll S[table-format=1.3] S[table-format=5.6] S[table-format=+3.1] S[table-format=3.4] S[table-format=+3.1]}
\toprule
\multirow{2}{*}{\textbf{Molecule}} & 
\multirow{2}{*}{\textbf{Metric (MAE)}} &
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Hamiltonian (meV)}}} &
% \multicolumn 범위를 4로 유지
\multicolumn{4}{c}{\textbf{(Pred $-$ Targ)}} \\
% \cmidrule 범위를 4-7로 유지, 헤더 순서 변경
\cmidrule(lr){4-7}
 & & & \multicolumn{1}{c}{\textbf{Energy (meV)}} & \multicolumn{1}{c}{\textbf{E. Reduc. (\%)}} & \multicolumn{1}{c}{\textbf{Force (meV/\AA)}} & \multicolumn{1}{c}{\textbf{F. Reduc. (\%)}} \\
\midrule

% \multirow{6}{*}{{Water}} 
%  & DFT-variance & {-} & 0.00008 & {-} & 0.0491 & {-} \\
%  & UMA-omol (MLFF) & {-} & 4326. & {-} & 362. & {-} \\
%  & Equiformer (MLFF) & {-} & {-} & {-} & {-} & {-} \\
%  & QHNet (DFT) & 0.323 & 0.048 & {-} & 0.803 & {-} \\ 
%  & QHFlow (DFT) &  0.105 &  0.015 & {-} &  0.270 & {-} \\
%  & \textbf{eSCFlow} (DFT) & {-} & {-} & {-} & {-} & {-} \\ 
% \midrule

\multirow{6}{*}{{Ethanol}} 
 & DFT-variance & {-} & 0.0002 & {-} & 0.088 & {-} \\
 & UMA-omol (MLFF) & {-} & 8194. & {-} & 334. & {-} \\
 % Equiformer를 기준으로 0.0 표기
 & Equiformer (MLFF) & {-} & 2.2 & 0.0 & 2.9 & 0.0 \\
 & QHNet (DFT)  & 0.633 & 0.323 & -85.3 & 2.513 & -13.3 \\
 & QHFlow (DFT) & 0.152 & 0.019 & -99.1 & 0.775 & -73.3 \\
 & \textbf{eSCFlow} (DFT) & \bfseries 0.092 & \bfseries 0.007 & \bfseries -99.68 & \bfseries 0.443 & \bfseries -84.72 \\ 
\midrule

\multirow{6}{*}{{Malondialdehyde}} 
 & DFT-variance & {-} & 0.0004 & {-} & 0.1469 & {-} \\
 & UMA-omol (MLFF) & {-} & 13166. & {-} & 487. & {-} \\
 % Equiformer를 기준으로 0.0 표기
 & Equiformer (MLFF) & {-} & 3.2 & 0.0 & 5.4 & 0.0 \\
 & QHNet (DFT)  &  0.653 &  0.916 &  -71.4 &  4.949 &  -8.4 \\
 & QHFlow (DFT) &  0.116 &  0.035 &  -98.9 &  1.187 &  -78.0 \\
 & \textbf{eSCFlow} (DFT) & \bfseries 0.072 & \bfseries 0.014 & \bfseries -99.56 & \bfseries 0.728 & \bfseries -86.51 \\ 
\midrule

\multirow{6}{*}{{Uracil}} 
 & DFT-variance & {-} & 0.0004 & {-} & 0.2955 & {-} \\
 & UMA-omol (MLFF) & {-} & 21212. & {-} & 367. & {-} \\
 % Equiformer를 기준으로 0.0 표기
 & Equiformer (MLFF) & {-} & 4.3 & 0.0 & 3.3 & 0.0 \\
 & QHNet (DFT)  & 0.546  &  2.351 &  -45.3 &  6.798 & +106.0 \\
 & QHFlow (DFT) &  0.109 &  0.106 &  -97.5 &  1.869 &  -43.4 \\
 & \textbf{eSCFlow} (DFT) & \bfseries 0.064 & \bfseries 0.097 & \bfseries -97.74 & \bfseries 1.248 & \bfseries -62.18 \\ 
\bottomrule
\end{tabular}
}
\end{table*}

==> table/unuse/md17_EF_full.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{MD17 benchmark.} Results shown in \textbf{bold} denote the best in each column, and the \underline{underlined} ones indicate the second best.}
\label{tab:md17_results}
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{llccccccccc}
\toprule
\multirow{2}{*}{\textbf{Molecule}} & 
\multirow{2}{*}{\textbf{Metric (MAE)}} &
\multirow{2}{*}{\textbf{Hamiltonian}} &
\multicolumn{3}{c}{\cellcolor{green!10}Energy (meV)} &
\multicolumn{3}{c}{\cellcolor{blue!10}Force (meV/\AA)} \\
\cmidrule(lr){4-6} \cmidrule(lr){7-9}
 & & & (Pred $-$ Targ) & (Pred $-$ Calc) & (Targ $-$ Calc) & (Pred $-$ Targ) & (Pred $-$ Calc) & (Targ $-$ Calc) \\
\midrule

\multirow{4}{*}{\textbf{Water (3999)}} 
 & UMA-omol (MLFF) & - & 4326.0 & 4326.0 & - & 362.0 & 362.0 & - \\
 & Equiformer (MLFF) & - & - & - & - & - & - & - \\
 & QHNet (DFT) & 0.3231 & 0.048156 & 0.048422 & 0.000075 & 0.803774 & 0.804033 & - \\
 & \cellcolor{orange!10}QHFlow (DFT) & \cellcolor{orange!10}\textbf{0.1045} & \cellcolor{orange!10}\textbf{0.014922} & \cellcolor{orange!10}\textbf{0.014997} & \cellcolor{orange!10}0.000075 & \cellcolor{orange!10}\textbf{0.269742} & \cellcolor{orange!10}\textbf{0.268452} & \cellcolor{orange!10}0.049198 \\
\midrule

\multirow{4}{*}{\textbf{Ethanol (4000)}} 
 & UMA-omol (MLFF) & - & 8194.0 & 8194.0 & - & 334.0 & 334.0 & - \\
 & Equiformer (MLFF) & - & 2.200000 & 2.900000 & 2.900000 & - & - & - \\
 & QHNet (DFT) & 0.6332 & 0.322580 & 0.322800 & 0.000220 & 2.513448 & 2.520802 & - \\
 & \cellcolor{orange!10}QHFlow (DFT) & \cellcolor{orange!10}\textbf{0.1524} & \cellcolor{orange!10}\textbf{0.018826} & \cellcolor{orange!10}\textbf{0.019046} & \cellcolor{orange!10}0.000220 & \cellcolor{orange!10}\textbf{0.774839} & \cellcolor{orange!10}\textbf{0.767824} & \cellcolor{orange!10}0.088317 \\
\midrule

\multirow{4}{*}{\textbf{Malondialdehyde (1498)}} 
 & UMA-omol (MLFF) & - & 13166.0 & 13166.0 & - & 487.0 & 487.0 & - \\
 & Equiformer (MLFF) & - & 3.200000 & 3.200000 & - & 5.400000 & 5.400000 & - \\
 & QHNet (DFT) & 0.6533 & 0.915961 & 0.916372 & 0.000410 & 4.949360 & 4.947794 & - \\
 & \cellcolor{orange!10}QHFlow (DFT) & \cellcolor{orange!10}\textbf{0.1158} & \cellcolor{orange!10}\textbf{0.034473} & \cellcolor{orange!10}\textbf{0.034884} & \cellcolor{orange!10}0.000410 & \cellcolor{orange!10}\textbf{1.186936} & \cellcolor{orange!10}\textbf{1.184606} & \cellcolor{orange!10}0.146898 \\
\midrule

\multirow{4}{*}{\textbf{Uracil (4500)}} 
 & UMA-omol (MLFF) & - & 21212.0 & 21212.0 & - & 367.0 & 367.0 & - \\
 & Equiformer (MLFF) & - & 4.300000 & 4.300000 & - & 3.300000 & 3.300000 & - \\
 & QHNet (DFT) & 0.5464 & 2.351676 & 2.352124 & 0.000448 & 6.798087 & 6.806976 & - \\
 & \cellcolor{orange!10}QHFlow (DFT) & \cellcolor{orange!10}\textbf{0.1086} & \cellcolor{orange!10}\textbf{0.106172} & \cellcolor{orange!10}\textbf{0.106621} & \cellcolor{orange!10}0.000448 & \cellcolor{orange!10}\textbf{1.869229} & \cellcolor{orange!10}\textbf{1.900374} & \cellcolor{orange!10}0.295586 \\
\bottomrule
\end{tabular}
}
\end{table*}

==> table/unuse/md17_EF_qhflow.tex <==
% 문서 상단(Preamble)에 이 패키지를 추가하세요
% \usepackage{siunitx}
% \usepackage{multirow}
% \usepackage{booktabs}
% \usepackage[table]{xcolor} % \cellcolor를 위해

\begin{table*}[t]
\centering
\caption{\textbf{MD17 benchmark.} Results shown in \textbf{bold} denote the best in each column, and the \underline{underlined} ones indicate the second best. Only (Pred $-$ Targ) metrics are reported.}
\label{tab:md17_results_predtarg}
% 테이블이 넓어졌으므로 \textwidth로 조정
\resizebox{\textwidth}{!}{
\sisetup{detect-all=true}
% S 컬럼 순서 변경 및 Reduction %를 위해 table-format=+3.1 (예: +106.0) 추가
\begin{tabular}{ll S[table-format=1.3] S[table-format=5.6] S[table-format=+3.1] S[table-format=3.4] S[table-format=+3.1]}
\toprule
\textbf{Molecule} &
\textbf{Metric} &
\textbf{Hamiltonian}{~[meV]} &
\textbf{Energy}{~[meV]} &
\textbf{E. Reduc.}{~[\%]} &
\textbf{Force}{~[meV/\AA]} &
\textbf{F. Reduc.}{~[\%]} \\
\midrule

% \multirow{6}{*}{{Water}} 
%  & DFT-variance & {-} & 0.00008 & {-} & 0.0491 & {-} \\
%  & UMA-omol (MLFF) & {-} & 4326. & {-} & 362. & {-} \\
%  & Equiformer (MLFF) & {-} & {-} & {-} & {-} & {-} \\
%  & QHNet (DFT) & 0.323 & 0.048 & {-} & 0.803 & {-} \\ 
%  & QHFlow (DFT) &  0.105 &  0.015 & {-} &  0.270 & {-} \\
%  & \textbf{eSCFlow} (DFT) & {-} & {-} & {-} & {-} & {-} \\ 
% \midrule

\multirow{3}{*}{{Ethanol}} 
 % & DFT-variance & {-} & 0.0002 & {-} & 0.088 & {-} \\
 % & UMA-omol (MLFF) & {-} & 8194. & {-} & 334. & {-} \\
 % Equiformer를 기준으로 0.0 표기
 & Equiformer (MLFF) & {-} & 2.2 & 0.0 & 2.9 & 0.0 \\
 & QHNet (DFT)  & 0.633 & 0.323 & -85.3 & 2.513 & -13.3 \\
 & \textbf{QHFlow} (DFT) & \bfseries 0.152 & \bfseries 0.019 & \bfseries -99.1 & \bfseries 0.775 & \bfseries -73.3 \\
 % & \textbf{eSCFlow} (DFT) & \bfseries 0.092 & \bfseries 0.007 & \bfseries -99.68 & \bfseries 0.443 & \bfseries -84.72 \\ 
\midrule

\multirow{3}{*}{{Malondialdehyde}} 
 % & DFT-variance & {-} & 0.0004 & {-} & 0.1469 & {-} \\
 % & UMA-omol (MLFF) & {-} & 13166. & {-} & 487. & {-} \\
 % Equiformer를 기준으로 0.0 표기
 & Equiformer (MLFF) & {-} & 3.2 & 0.0 & 5.4 & 0.0 \\
 & QHNet (DFT)  &   0.653 &   0.916 &   -71.4 &   4.949 &   -8.4 \\
 & \textbf{QHFlow} (DFT) &  \bfseries 0.116 &  \bfseries 0.035 &  \bfseries -98.9 &  \bfseries 1.187 &  \bfseries -78.0 \\
 % & \textbf{eSCFlow} (DFT) & \bfseries 0.072 & \bfseries 0.014 & \bfseries -99.56 & \bfseries 0.728 & \bfseries -86.51 \\ 
\midrule

\multirow{3}{*}{{Uracil}} 
 % & DFT-variance & {-} & 0.0004 & {-} & 0.2955 & {-} \\
 % & UMA-omol (MLFF) & {-} & 21212. & {-} & 367. & {-} \\
 % Equiformer를 기준으로 0.0 표기
 & Equiformer (MLFF) & {-} & 4.3 & 0.0 & 3.3 & 0.0 \\
 & QHNet (DFT)  & 0.546  &   2.351 &   -45.3 &   6.798 &  +106.0 \\
 & \textbf{QHFlow} (DFT) &  \bfseries 0.109 &  \bfseries 0.106 &  \bfseries -97.5 &  \bfseries 1.869 &  \bfseries -43.4 \\
 % & \textbf{eSCFlow} (DFT) & \bfseries 0.064 & \bfseries 0.097 & \bfseries -97.74 & \bfseries 1.248 & \bfseries -62.18 \\ 
\bottomrule
\end{tabular}
}
\end{table*}

==> table/unuse/md17_trans.tex <==
\begin{table}[t]
\centering
\captionof{table}{\textbf{MD17 benchmark (grouped by Metric, then Molecule).}
Best results are in \textbf{bold}, second best are \underline{underlined}.}
\label{tab:md17_results_by_metric}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{llcccccc}
\toprule
{Metric} & {Molecule} & {SchNOrb} & {PhiSNet} & {QHNet}\footnotemark[1] & {SPHNet} & {QHFlow} & \textbf{QHFlow-v3} \\
\midrule
\midrule
\multirow{6}{*}{$H$ [$\mu E_h$]}
 % & Water (3)           & 165.4  & 15.67              & \underline{11.70} & 23.18  & \textbf{4.93} & \textbf{4.93} \\
 & Ethanol (9)         & 187.4  & {20.09}  & 27.99   & 21.02   & {5.33} & \textbf{3.39} \\
 & Malondialdehyde (9) & 191.1  & 21.31    & 29.60   & {20.67} & {3.80} & \textbf{2.67} \\
 & Uracil (12)         & 227.8  & {18.65}  & 26.80   & 19.36   & {3.68} & \textbf{2.37} \\
 & Salicylic Acid (16) & -  & -  & xx   & xx   & xx & xx \\
 & Naphthalene (19)    & -  & -  & xx   & xx   & xx & xx \\
 & Asprin (21)         & -  & -  & xx   & xx   & xx & xx \\
\midrule
\multirow{6}{*}{$\epsilon_{\text{occ}}$ [$\mu E_h$]}
 % & Water (3)           & 279.3  & 85.53              & \underline{26.06} & 182.29 & \textbf{19.29} & \textbf{19.29} \\
 & Ethanol (9)         & 334.4  & 102.04  & 99.33   & {82.30}  & 29.03   & \textbf{18.40} \\
 & Malondialdehyde (9) & 400.6  & 100.6   & 100.16  & {95.77}  & {22.68} & \textbf{15.13} \\
 & Uracil (12)         & 1760.  & 143.36  & 127.93  & {118.21} & {30.54} & \textbf{21.59} \\
  & Salicylic Acid (16) & -  & -  & xx   & xx   & xx & xx \\
 & Naphthalene (19)    & -  & -  & xx   & xx   & xx & xx \\
 & Asprin (21)         & -  & -  & xx   & xx   & xx & xx \\
\midrule
\multirow{6}{*}{$S_C$ [\%]}
 % & Water (3)           & \textbf{100.00} & \textbf{100.00} & \textbf{100.00} & \textbf{100.00} & 100.00 & 100.00 \\
 & Ethanol (9)         & \textbf{100.00} & 99.81           & {99.99} & \textbf{100.00} & \textbf{100.00} & \textbf{100.00} \\
 & Malondialdehyde (9) & 99.00           & 99.89           & {99.92} & \textbf{99.99} & \textbf{99.99} & \textbf{99.99} \\
 & Uracil (12)         & 90.00           & 99.86           & {99.87} & \textbf{99.99} & \textbf{99.99} & \textbf{99.99} \\
 & Salicylic Acid (16) & -  & -  & xx   & xx   & xx & xx \\
 & Naphthalene (19)    & -  & -  & xx   & xx   & xx & xx \\
 & Asprin (21)         & -  & -  & xx   & xx   & xx & xx \\
 \midrule
 \multirow{6}{*}{$E$ [meV]}
 % & Water (3)           & \textbf{100.00} & \textbf{100.00} & \textbf{100.00} & \textbf{100.00} & 100.00 & 100.00 \\
 & Ethanol (9)         & -  & -  & 0.322   & -   & 0.019 & xx \\
 & Malondialdehyde (9) & -  & -  & 0.915   & -   & 0.034 & xx \\
 & Uracil (12)         & -  & -  & 2.351   & -   & 0.105 & xx \\
 & Salicylic Acid (16) & -  & -  & xx   & -   & xx & xx \\
 & Naphthalene (19)    & -  & -  & xx   & -   & xx & xx \\
 & Asprin (21)         & -  & -  & xx   & -   & xx & xx \\
  \midrule
  \multirow{6}{*}{$F$ [meV/\AA]}
 % & Water (3)           & \textbf{100.00} & \textbf{100.00} & \textbf{100.00} & \textbf{100.00} & 100.00 & 100.00 \\
 & Ethanol (9)         & -  & -  & 2.513   & -   & 0.774 & xx \\
 & Malondialdehyde (9) & -  & -  & 4.949   & -   & 1.187 & xx \\
 & Uracil (12)         & -  & -  & 6.798   & -   & 1.869 & xx \\
 & Salicylic Acid (16) & -  & -  & xx   & -   & xx & xx \\
 & Naphthalene (19)    & -  & -  & xx   & -   & xx & xx \\
 & Asprin (21)         & -  & -  & xx   & -   & xx & xx \\
\bottomrule
\end{tabular}
}
\vspace{-10pt}
\end{table}


==> table/unuse/qh9.tex <==

\begin{table}[t]
\centering
\caption{\textbf{QH9 benchmark.} WA-FT implies finetuned model with WAloss. Results shown in \textbf{bold} denote the best result in each column, whereas those that are \underline{underlined} indicate the second best.}
\label{tab:qh9_results}
\resizebox{\textwidth}{!}{
\begin{tabular}{clrcccccc}
\toprule
 % &  & $H$  $\downarrow$  & \OCC~ $\downarrow$  & \SC~ $\uparrow$ &
 % \LUMO~  $\downarrow$ & \HOMO~ $\downarrow$ & \GAP~$\downarrow$  \\

 % \textbf{Dataset} & \textbf{Model} & [$\mu E_h$]   & [$\mu E_h$]  & [$\%$]  &
 % [$\mu E_h$]  & [$\mu E_h$] & [$\mu E_h$] \\
 
  \textbf{Dataset} & \textbf{Model} &  \textbf{Param.} & $H$  $\downarrow$ [$\mu E_h$]  & \OCC~ $\downarrow$ [$\mu E_h$]  & \SC~ $\uparrow$ [$\%$] &
 \LUMO~  $\downarrow$ [$\mu E_h$] & \HOMO~ $\downarrow$ [$\mu E_h$] & \GAP~$\downarrow$  [$\mu E_h$] \\


\midrule
\midrule
\arrayrulecolor{gray}

%%%% SIZE-id
% \rowcolor{Gray}\cellcolor{white}
% & \texttt{1e} & \ptz0.10 & \ptz\ptz2.47& 99.99 & \ptz\ptz\ptz\ptz0.93 & \ptz\ptz\ptz1.57 & \ptz\ptz\ptz\ptz1.49 \\
% & QHNet    & 76.31  & 798.51  & 95.85 & - & - & - \\
 \multirow{12}{*}{\shortstack{QH9-stable \\ (\texttt{id})}}
& QHNet$^*$& \ptz20M & \ptz77.72\ptpz{0.001}  & \ptz963.45\ptpz{0.001}  & 94.80\ptpz{0.001} & 18257.34\ptpz{0.001} & 1546.27\ptpz{0.001} & 17822.62\ptpz{0.001} \\
& WANet    & \ptz29M & \ptz80.00\ptpz{0.001}  & \ptz833.62\ptpz{0.001}  & 96.86\ptpz{0.001} & - & - & -  \\
& SPHNet   & \ptz30M & \ptz45.48\ptpz{0.001}  & \ptz334.28\ptpz{0.001}  & 97.75\ptpz{0.001} & - & - & -  \\


%  & \textbf{QHFlow}     & \textbf{23.44}  & \underline{123.73}  & \underline{99.48} & \ptz\ptz\underline{505.63} & \ptz\underline{181.13} & \ptz\ptz\underline{612.53}  \\
\arrayrulecolor{lightgray}
\cmidrule(lr){2-9}
\arrayrulecolor{gray}

 & {QHFlow}   & \ptz28M  & \ptz{22.95}\tpz{0.001}  & \ptz{119.67}\tpz{0.211}  & {99.51}\tpz{0.001} & \ptz\ptz{437.96}\tpz{7.452} & \ptz{179.48}\tpz{0.098} & \ptz\ptz{553.87}\tpz{7.454}  \\

& {QHFlow (WA-FT)} & \ptz28M  & \ptz{23.85}\tpz{0.003}  &  \ptz{101.92}\tpz{0.279}  &   {99.56}\tpz{0.002} & \ptz\ptz{187.48}\tpz{6.434} & \ptz\ptz{92.22}\tpz{0.234}  & \ptz\ptz{206.15}\tpz{6.197} \\

\arrayrulecolor{lightgray}
\cmidrule(lr){2-9}
\arrayrulecolor{gray}

% & \textbf{eSCFlow}-tiny   & \ptz\ptz4M  & \ptz{-}\tpz{0.003}  & \ptz{-}\tpz{0.003}  & {-}\tpz{0.001} & \ptz\ptz{-}\tpz{7.452} & \ptz{-}\tpz{0.098} & \ptz\ptz{-}\tpz{7.454}  \\

& \textbf{eSCFlow}-small   & \ptz  12M  & \ptz{16.29}\tpz{0.003}  & \ptz\ptz{94.89}\tpz{0.003}  & {99.63}\tpz{0.001} & \ptz\ptz{304.69}\tpz{7.452} & \ptz\ptz{148.42}\tpz{0.098} & \ptz\ptz{411.41}\tpz{7.454}  \\

& \textbf{eSCFlow}-middle   & \ptz43M  & \ptz\ptz{9.18}\tpz{0.003}  & \ptz\ptz{59.23}\tpz{0.003}  & {99.73}\tpz{0.001} & \ptz\ptz{175.68}\tpz{7.452} & \ptz\ptz{77.67}\tpz{0.098} & \ptz\ptz{215.99}\tpz{7.454}  \\

& \textbf{eSCFlow}-large   & 183M  & \ptz\ptz{5.93}\tpz{0.003}  & \ptz\ptz{45.73}\tpz{0.003}  & {99.81}\tpz{0.001} & \ptz\ptz{103.32}\tpz{7.452} & \ptz\ptz{50.50}\tpz{0.098} & \ptz\ptz{119.62}\tpz{7.454}  \\

& \textbf{eSCFlow}-xlarge   & 990M  & \ptz\ptz\textbf{4.58}\tpz{0.003}  & \ptz\ptz\textbf{39.36}\tpz{0.003}  & \textbf{99.84}\tpz{0.001} & \ptz\ptz\ptz\textbf{73.19}\tpz{7.452} & \ptz\ptz\textbf{40.30}\tpz{0.098} & \ptz\ptz\ptz\textbf{87.74}\tpz{7.454}  \\

\arrayrulecolor{lightgray}
\cmidrule(lr){2-9}
\arrayrulecolor{gray}

& \textbf{eSCFlow}-large (WA-FT)   & 183M  & \ptz\ptz{5.86}\tpz{0.003}  & \ptz\ptz{39.78}\tpz{0.003}  & {99.84}\tpz{0.001} & \ptz\ptz\ptz{68.48}\tpz{7.452} & \ptz\ptz{40.17}\tpz{7.454} & \ptz\ptz\ptz{78.04}\tpz{0.098}    \\

% \arrayrulecolor{lightgray}
% \cmidrule(lr){2-9}
% \arrayrulecolor{gray}

% & {QHFlow-v3-large (no init)}   & 183M  & \ptz{16.22}\tpz{0.003}  & \ptz{150.04}\tpz{0.003}  & {99.52}\tpz{0.001} & \ptz\ptz{794.71}\tpz{7.452} & \ptz{109.16}\tpz{0.098} & \ptz\ptz{825.32}\tpz{7.454}  \\

\midrule

% \cmidrule(lr){1-8}



%%%% SIZE-OOD
% \rowcolor{Gray}\cellcolor{white}
% & \texttt{1e} & \ptz0.10 & \ptz\ptz2.47& 99.99 & \ptz\ptz\ptz\ptz0.93 & \ptz\ptz\ptz1.57 & \ptz\ptz\ptz\ptz1.49 \\
% & QHNet    & 72.11  & 644.17  & 93.68 & - & - & -  \\
\multirow{11}{*}{\shortstack{QH9-stable \\ (\texttt{ood})}} 
& QHNet$^*$ &\ptz20M &  \ptz69.69\ptpz{0.001}  & \ptz884.97\ptpz{0.001}  & 93.01\ptpz{0.001} & 25848.83\ptpz{0.001} & 1045.99\ptpz{0.001} & 25370.10\ptpz{0.001}  \\
& SPHNet  &~30M  & \ptz43.33\ptpz{0.001}  & \ptz186.40\ptpz{0.001}  & 98.16\ptpz{0.001} & - & - & -  \\

%  & \textbf{QHFlow}     & \textbf{20.41}  & \ptz\underline{82.83}  & \underline{99.03} & \ptz\ptz\underline{344.05} & \ptz\underline{111.97} & \ptz\ptz\underline{301.31} \\
\arrayrulecolor{lightgray}
\cmidrule(lr){2-9}
\arrayrulecolor{gray}

 & QHFlow   &\ptz28M  & \ptz{20.01}\tpz{0.001}  & \ptz\ptz{84.54}\tpz{0.007}  & {99.04}\tpz{0.003} & \ptz\ptz{321.20}\tpz{1.497} & \ptz{130.74}\tpz{0.043} & \ptz\ptz{395.83}\tpz{1.510} \\

 
& QHFlow (WA-FT)   &\ptz28M  & \ptz{20.55}\tpz{0.002}  & \ptz\ptz{72.64}\tpz{0.018}  & {99.16}\tpz{0.006} & \ptz\ptz{171.24}\tpz{0.273} & \ptz\ptz{77.96}\tpz{0.095} & \ptz\ptz{179.57}\tpz{0.271} \\


\arrayrulecolor{lightgray}
\cmidrule(lr){2-9}
\arrayrulecolor{gray}

% & \textbf{eSCFlow}-tiny   & \ptz\ptz4M  & \ptz{-}\tpz{0.003}  & \ptz{-}\tpz{0.003}  & {-}\tpz{0.001} & \ptz\ptz{-}\tpz{7.452} & \ptz{-}\tpz{0.098} & \ptz\ptz{-}\tpz{7.454}  \\

& \textbf{eSCFlow}-small   & \ptz  12M  & \ptz{12.52}\tpz{0.003}  & \ptz\ptz{54.56}\tpz{0.003}  & {99.37}\tpz{0.001} & \ptz\ptz{182.94}\tpz{7.452} & \ptz\ptz{72.78}\tpz{0.098} & \ptz\ptz{200.18}\tpz{7.454}  \\

& \textbf{eSCFlow}-middle   & \ptz43M  & \ptz\ptz{7.84}\tpz{0.003}  & \ptz\ptz{42.11}\tpz{0.003}  & {99.53}\tpz{0.001} & \ptz\ptz{134.83}\tpz{7.452} & \ptz\ptz{49.54}\tpz{0.098} & \ptz\ptz{147.30}\tpz{7.454}  \\

& \textbf{eSCFlow}-large   & 183M  & \ptz\ptz{5.18}\tpz{0.003}  & \ptz\ptz{31.86}\tpz{0.003}  & {99.65}\tpz{0.001} & \ptz\ptz\ptz{98.98}\tpz{7.452} & \ptz\ptz{33.69}\tpz{7.454} & \ptz\ptz{105.87}\tpz{0.098}    \\

& \textbf{eSCFlow}-xlarge   & 990M  & \ptz\ptz\textbf{4.14}\tpz{0.003}  & \ptz\ptz\textbf{26.77}\tpz{0.003}  & \textbf{99.71}\tpz{0.001} & \ptz\ptz\ptz\textbf{97.83}\tpz{7.452} & \ptz\ptz\textbf{28.75}\tpz{0.098} & \ptz\ptz\textbf{105.72}\tpz{7.454}  \\



% & \textbf{QHFlow (WAD-FT)}     & \underline{20.36}  & \ptz\ptz\textbf{70.30}  & \textbf{99.19} & \ptz\ptz\textbf{177.67} & \ptz\ptz\textbf{74.92} & \ptz\ptz\textbf{184.86} \\
\midrule
% \cmidrule(lr){1-8}

% %%%% 300k-geo
% \rowcolor{Gray}\cellcolor{white}
% & \texttt{1e} & \ptz0.08 & \ptz\ptz\ptz1.89 & 99.99 & \ptz\ptz\ptz\ptz1.22 & \ptz\ptz\ptz0.74 & \ptz\ptz\ptz\ptz1.19 \\
% & QHNet    & 70.03  & \ptz408.31  & 97.60 & - & - & -  \\
\multirow{11}{*}{\shortstack{QH9-dynamic\\ (300k-\texttt{geo})}} 
& QHNet$^*$&\ptz20M & \ptz88.36\ptpz{0.001}  & 1170.50\ptpz{0.001} & 93.65\ptpz{0.001}  & 23269.41\ptpz{0.001} & 2040.06\ptpz{0.001} & 22407.96\ptpz{0.001}\\
& WANet   &\ptz29M  & \ptz74.74\ptpz{0.001}  & \ptz416.57\ptpz{0.001}  & 99.68\ptpz{0.001} & - & - & -  \\
& SPHNet  &\ptz30M & \ptz52.18\ptpz{0.001}  & \ptz{100.88}\ptpz{0.001}  & 99.12\ptpz{0.001} & - & - & -  \\

%  & \textbf{QHFlow}     & \textbf{26.73}  & \ptz112.36  & \underline{99.59} & \ptz\ptz\underline{354.66} & \ptz\underline{204.34} & \ptz\ptz\underline{515.42}\\

\arrayrulecolor{lightgray}
\cmidrule(lr){2-9}
\arrayrulecolor{gray}

 & {QHFlow} &\ptz28M    & \ptz{25.94}\tpz{0.001}  & \ptz103.11\tpz{0.031}  & {99.59}\tpz{0.001} & \ptz\ptz{425.18}\tpz{1.119} & \ptz{175.18}\tpz{0.255} & \ptz\ptz{547.33}\tpz{1.168}\\

 
& {QHFlow (WA-FT)} &\ptz28M    & \ptz{27.12}\tpz{0.002}  & \ptz\ptz{89.03}\tpz{0.213}  & {99.65}\tpz{0.001} & \ptz\ptz{136.63}\tpz{4.661} & 
\ptz\ptz{84.17}\tpz{0.211} & \ptz\ptz{154.68}\tpz{4.449}  \\

\arrayrulecolor{lightgray}
\cmidrule(lr){2-9}
\arrayrulecolor{gray}

% & \textbf{eSCFlow}-tiny   & \ptz\ptz4M  & \ptz{-}\tpz{0.003}  & \ptz{-}\tpz{0.003}  & {-}\tpz{0.001} & \ptz\ptz{-}\tpz{7.452} & \ptz{-}\tpz{0.098} & \ptz\ptz{-}\tpz{7.454}  \\

& \textbf{eSCFlow}-small   & \ptz  12M  & \ptz{15.44}\tpz{0.003}  & \ptz\ptz{53.82}\tpz{0.003}  & {99.72}\tpz{0.001} & \ptz\ptz{430.13}\tpz{7.452} & \ptz\ptz{67.27}\tpz{0.098} & \ptz\ptz{447.54}\tpz{7.454}  \\

& \textbf{eSCFlow}-middle   & \ptz43M  & \ptz\ptz{8.70}\tpz{0.003}  & \ptz\ptz{42.51}\tpz{0.003}  & {99.89}\tpz{0.001} & \ptz\ptz{113.54}\tpz{7.452} & \ptz\ptz{51.80}\tpz{0.098} & \ptz\ptz{143.97}\tpz{7.454}  \\

& \textbf{eSCFlow}-large   & 183M  & \ptz\ptz{5.25}\tpz{0.003}  & \ptz\ptz{28.19}\tpz{0.003}  & {99.94}\tpz{0.001} & \ptz\ptz\ptz{88.76}\tpz{7.452} & \ptz\ptz{30.58}\tpz{0.098} & \ptz\ptz{101.68}\tpz{7.454}  \\

& \textbf{eSCFlow}-xlarge   & 990M  & \ptz\ptz\textbf{3.74}\tpz{0.003}  & \ptz\ptz\textbf{22.84}\tpz{0.003}  & \textbf{99.96}\tpz{0.001} & \ptz\ptz\ptz\textbf{44.35}\tpz{7.452} & \ptz\ptz\textbf{21.01}\tpz{0.098} & \ptz\ptz\ptz\textbf{50.57}\tpz{7.454}  \\


% & \textbf{QHFlow (WAD-FT)}     & \textbf{25.71}  & \ptz\ptz\textbf{79.55}  & \textbf{99.68} & \ptz\ptz\textbf{123.68} & \ptz\ptz\textbf{75.53} & \ptz\ptz\textbf{138.56}  \\
\midrule
% \cmidrule(lr){1-8}


%%%% 300k-mol
% \rowcolor{Gray}\cellcolor{white}
% & \texttt{1e} & \ptz\ptz0.08 & \ptz\ptz\ptz1.89 & 99.99 & \ptz\ptz\ptz\ptz1.22 & \ptz\ptz\ptz0.74 & \ptz\ptz\ptz\ptz1.19 \\
% & QHNet    & 120.10  & 2182.06  & 89.63 & - & - & - \\
\multirow{11}{*}{\shortstack{QH9-dynamic\\ (300k-\texttt{mol})}}
& QHNet$^*$&\ptz20M & 121.39\ptpz{0.001}  & 5554.36\ptpz{0.001}  & 86.02\ptpz{0.001} & 53505.09\ptpz{0.001}& 4352.76\ptpz{0.001} & 50424.86\ptpz{0.001} \\
& SPHNet   &\ptz30M & 108.19\ptpz{0.001}  & 1724.10\ptpz{0.001}  & 91.49\ptpz{0.001}  & - & - & -  \\

%  & \textbf{QHFlow}     & \ptz\underline{38.14}  & \ptz\underline{282.74}  & \underline{98.79} & \ptz\underline{1237.48} & \ptz\underline{316.78} & \ptz\underline{1403.95}  \\
\arrayrulecolor{lightgray}
\cmidrule(lr){2-9}
\arrayrulecolor{gray}

& {QHFlow} &\ptz28M     & \ptz{45.91}\tpz{0.001}  & \ptz{442.56}\tpz{0.171}  & {98.65}\tpz{0.001} & \ptz{1344.68}\tpz{2.338} & \ptz{479.71}\tpz{0.150} & \ptz{1605.03}\tpz{2.286}  \\

& {QHFlow (WA-FT)}  &\ptz28M    & \ptz{46.60}\tpz{0.003}  & \ptz{424.75}\tpz{0.324}  & {98.74}\tpz{0.001} & \ptz\ptz{912.10}\tpz{2.941} & \ptz{403.51}\tpz{1.861} & \ptz{1047.88}\tpz{2.683} \\

\arrayrulecolor{lightgray}
\cmidrule(lr){2-9}
\arrayrulecolor{gray}

% & \textbf{eSCFlow}-tiny   & \ptz\ptz4M  & \ptz{-}\tpz{0.003}  & \ptz{-}\tpz{0.003}  & {-}\tpz{0.001} & \ptz\ptz{-}\tpz{7.452} & \ptz{-}\tpz{0.098} & \ptz\ptz{-}\tpz{7.454}  \\

& \textbf{eSCFlow}-small   & \ptz  12M  & \ptz{29.68}\tpz{0.003}  & \ptz{261.32}\tpz{0.003}  & {99.22}\tpz{0.001} & \ptz\ptz{644.01}\tpz{7.452} & \ptz{263.24}\tpz{0.098} & \ptz\ptz{772.89}\tpz{7.454}  \\

& \textbf{eSCFlow}-middle   & \ptz43M  & \ptz{21.99}\tpz{0.003}  & \ptz{240.09}\tpz{0.003}  & {99.39}\tpz{0.001} & \ptz\ptz{378.78}\tpz{7.452} & \ptz{207.16}\tpz{0.098} & \ptz\ptz{468.62}\tpz{7.454}  \\

 & \textbf{eSCFlow}-large   & 183M  & \ptz{17.54}\tpz{0.003}  & \ptz{214.51}\tpz{0.003}  & {99.52}\tpz{0.001} & \ptz\ptz{261.68}\tpz{7.452} & \ptz{179.23}\tpz{0.098} & \ptz\ptz{324.99}\tpz{7.454}  \\

& \textbf{eSCFlow}-xlarge   & 990M  & \ptz\textbf{15.90}\tpz{0.003}  & \ptz\textbf{202.32}\tpz{0.003}  & \textbf{99.55}\tpz{0.001} & \ptz\ptz\textbf{219.52}\tpz{7.452} & \ptz\textbf{167.38}\tpz{0.098} & \ptz\ptz\textbf{278.06}\tpz{7.454}  \\


% & \textbf{QHFlow (WAD-FT)}     & \ptz\textbf{25.64}  & \ptz\textbf{111.21}  & \textbf{99.27} & \ptz\ptz\textbf{212.36} & \ptz\textbf{118.53} & \ptz\ptz\textbf{218.32} \\
\arrayrulecolor{black}
\bottomrule
\end{tabular}}
\vspace{-10pt}
\end{table}

% 0.46635
% 0.47034
% 0.49252
% 0.23689
% --
% 0.416525
% 0.583475

==> table/unuse/qh9_EF_old.tex <==
% 문서 상단(Preamble)에 이 패키지를 추가하세요
% \usepackage{siunitx}
% \usepackage{multirow}
% \usepackage{booktabs}
% \usepackage[table]{xcolor} % \cellcolor를 위해

\begin{table*}[t]
\centering
\caption{\textbf{QH9 benchmark.} Results shown in \textbf{bold} denote the best in each column, and the \underline{underlined} ones indicate the second best. Only (Pred $-$ Targ) metrics are reported.}
\label{tab:md17_results_predtarg}
% 테이블이 넓어졌으므로 \textwidth로 조정
\resizebox{\textwidth}{!}{
\sisetup{detect-all=true}
% S 컬럼 포맷을 데이터에 맞게 수정 (예: 1.3 -> 3.2, 5.5 -> 5.0, 3.4 -> 4.0)
\begin{tabular}{ll S[table-format=3.2] S[table-format=5.0] S[table-format=-4.3] S[table-format=4.0] S[table-format=-4.3]}
\toprule
\multirow{2}{*}{\textbf{Molecule}} & 
\multirow{2}{*}{\textbf{Metric (MAE)}} &
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Hamiltonian (meV)}}} &
% \multicolumn 범위를 4로 유지
\multicolumn{4}{c}{\textbf{(Pred $-$ Targ)}} \\
% \cmidrule 범위를 4-7로 유지, 헤더 순서 변경
\cmidrule(lr){4-7}
 & & & \multicolumn{1}{c}{\textbf{Energy (meV)}} & \multicolumn{1}{c}{\textbf{E. Reduc. (\%)}} & \multicolumn{1}{c}{\textbf{Force (meV/\AA)}} & \multicolumn{1}{c}{\textbf{F. Reduc. (\%)}} \\
\midrule

\multirow{7}{*}{Stable-iid} 
 % & DFT-variance & {-} & 0.00008 & {-} & 0.0491 & {-} \\
 & UMA-omol (MLFF) & {-} & 21484 & {0.000} & 359 & {0.000} \\
 & Equiformer (MLFF) & {-} & {-} & {-} & {-} & {-} \\
 & QHNet (DFT) & 107.84 & 7727 & -64.034 & 2946 & +720.613 \\ 
 & QHFlow (DFT) & \bfseries 23.06 &  \bfseries 52 & \bfseries -99.758 &  \bfseries 35 & \bfseries -90.251 \\
& \textbf{eSCFlow}-12M (DFT) & {-} & {23} & {-} & {41} & {-} \\
 & \textbf{eSCFlow}-183M (DFT) & {-} & {-} & {-} & {-} & {-} \\
 & \textbf{eSCFlow}-990M (DFT) & {-} & {-} & {-} & {-} & {-} \\
\midrule

\multirow{7}{*}{Stable-ood} 
 % & DFT-variance & {-} & 0.0002 & {-} & 0.088 & {-} \\
 & UMA-omol (MLFF) & {-} & 20295 & {0.000} & 289 & {0.000} \\
 % Equiformer를 기준으로 0.0 표기
 & Equiformer (MLFF) & {-} & {-} & {-} & {-} & {-} \\
 & QHNet (DFT) & 93.29 & 2806 & -86.174 & 611 & +111.419 \\
 & QHFlow (DFT) & \bfseries 19.64 & \bfseries 9 & \bfseries -99.956 & \bfseries 10 & \bfseries -96.540 \\
& \textbf{eSCFlow}-12M (DFT) & {-} & {-} & {-} & {-} & {-} \\
 & \textbf{eSCFlow}-183M (DFT) & {-} & {-} & {-} & {-} & {-} \\
 & \textbf{eSCFlow}-990M (DFT) & {-} & {-} & {-} & {-} & {-} \\
\midrule

\multirow{7}{*}{Dynamic-geo} 
 % & DFT-variance & {-} & 0.0004 & {-} & 0.1469 & {-} \\
 & UMA-omol (MLFF) & {-} & 21395 & {0.000} & 359 & {0.000} \\
 % Equiformer를 기준으로 0.0 표기
 & Equiformer (MLFF) & {-} & {-} & {-} & {-} & {-} \\
 & QHNet (DFT) & 118.02 & 8210 & -61.627 & 2807 & +681.894 \\
 & QHFlow (DFT) & \bfseries 26.56 & \bfseries 5 & \bfseries -99.977 & \bfseries 16 & \bfseries -95.543 \\
& \textbf{eSCFlow}-12M (DFT) & {-} & {-} & {-} & {-} & {-} \\
 & \textbf{eSCFlow}-183M (DFT) & {-} & {-} & {-} & {-} & {-} \\
 & \textbf{eSCFlow}-990M (DFT) & {-} & {-} & {-} & {-} & {-} \\
\midrule

\multirow{7}{*}{Dynamic-mol} 
 % & DFT-variance & {-} & 0.0004 & {-} & 0.2955 & {-} \\
 & UMA-omol (MLFF) & {-} & 20903 & {0.000} & 343 & {0.000} \\
 % Equiformer를 기준으로 0.0 표기
 & Equiformer (MLFF) & {-} & {-} & {-} & {-} & {-} \\
 & QHNet (DFT) & 142.40 & 13609 & -34.895 & 4683 & +1265.306 \\
 & QHFlow (DFT) & \bfseries 39.37 & \bfseries 31 & \bfseries -99.852 & \bfseries 28 & \bfseries -91.837 \\
& \textbf{eSCFlow}-12M (DFT) & {-} & {-} & {-} & {-} & {-} \\
 & \textbf{eSCFlow}-183M (DFT) & {-} & {-} & {-} & {-} & {-} \\
 & \textbf{eSCFlow}-990M (DFT) & {-} & {-} & {-} & {-} & {-} \\
\midrule

\multirow{7}{*}{\textbf{Average}} 
 & UMA-omol (MLFF) & {-} & 21019 & {0.000} & 338 & {0.000} \\
 & Equiformer (MLFF) & {-} & {-} & {-} & {-} & {-} \\
 & QHNet (DFT) & 115.39 & 8088 & -61.683 & 2762 & +694.808 \\ 
 & QHFlow (DFT) & \bfseries 27.16 &  \bfseries 24 & \bfseries -99.886 &  \bfseries 22 & \bfseries -93.543 \\
 & \textbf{eSCFlow}-12M (DFT) & {-} & {-} & {-} & {-} & {-} \\
 & \textbf{eSCFlow}-183M (DFT) & {-} & {-} & {-} & {-} & {-} \\
 & \textbf{eSCFlow}-990M (DFT) & {-} & {-} & {-} & {-} & {-} \\
\bottomrule
\end{tabular}
}
\end{table*}

==> table/unuse/qh9_distribution.tex <==
\begin{wraptable}{R}{5.4cm}
\vspace{-11.5pt}
\centering
\captionof{table}{\textbf{Effect of prior distribution.}}
\label{tab:qh9_dist}
\resizebox{\linewidth}{!}{ % Optional: resize if space is limited
\begin{tabular}{llccc}
\toprule
\textbf{Data} & \textbf{Prior} & $H \downarrow$ $[\mu E_h]$ & \OCC $\downarrow$ $[\mu E_h]$& \SC $\uparrow$ $[\%]$\\
% & &  & $[\mu E_h]$ & $[10^{-2}]$ \\
\midrule
\midrule
\arrayrulecolor{gray}
\multirow{2}{*}{\texttt{id }}
& GOE & 25.93 & 154.65 & 99.39 \\
& TE  & \textbf{22.95} & \textbf{119.61} & \textbf{99.51} \\

\midrule
\multirow{2}{*}{\texttt{ood}}
& GOE & 20.41 & \ptz{87.32} & 98.95 \\
& TE  &\textbf{20.01} & \ptz\textbf{84.54} & \textbf{99.04} \\

\midrule
\multirow{2}{*}{\texttt{geo}}
& GOE & 29.39 & 122.14 & 99.49 \\
& TE  &\textbf{25.94} & \textbf{103.11} & \textbf{99.59} \\

\midrule
\multirow{2}{*}{\texttt{mol}}
& GOE & 46.78 & \textbf{419.68} & 98.65 \\
& TE  & \textbf{45.91} & 442.56 & \textbf{98.65} \\
\arrayrulecolor{black}

\bottomrule
\end{tabular}
}
\vspace{-10pt}
\end{wraptable}

==> table/unuse/qh9_flow.tex <==
\begin{wraptable}{R}{6.0cm}
\vspace{-11.5pt}
\centering
\captionof{table}{\textbf{Comparing Flow-based loss (flow) and MAE+MSE (default).}}
\label{tab:qh9_flow}
\resizebox{\linewidth}{!}{ % Optional: resize if space is limited
\begin{tabular}{llcccc}
\toprule
\textbf{Dataset} & \textbf{Type}& Step & $H \downarrow$ $[\mu E_h]$ & \OCC $\downarrow$ $[\mu E_h]$ & \SC $\uparrow$ $[\%]$ \\
\midrule\midrule
& Default  &    & 35.85 & 213.45 & 98.89 \\
\RC& & & 22.96 & 119.62 & {99.51} \\
\RC\multirow{-3}{*}{\texttt{id}}& \multirow{-2}{*}{\textbf{Flow}}&\multirow{-2}{*}{\shortstack{1\\3}}& \textbf{22.95} & \textbf{118.98} & \textbf{99.50} \\
\midrule

& Default   &   & 30.24 & 138.99 & 98.30 \\
\RC& & & \textbf{20.01} & {84.07} & {99.05} \\
\RC\multirow{-3}{*}{\texttt{ood}}& \multirow{-2}{*}{\textbf{Flow}}&\multirow{-2}{*}{\shortstack{1\\3}}& \textbf{20.01} & \textbf{83.55} & \textbf{99.05} \\
\midrule

& Default  &    & 41.68 & 211.90 & 98.85 \\
\RC&  & & 25.95 & 103.26 & \textbf{99.59} \\
\RC\multirow{-3}{*}{\texttt{geo}}& \multirow{-2}{*}{\textbf{Flow}}&\multirow{-2}{*}{\shortstack{1\\3}}& \textbf{25.94} & \textbf{103.11} & \textbf{99.59} \\
\midrule

& Default   &   & 66.47 & 864.63 & 96.41 \\
\RC& & & \textbf{45.91} & \textbf{441.87} & \textbf{98.66} \\
\RC\multirow{-3}{*}{\texttt{mol}}& \multirow{-2}{*}{\textbf{Flow}}&\multirow{-2}{*}{\shortstack{1\\3}}& \textbf{45.91} & 442.56 & \textbf{98.66} \\
\bottomrule
\end{tabular}
}
\vspace{-10pt}
\end{wraptable}


% \begin{minipage}[t]{0.48\textwidth}
% \vspace{-6pt}
% \centering
% \captionof{table}{Results on QH9 along prior distribution.}
% \label{tab:qh9_dist}
% \resizebox{1.0\textwidth}{!}{ % Optional: resize if space is limited
% \begin{tabular}{llccc}
% \toprule
% \textbf{Prior} & \textbf{Split} & $H \downarrow$ $[\mu E_h]$ & \OCC $\downarrow$ $[\mu E_h]$& \SC $\uparrow$ $[10^{-2}]$\\
% % & &  & $[\mu E_h]$ & $[10^{-2}]$ \\
% \midrule
% \midrule
% \multirow{4}{*}{GOE}
% & id   & 23.44 & 123.73 & 99.48 \\
% & ood  & 20.41 & \ptz82.83 & 99.03 \\
% & geo & 26.73 & 112.36 & 99.59 \\
% & mol & 38.14 & \textbf{278.74} & 98.79 \\
% \midrule
% \multirow{4}{*}{\shortstack{Exps.}}
% & id   & \textbf{22.81} & \textbf{103.67} & \textbf{99.53} \\
% & ood  & \textbf{20.01} & \ptz84.53 & \textbf{99.04} \\
% & geo & \textbf{26.15} & \textbf{107.80} & \textbf{99.59} \\
% & mol & \textbf{36.90} & 278.88 & \textbf{98.87} \\
% \bottomrule
% \end{tabular}
% }
% \end{minipage}

==> table/unuse/qh9_flow3.tex <==
\begin{table}[h]
\centering
\caption{Experimental results on QH9 dataset.}
\label{tab:qh9_results}

\begin{tabular}{ccccccc}
\toprule
 & $H \downarrow$  & $\epsilon \downarrow$  & $\psi \uparrow$ & $H \downarrow$  & $\epsilon \downarrow$  & $\psi \uparrow$ \\
\textbf{Model} & [$10^{-6}E_h$] &  [$10^{-6}E_h$] &  [$10^{-2}$] &  [$10^{-6}E_h$] &  [$10^{-6}E_h$] &  [$10^{-2}$] \\
\midrule
% & QHNet    & 76.31  & 798.51  & 95.85 & - & - & - \\
QHNet$^*$& 77.72  & 963.45  & 94.80 & 18257.34 & 1546.27 & 17822.62 \\
WANet    & 80.00  & 833.62  & 96.86 & - & - & -  \\
SPHNet   & 45.48  & 334.28  & 97.75 & - & - & - \\
\rowcolor{lightorange} \textbf{Ours}     & \textbf{26.05}  & \textbf{158.62}  & \textbf{99.39} & \ptz\ptz\textbf{608.62} & \ptz\textbf{215.58} & \ptz\ptz\textbf{723.90} \\
\bottomrule
\end{tabular}
\end{table}

% \resizebox{\textwidth}{!}{
% }
% 0.42
% 0.49
% 0.30
% 0.51
% --
% 0.43

==> table/unuse/qh9_flow_full.tex <==
% \NewTableCommand\SCC[2]{\SetCell{bg=#1, fg=#2}}
% \NewTableCommand\cco{\SetCell{bg=lightorange}}
% \newcolumntype{s}{>{\columncolor{white}} c}
% \newcommand{\RC}{\rowcolor{lightorange}\cellcolor{white}}

% \rowcolor{lightorange}

\begin{table}[t]
\centering
\caption{Full experimental results of the advantage of flow matching on QH9 dataset. Results shown in \textbf{bold} denote the best result in each column.}
\label{tab:qh9_flow_full}
\resizebox{\textwidth}{!}{
\begin{tabular}{clccccccc}
\toprule
 & & \multirow{2}{*}{ODE Steps}  & $H \downarrow$  & \OCC $\downarrow$  & \SC $\uparrow$
 & \LUMO $\downarrow$ & \HOMO $\downarrow$ & \GAP $\downarrow$  \\
\textbf{Dataset} & \textbf{Type} &  & [$10^{-6}E_h$] &  [$10^{-6}E_h$] &  [$10^{-2}$] &  [$10^{-6}E_h$]  &  [$10^{-6}E_h$] &  [$10^{-6}E_h$]  \\

% Stable id
\midrule\midrule
& MAE + MSE &
- & 35.85  & 213.45  & 98.89 & 1548.62 & 330.77 & 1738.99\\

% GOE
% \RC &  &
% 1 & 23.45  & 124.74  & \textbf{99.48} & \ptz511.37 & \textbf{178.39} & \ptz 616.66 \\
% % \RC &  &
% % 2 & \textbf{26.05}  & 160.16  & \textbf{99.39} & \ptz{597.54} & 216.46 & \ptz\textbf{713.62} \\
% \RC \multirow{-3}{*}{\shortstack{QH9-stable \\ (id)}} & 
% \multirow{-2}{*}{\textbf{Flow}} &
% 3 & \textbf{23.44}  & \textbf{124.73}  & \textbf{99.48} & \ptz\textbf{505.63} & 181.13 & \ptz\textbf{612.53} \\

% Expand
\RC &  &
1 & 22.96  & 119.62  & {99.51} & \ptz{456.26} & \textbf{175.57} & \ptz{567.95} \\
% \RC &  &
% 2 & \textbf{26.05}  & 160.16  & \textbf{99.39} & \ptz{597.54} & 216.46 & \ptz\textbf{713.62} \\
\RC \multirow{-3}{*}{\shortstack{QH9-stable \\ (id)}} & 
\multirow{-2}{*}{\textbf{Flow (TE)}} &
3 & \textbf{22.95}  & \textbf{118.98}  & \textbf{99.50} & \ptz\textbf{433.97} & 179.43 & \ptz\textbf{549.80} \\

% Stable ood
\midrule
& MAE + MSE &
- & 30.24  & 138.99  & 98.30 & \ptz997.22 & 232.90 & 1085.13\\

% GOE
% \RC &  &
% 1 & 20.42  & \ptz\textbf{82.51}  & \textbf{99.03} & \ptz355.36 & \textbf{109.12} & \ptz 409.21 \\
% % \RC &  &
% % 2 & 22.06  & \ptz95.77  & 98.94 & \ptz\textbf{570.84} & 108.75 & \ptz\textbf{595.75} \\
% \RC \multirow{-3}{*}{\shortstack{QH9-stable \\ (ood)}} & 
% \multirow{-2}{*}{\textbf{Flow}} &
% 3 & \textbf{20.41}  & \ptz{82.83}  & \textbf{99.03} & \ptz\textbf{344.05} & {111.97} & \ptz\textbf{301.31} \\

% Expand
\RC &  &
1 & \textbf{20.01}  & \ptz{84.07}  & \textbf{99.05} & \ptz\textbf{313.79} & \textbf{126.48} & \ptz \textbf{380.02} \\
% \RC &  &
% 2 & 22.06  & \ptz95.77  & 98.94 & \ptz\textbf{570.84} & 108.75 & \ptz\textbf{595.75} \\
\RC \multirow{-3}{*}{\shortstack{QH9-stable \\ (ood)}} & 
\multirow{-2}{*}{\textbf{Flow (TE)}} &
3 & \textbf{20.01}  & \ptz\textbf{83.55}  & \textbf{99.05} & \ptz{320.04} & {130.73} & \ptz{394.63} \\

% 300k-geo
\midrule
& MAE + MSE &
- & 41.68  & 211.90  & 98.85 & 1539.41 & \ptz349.25 & 1734.73\\

% % GOE
% \RC &  &
% 1 & \textbf{26.73}  & \textbf{111.14}  & \textbf{99.59} & \ptz 364.91 & \ptz {197.49} & \ptz 518.65 \\
% % \RC &  &
% % 2 & 46.78  & 419.81  & 98.65 & 1424.02 & \ptz 479.15 & 1735.26 \\
% \RC \multirow{-3}{*}{\shortstack{QH9-dynamic\\ (300k-geo)}} & 
% \multirow{-2}{*}{\textbf{Flow}} &
% 3 & \textbf{26.73}  & {112.36}  & {99.59} & \ptz \textbf{354.66} & \ptz{205.34} & \ptz \textbf{515.43} \\

% expand
\RC &  &
1 & 25.95  & 103.26  & \textbf{99.59} & \ptz 431.64 & \ptz \textbf{171.81} & \ptz 549.73 \\
% \RC &  &
% 2 & 46.78  & 419.81  & 98.65 & 1424.02 & \ptz 479.15 & 1735.26 \\
\RC \multirow{-3}{*}{\shortstack{QH9-dynamic\\ (300k-geo)}} & 
\multirow{-2}{*}{\textbf{Flow (TE)}} &
3 & \textbf{25.94}  & \textbf{103.11}  & \textbf{99.59} & \ptz \textbf{427.66} & \ptz{175.22} & \ptz\textbf{549.82} \\


% 300k-mol
\midrule
& MAE + MSE &
- & 66.47  & 864.63  & 96.41 & 6780.18 & 1162.25 & 6502.34\\

% % GOE
% \RC &  &
% 1 & 38.16  & 283.55  & \textbf{98.78} & 1250.97 & \ptz {317.33} & 1416.25 \\
% % \RC &  &
% % 2 & 46.78  & 419.81  & 98.65 & 1424.02 & \ptz 479.15 & 1735.26 \\
% \RC \multirow{-3}{*}{\shortstack{QH9-dynamic\\ (300k-mol)}} & 
% \multirow{-2}{*}{\textbf{Flow}} &
% 3 & \textbf{38.14}  & \textbf{282.74}  & {98.79} & \textbf{1237.48} & \ptz\textbf{316.78} & \textbf{1403.95} \\


% expand
\RC &  &
1 & \textbf{45.91}  & \textbf{441.87}  & \textbf{98.66} & \textbf{1344.32} & \textbf{476.04} & \textbf{1603.14} \\
% \RC &  &
% 2 & 46.78  & 419.81  & 98.65 & 1424.02 & \ptz 479.15 & 1735.26 \\
\RC \multirow{-3}{*}{\shortstack{QH9-dynamic\\ (300k-mol)}} & 
\multirow{-2}{*}{\textbf{Flow (TE)}} &
3 & \textbf{45.91}  & {442.56}  & \textbf{98.66} & {1347.94} & \ptz{480.64} & {1608.32} \\


\bottomrule
\end{tabular}}
\end{table}

==> table/unuse/qh9_flow_small.tex <==
\begin{wraptable}{R}{5.5cm}
\vspace{-11.5pt}
\centering
\captionof{table}{\textbf{Ablation comparing flow-based loss and MAE+MSE (default).}}
\label{tab:qh9_flow}
\resizebox{\linewidth}{!}{ % Optional: resize if space is limited
\begin{tabular}{llccc}
\toprule
\textbf{Dataset} & \textbf{Type}& Step & $H \downarrow$ $[\mu E_h]$ & \OCC $\downarrow$ $[\mu E_h]$\\
\midrule\midrule
& Default  &    & 35.85 & 213.45 \\
\RC& & & 22.96 & 119.62  \\
\RC\multirow{-3}{*}{\texttt{id}}& \multirow{-2}{*}{\textbf{Flow}}&\multirow{-2}{*}{\shortstack{1\\3}}& \textbf{22.95} & \textbf{118.98} \\
\midrule

& Default   &   & 30.24 & 138.99 \\
\RC& & & \textbf{20.01} & {84.07} \\
\RC\multirow{-3}{*}{\texttt{ood}}& \multirow{-2}{*}{\textbf{Flow}}&\multirow{-2}{*}{\shortstack{1\\3}}& \textbf{20.01} & \textbf{83.55} \\
\midrule

& Default  &    & 41.68 & 211.90 \\
\RC&  & & 25.95 & 103.26  \\
\RC\multirow{-3}{*}{\texttt{geo}}& \multirow{-2}{*}{\textbf{Flow}}&\multirow{-2}{*}{\shortstack{1\\3}}& \textbf{25.94} & \textbf{103.11} \\
\midrule

& Default   &   & 66.47 & 864.63  \\
\RC& & & \textbf{45.91} & \textbf{441.87} \\
\RC\multirow{-3}{*}{\texttt{mol}}& \multirow{-2}{*}{\textbf{Flow}}&\multirow{-2}{*}{\shortstack{1\\3}}& \textbf{45.91} & 442.56  \\
\bottomrule
\end{tabular}
}
\vspace{-10pt}
\end{wraptable}


% \begin{minipage}[t]{0.48\textwidth}
% \vspace{-6pt}
% \centering
% \captionof{table}{Results on QH9 along prior distribution.}
% \label{tab:qh9_dist}
% \resizebox{1.0\textwidth}{!}{ % Optional: resize if space is limited
% \begin{tabular}{llccc}
% \toprule
% \textbf{Prior} & \textbf{Split} & $H \downarrow$ $[\mu E_h]$ & \OCC $\downarrow$ $[\mu E_h]$& \SC $\uparrow$ $[10^{-2}]$\\
% % & &  & $[\mu E_h]$ & $[10^{-2}]$ \\
% \midrule
% \midrule
% \multirow{4}{*}{GOE}
% & id   & 23.44 & 123.73 & 99.48 \\
% & ood  & 20.41 & \ptz82.83 & 99.03 \\
% & geo & 26.73 & 112.36 & 99.59 \\
% & mol & 38.14 & \textbf{278.74} & 98.79 \\
% \midrule
% \multirow{4}{*}{\shortstack{Exps.}}
% & id   & \textbf{22.81} & \textbf{103.67} & \textbf{99.53} \\
% & ood  & \textbf{20.01} & \ptz84.53 & \textbf{99.04} \\
% & geo & \textbf{26.15} & \textbf{107.80} & \textbf{99.59} \\
% & mol & \textbf{36.90} & 278.88 & \textbf{98.87} \\
% \bottomrule
% \end{tabular}
% }
% \end{minipage}

==> table/unuse/qh9_old.tex <==

\begin{table}[h]
\centering
\caption{Experimental results on QH9 dataset.}
\label{tab:qh9_results}
\resizebox{\textwidth}{!}{
\begin{tabular}{clccccccccc}
\toprule
 &  & $H \downarrow$  & $\epsilon \downarrow$  & $\psi \uparrow$ & LUMO $\downarrow$ & HOMO $\downarrow$ & GAP $\downarrow$ & SCF it Ratio $\downarrow$ & SCF T Ratio $\downarrow$ \\
\textbf{Dataset} & \textbf{Model} & [$10^{-6}E_h$] &  [$10^{-6}E_h$] &  [$10^{-2}$] &  [$10^{-6}E_h$]  &  [$10^{-6}E_h$] &  [$10^{-6}E_h$] & [$10^{-2}$] &  [$10^{-2}$] \\
\midrule

%%%% SIZE-iid
\rowcolor{Gray}\cellcolor{white}
& \texttt{1e} & \ptz0.10 & \ptz\ptz2.47& 99.99 & \ptz\ptz\ptz\ptz0.93 & \ptz\ptz\ptz1.57 & \ptz\ptz\ptz\ptz1.49 & 100.00 & 100.00 \\
% & QHNet    & 76.31  & 798.51  & 95.85 & - & - & - \\
& QHNet$^*$& 77.72  & 963.45  & 94.80 & 18257.34 & 1546.27 & 17822.62 & \ptz40.56 & \ptz53.46\\
& WANet    & 80.00  & 833.62  & 96.86 & - & - & - & - & - \\
& SPHNet   & 45.48  & 334.28  & 97.75 & - & - & - & - & - \\
\RC& \textbf{Ours}     & \textbf{26.05}  & \textbf{158.62}  & \textbf{99.39} & \ptz\ptz\textbf{608.62} & \ptz\textbf{215.58} & \ptz\ptz\textbf{723.90}  & \ptz\textbf{32.43} & \ptz\textbf{47.10}\\
\RC\multirow{-6}{*}{\shortstack{QH9-stable \\ (iid)}}
& \textbf{Ours (WAD-FT)}     &   &  &  &  &  & & &\\
\midrule

%%%% SIZE-OOD
\rowcolor{Gray}\cellcolor{white}
& \texttt{1e} & \ptz0.10 & \ptz\ptz2.47& 99.99 & \ptz\ptz\ptz\ptz0.93 & \ptz\ptz\ptz1.57 & \ptz\ptz\ptz\ptz1.49 & 100.00 & 100.00 \\
% & QHNet    & 72.11  & 644.17  & 93.68 & - & - & -  \\
& QHNet$^*$& 69.69  & 884.97  & 93.01 & 25848.83 & 1045.99 & 25370.10 & \ptz37.74 & \ptz52.83 \\
& SPHNet   & 43.33  & 186.40  & 98.16 & - & - & - & - & - \\
\RC& \textbf{Ours}     & \textbf{22.05}  & \ptz\underline{95.44}  & \underline{98.95} & \ptz\ptz\underline{589.08} & \ptz\underline{108.56} & \ptz\ptz\underline{614.84} & \ptz\textbf{30.30} & \ptz\textbf{46.80} \\
\RC\multirow{-5}{*}{\shortstack{QH9-stable \\ (ood)}} 
& \textbf{Ours (WAD-FT)}     & \underline{23.45}  & \ptz\textbf{77.33}  & \textbf{99.08} & \ptz\ptz\textbf{272.88} & \ptz\ptz\textbf{82.83} & \ptz\ptz\textbf{283.97} & \ptz\underline{30.85} & \ptz\underline{47.31} \\
\midrule

%%%% 300k-geo
\rowcolor{Gray}\cellcolor{white}
& \texttt{1e} & \ptz0.08 & \ptz\ptz\ptz1.89 & 99.99 & \ptz\ptz\ptz\ptz1.22 & \ptz\ptz\ptz0.74 & \ptz\ptz\ptz\ptz1.19 & 100.00 & 100.00 \\
% & QHNet    & 70.03  & \ptz408.31  & 97.60 & - & - & -  \\
& QHNet$^*$& 88.36  & 1170.50 & 93.65  & 23269.41 & 2040.06 & 22407.96 & \ptz41.39 & \ptz54.18\\
& WANet    & 74.74  & \ptz416.57  & 99.68 & - & - & - & - & - \\
& SPHNet   & 52.18  & \ptz\underline{100.88}  & 99.12 & - & - & - & - & - \\
\RC& \textbf{Ours}     & \textbf{29.63}  & \ptz128.77  & \underline{99.48} & \ptz\ptz\underline{639.80} & \ptz\underline{235.64} & \ptz\ptz\underline{791.24}  & \ptz\textbf{31.90} & \ptz\textbf{46.45}\\
\RC\multirow{-6}{*}{\shortstack{QH9-dynamic\\ (300k-geo)}}
& \textbf{Ours (WAD-FT)}     & \underline{31.33}  & \ptz\ptz\textbf{95.45}  & \textbf{99.59} & \ptz\ptz\textbf{150.42} & \ptz\ptz\textbf{86.64} & \ptz\ptz\textbf{170.62}  & \ptz\textbf{00.00} & \ptz\textbf{00.00}\\
\midrule

%%%% 300k-mol
\rowcolor{Gray}\cellcolor{white}
& \texttt{1e} & \ptz\ptz0.08 & \ptz\ptz\ptz1.89 & 99.99 & \ptz\ptz\ptz\ptz1.22 & \ptz\ptz\ptz0.74 & \ptz\ptz\ptz\ptz1.19 & 100.00 & 100.00 \\
% & QHNet    & 120.10  & 2182.06  & 89.63 & - & - & - \\
& QHNet$^*$& 121.39  & 5554.36  & 86.02 & 53505.09 & 4352.76 & 50424.86 & \ptz41.69 & \ptz55.38 \\
& SPHNet   & 108.19  & 1724.10 & 91.49  & - & - & - & - & - \\
\RC& \textbf{Ours}     & \ptz\underline{46.78}  & \ptz\underline{419.66}  & \underline{98.65} & \ptz\underline{1398.83} & \ptz\underline{477.79} & \ptz\underline{1709.58} & \ptz\textbf{31.52} & \ptz\textbf{47.30} \\
\RC\multirow{-5}{*}{\shortstack{QH9-dynamic\\ (300k-mol)}} 
& \textbf{Ours (WAD-FT)}     & \ptz\textbf{40.71}  & \ptz\textbf{260.39}  & \textbf{98.93} & \ptz\ptz\textbf{449.00} & \ptz\textbf{230.84} & \ptz\ptz\textbf{475.22} & \ptz\underline{31.82} & \ptz\underline{47.78} \\


\bottomrule
\end{tabular}}
\end{table}

% 0.42
% 0.49
% 0.30
% 0.51
% --
% 0.43

==> table/unuse/qh9_old2.tex <==

\begin{table}[t]
\centering
\caption{\textbf{QH9 benchmark.} WA-FT implies finetuned model with WAloss. Results shown in \textbf{bold} denote the best result in each column, whereas those that are \underline{underlined} indicate the second best.}
\label{tab:qh9_results}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{clccccccc}
\toprule
 % &  & $H$  $\downarrow$  & \OCC~ $\downarrow$  & \SC~ $\uparrow$ &
 % \LUMO~  $\downarrow$ & \HOMO~ $\downarrow$ & \GAP~$\downarrow$  \\

 % \textbf{Dataset} & \textbf{Model} & [$\mu E_h$]   & [$\mu E_h$]  & [$\%$]  &
 % [$\mu E_h$]  & [$\mu E_h$] & [$\mu E_h$] \\
 
  \textbf{Dataset} & \textbf{Model} &  \textbf{Param.} & $H$  $\downarrow$ [$\mu E_h$]  & \OCC~ $\downarrow$ [$\mu E_h$]  & \SC~ $\uparrow$ [$\%$] &
 \LUMO~  $\downarrow$ [$\mu E_h$] & \HOMO~ $\downarrow$ [$\mu E_h$] & \GAP~$\downarrow$  [$\mu E_h$] \\


\midrule
\midrule
\arrayrulecolor{gray}

%%%% SIZE-id
% \rowcolor{Gray}\cellcolor{white}
% & \texttt{1e} & \ptz0.10 & \ptz\ptz2.47& 99.99 & \ptz\ptz\ptz\ptz0.93 & \ptz\ptz\ptz1.57 & \ptz\ptz\ptz\ptz1.49 \\
% & QHNet    & 76.31  & 798.51  & 95.85 & - & - & - \\
& QHNet$^*$& \ptz30M & \ptz77.72\ptpz{0.001}  & \ptz963.45\ptpz{0.001}  & 94.80\ptpz{0.001} & 18257.34\ptpz{0.001} & 1546.27\ptpz{0.001} & 17822.62\ptpz{0.001} \\
& WANet    & \ptz30M & \ptz80.00\ptpz{0.001}  & \ptz833.62\ptpz{0.001}  & 96.86\ptpz{0.001} & - & - & -  \\
& SPHNet   & \ptz30M & \ptz45.48\ptpz{0.001}  & \ptz334.28\ptpz{0.001}  & 97.75\ptpz{0.001} & - & - & -  \\


% \RC& \textbf{QHFlow}     & \textbf{23.44}  & \underline{123.73}  & \underline{99.48} & \ptz\ptz\underline{505.63} & \ptz\underline{181.13} & \ptz\ptz\underline{612.53}  \\
\arrayrulecolor{lightgray}
\cmidrule(lr){2-9}
\arrayrulecolor{gray}

\RC& {QHFlow}   & \ptz30M  & \ptz{22.95}\tpz{0.001}  & \ptz{119.67}\tpz{0.211}  & {99.51}\tpz{0.001} & \ptz\ptz{437.96}\tpz{7.452} & \ptz{179.48}\tpz{0.098} & \ptz\ptz{553.87}\tpz{7.454}  \\

\RC\multirow{-1}{*}{\shortstack{QH9-stable \\ (\texttt{id})}}
& {QHFlow (WA-FT)} & \ptz30M  & \ptz{23.85}\tpz{0.003}  &  \ptz{101.92}\tpz{0.279}  &   {99.56}\tpz{0.002} & \ptz\ptz{187.48}\tpz{6.434} & \ptz\ptz{92.22}\tpz{0.234}  & \ptz\ptz{206.15}\tpz{6.197} \\

\arrayrulecolor{lightgray}
\cmidrule(lr){2-9}
\arrayrulecolor{gray}

& {QHFlow-v2-small (old)}   & \ptz30M  & \ptz{28.52}\tpz{0.003}  & \ptz{162.10}\tpz{0.003}  & {99.55}\tpz{0.001} & \ptz\ptz{629.16}\tpz{7.452} & \ptz{240.26}\tpz{0.098} & \ptz\ptz{818.47}\tpz{7.454}  \\

& {QHFlow-v2-small-EF (old)}   & \ptz30M  & \ptz{28.30}\tpz{0.003}  & \ptz{122.07}\tpz{0.003}  & {99.57}\tpz{0.001} & \ptz\ptz{618.47}\tpz{7.452} & \ptz{235.27}\tpz{0.098} & \ptz\ptz{800.04}\tpz{7.454}  \\

& {QHFlow-v2-large (old)}   & 130M  & \ptz{16.89}\tpz{0.003}  & \ptz\ptz{59.72}\tpz{0.003}  & {99.72}\tpz{0.001} & \ptz\ptz{247.17}\tpz{7.452} & \ptz{114.72}\tpz{0.098} & \ptz\ptz{327.39}\tpz{7.454}  \\

& \textbf{QHFlow-v3-large (new)}   & 183M  & \ptz\ptz\textbf{5.93}\tpz{0.003}  & \ptz\ptz\textbf{45.73}\tpz{0.003}  & \textbf{99.81}\tpz{0.001} & \ptz\ptz\textbf{103.32}\tpz{7.452} & \ptz\ptz\textbf{50.50}\tpz{0.098} & \ptz\ptz\textbf{119.62}\tpz{7.454}  \\
\arrayrulecolor{lightgray}
\cmidrule(lr){2-9}
\arrayrulecolor{gray}
& {QHFlow-v3-large (no init)}   & 183M  & \ptz{16.22}\tpz{0.003}  & \ptz{150.04}\tpz{0.003}  & {99.52}\tpz{0.001} & \ptz\ptz{794.71}\tpz{7.452} & \ptz{109.16}\tpz{0.098} & \ptz\ptz{825.32}\tpz{7.454}  \\
% & \textbf{QHFlow (WDA-FT)}  & \textbf{21.23}  &  \ptz\ptz\textbf{71.75}  &   \textbf{99.65} & \ptz\ptz\textbf{135.08} & \ptz\ptz\textbf{70.50}  & \ptz\ptz\textbf{148.34}  \\
\midrule
% \cmidrule(lr){1-8}



%%%% SIZE-OOD
% \rowcolor{Gray}\cellcolor{white}
% & \texttt{1e} & \ptz0.10 & \ptz\ptz2.47& 99.99 & \ptz\ptz\ptz\ptz0.93 & \ptz\ptz\ptz1.57 & \ptz\ptz\ptz\ptz1.49 \\
% & QHNet    & 72.11  & 644.17  & 93.68 & - & - & -  \\
& QHNet$^*$ &\ptz30M &  \ptz69.69\ptpz{0.001}  & \ptz884.97\ptpz{0.001}  & 93.01\ptpz{0.001} & 25848.83\ptpz{0.001} & 1045.99\ptpz{0.001} & 25370.10\ptpz{0.001}  \\
& SPHNet  &~30M  & \ptz43.33\ptpz{0.001}  & \ptz186.40\ptpz{0.001}  & 98.16\ptpz{0.001} & - & - & -  \\

% \RC& \textbf{QHFlow}     & \textbf{20.41}  & \ptz\underline{82.83}  & \underline{99.03} & \ptz\ptz\underline{344.05} & \ptz\underline{111.97} & \ptz\ptz\underline{301.31} \\
\arrayrulecolor{lightgray}
\cmidrule(lr){2-9}
\arrayrulecolor{gray}

\RC& QHFlow   &\ptz30M  & \ptz{20.01}\tpz{0.001}  & \ptz\ptz{84.54}\tpz{0.007}  & {99.04}\tpz{0.003} & \ptz\ptz{321.20}\tpz{1.497} & \ptz{130.74}\tpz{0.043} & \ptz\ptz{395.83}\tpz{1.510} \\

\RC
& QHFlow (WA-FT)   &\ptz30M  & \ptz{20.55}\tpz{0.002}  & \ptz\ptz{72.64}\tpz{0.018}  & {99.16}\tpz{0.006} & \ptz\ptz{171.24}\tpz{0.273} & \ptz\ptz{77.96}\tpz{0.095} & \ptz\ptz{179.57}\tpz{0.271} \\


\arrayrulecolor{lightgray}
\cmidrule(lr){2-9}
\arrayrulecolor{gray}

\RC& {QHFlow-v2-small}   & \ptz30M  & \ptz{24.66}\tpz{0.003}  & \ptz\ptz{60.78}\tpz{0.003}  & {99.34}\tpz{0.001} & \ptz\ptz{354.53}\tpz{7.452} & \ptz{128.33}\tpz{0.098} & \ptz\ptz{442.06}\tpz{7.454}  \\

\multirow{-6}{*}{\shortstack{QH9-stable \\ (\texttt{ood})}} & \textbf{QHFlow-v3-large (new)}   & 183M  & \ptz\ptz\textbf{5.18}\tpz{0.003}  & \ptz\ptz\textbf{31.86}\tpz{0.003}  & \textbf{99.65}\tpz{0.001} & \ptz\ptz\ptz\textbf{98.98}\tpz{7.452} & \ptz\ptz\textbf{33.69}\tpz{7.454} & \ptz\ptz\textbf{105.87}\tpz{0.098}    \\

% & \textbf{QHFlow (WAD-FT)}     & \underline{20.36}  & \ptz\ptz\textbf{70.30}  & \textbf{99.19} & \ptz\ptz\textbf{177.67} & \ptz\ptz\textbf{74.92} & \ptz\ptz\textbf{184.86} \\
\midrule
% \cmidrule(lr){1-8}

% %%%% 300k-geo
% \rowcolor{Gray}\cellcolor{white}
% & \texttt{1e} & \ptz0.08 & \ptz\ptz\ptz1.89 & 99.99 & \ptz\ptz\ptz\ptz1.22 & \ptz\ptz\ptz0.74 & \ptz\ptz\ptz\ptz1.19 \\
% & QHNet    & 70.03  & \ptz408.31  & 97.60 & - & - & -  \\
& QHNet$^*$&\ptz30M & \ptz88.36\ptpz{0.001}  & 1170.50\ptpz{0.001} & 93.65\ptpz{0.001}  & 23269.41\ptpz{0.001} & 2040.06\ptpz{0.001} & 22407.96\ptpz{0.001}\\
& WANet   &\ptz30M  & \ptz74.74\ptpz{0.001}  & \ptz416.57\ptpz{0.001}  & 99.68\ptpz{0.001} & - & - & -  \\
& SPHNet  &\ptz30M & \ptz52.18\ptpz{0.001}  & \ptz{100.88}\ptpz{0.001}  & 99.12\ptpz{0.001} & - & - & -  \\

% \RC& \textbf{QHFlow}     & \textbf{26.73}  & \ptz112.36  & \underline{99.59} & \ptz\ptz\underline{354.66} & \ptz\underline{204.34} & \ptz\ptz\underline{515.42}\\

\arrayrulecolor{lightgray}
\cmidrule(lr){2-9}
\arrayrulecolor{gray}

\RC& {QHFlow} &\ptz30M    & \ptz{25.94}\tpz{0.001}  & \ptz103.11\tpz{0.031}  & {99.59}\tpz{0.001} & \ptz\ptz{425.18}\tpz{1.119} & \ptz{175.18}\tpz{0.255} & \ptz\ptz{547.33}\tpz{1.168}\\

\RC
& {QHFlow (WA-FT)} &\ptz30M    & \ptz{27.12}\tpz{0.002}  & \ptz\ptz{89.03}\tpz{0.213}  & {99.65}\tpz{0.001} & \ptz\ptz{136.63}\tpz{4.661} & 
\ptz\ptz{84.17}\tpz{0.211} & \ptz\ptz{154.68}\tpz{4.449}  \\

\arrayrulecolor{lightgray}
\cmidrule(lr){2-9}
\arrayrulecolor{gray}

\RC& {QHFlow-v2-large}   & 130M  & \ptz{16.46}\tpz{0.003}  & \ptz\ptz{40.31}\tpz{0.003}  & {99.88}\tpz{0.001} & \ptz\ptz{181.54}\tpz{7.452} & \ptz\ptz{74.65}\tpz{0.098} & \ptz\ptz{237.66}\tpz{7.454}  \\

\multirow{-8}{*}{\shortstack{QH9-dynamic\\ (300k-\texttt{geo})}} & \textbf{QHFlow-v3-large (new)}   & 183M  & \ptz\ptz\textbf{5.25}\tpz{0.003}  & \ptz\ptz\textbf{28.19}\tpz{0.003}  & \textbf{99.94}\tpz{0.001} & \ptz\ptz\ptz\textbf{88.76}\tpz{7.452} & \ptz\ptz\textbf{30.58}\tpz{0.098} & \ptz\ptz\textbf{101.68}\tpz{7.454}  \\

% & \textbf{QHFlow (WAD-FT)}     & \textbf{25.71}  & \ptz\ptz\textbf{79.55}  & \textbf{99.68} & \ptz\ptz\textbf{123.68} & \ptz\ptz\textbf{75.53} & \ptz\ptz\textbf{138.56}  \\
\midrule
% \cmidrule(lr){1-8}


%%%% 300k-mol
% \rowcolor{Gray}\cellcolor{white}
% & \texttt{1e} & \ptz\ptz0.08 & \ptz\ptz\ptz1.89 & 99.99 & \ptz\ptz\ptz\ptz1.22 & \ptz\ptz\ptz0.74 & \ptz\ptz\ptz\ptz1.19 \\
% & QHNet    & 120.10  & 2182.06  & 89.63 & - & - & - \\
& QHNet$^*$&\ptz30M & 121.39\ptpz{0.001}  & 5554.36\ptpz{0.001}  & 86.02\ptpz{0.001} & 53505.09\ptpz{0.001}& 4352.76\ptpz{0.001} & 50424.86\ptpz{0.001} \\
& SPHNet   &\ptz30M & 108.19\ptpz{0.001}  & 1724.10\ptpz{0.001}  & 91.49\ptpz{0.001}  & - & - & -  \\

% \RC& \textbf{QHFlow}     & \ptz\underline{38.14}  & \ptz\underline{282.74}  & \underline{98.79} & \ptz\underline{1237.48} & \ptz\underline{316.78} & \ptz\underline{1403.95}  \\
\arrayrulecolor{lightgray}
\cmidrule(lr){2-9}
\arrayrulecolor{gray}

\RC& {QHFlow} &\ptz30M     & \ptz{45.91}\tpz{0.001}  & \ptz{442.56}\tpz{0.171}  & {98.65}\tpz{0.001} & \ptz{1344.68}\tpz{2.338} & \ptz{479.71}\tpz{0.150} & \ptz{1605.03}\tpz{2.286}  \\

\RC & {QHFlow (WA-FT)}  &\ptz30M    & \ptz{46.60}\tpz{0.003}  & \ptz{424.75}\tpz{0.324}  & {98.74}\tpz{0.001} & \ptz\ptz{912.10}\tpz{2.941} & \ptz{403.51}\tpz{1.861} & \ptz{1047.88}\tpz{2.683} \\

\arrayrulecolor{lightgray}
\cmidrule(lr){2-9}
\arrayrulecolor{gray}

\RC& {QHFlow-v2-small}   & \ptz30M  & \ptz{51.88}\tpz{0.003}  & \ptz{307.61}\tpz{0.003}  & {98.72}\tpz{0.001} & \ptz{1913.77}\tpz{7.452} & \ptz{452.72}\tpz{0.098} & \ptz{2165.11}\tpz{7.454}  \\

\multirow{-7}{*}{\shortstack{QH9-dynamic\\ (300k-\texttt{mol})}} & \textbf{QHFlow-v3-large (new)}   & 183M  & \ptz\textbf{17.54}\tpz{0.003}  & \ptz\textbf{214.51}\tpz{0.003}  & \textbf{99.52}\tpz{0.001} & \ptz\ptz\textbf{261.68}\tpz{7.452} & \ptz\textbf{179.23}\tpz{0.098} & \ptz\ptz\textbf{324.99}\tpz{7.454}  \\


% & \textbf{QHFlow (WAD-FT)}     & \ptz\textbf{25.64}  & \ptz\textbf{111.21}  & \textbf{99.27} & \ptz\ptz\textbf{212.36} & \ptz\textbf{118.53} & \ptz\ptz\textbf{218.32} \\
\arrayrulecolor{black}
\bottomrule
\end{tabular}}
\vspace{-10pt}
\end{table}

% 0.46635
% 0.47034
% 0.49252
% 0.23689
% --
% 0.416525
% 0.583475

==> table/unuse/qh9_scf_time.tex <==
% \NewTableCommand\SCC[2]{\SetCell{bg=#1, fg=#2}}
% \NewTableCommand\cco{\SetCell{bg=lightorange}}
% \newcolumntype{s}{>{\columncolor{white}} c}
% \newcommand{\RC}{\rowcolor{lightorange}\cellcolor{white}}

% \rowcolor{lightorange}

\begin{table}[h]
\centering
\caption{Experimental results of SCF time on  300 samples from QH9 test dataset.}
\label{tab:qh9_scf_time}
\resizebox{\textwidth}{!}{
\begin{tabular}{clcccc}
\toprule

 &  & SCF \texttt{iter} Ratio $\downarrow$  & SCF \texttt{T} Ratio $\downarrow$ & Inf \texttt{T} Ratio $\downarrow$ & Total \texttt{T} Ratio $\downarrow$ \\
 
\textbf{Dataset} & \textbf{Model}  & [$10^{-2}$]  &  [$10^{-2}$] &  [$10^{-2}$] &  [$10^{-2}$] \\


% Stable id
\midrule\midrule
\rowcolor{Gray}\cellcolor{white}
& \texttt{minao}  & 100.00 & 100.00 & - & 100.00 \\
& QHNet$^*$   & \ptz40.56 & \ptz52.96  & \textbf{0.50} &\ptz53.46\\

% \RC &  &
%  \ptz{32.09} & \ptz{46.71} & \textbf{0.36} & \ptz{46.75} \\

\RC & \multirow{-1}{*}{\textbf{Ours}}&
 \ptz{\textbf{31.69}} & \ptz\textbf{45.45} & 0.83 & \ptz\textbf{46.28} \\

% \RC &  &
%  - & - & - & - \\

\RC \multirow{-4}{*}{\shortstack{QH9-stable \\ (id)}} &
\multirow{-1}{*}{\textbf{Ours (WAD-FT)}} &
 \ptz32.08 & \ptz45.95 & 0.91 & \ptz46.86 \\

% % Stable ood
\midrule
\rowcolor{Gray}\cellcolor{white}
& \texttt{minao}  & 100.00 & 100.00 & - & 100.00 \\
& QHNet$^*$   & \ptz37.74 & \ptz52.41  & \textbf{0.42} &\ptz52.83\\

% \RC &  &
%  \ptz{30.28} & \ptz{46.38} & \textbf{0.29} & \ptz\textbf{46.67} \\

\RC & \multirow{-1}{*}{\textbf{Ours}}&
 \ptz\textbf{30.25} & \ptz\textbf{45.77} & 0.66 & \ptz\textbf{46.43} \\

% \RC &  &
%  - & - & - & - \\

\RC \multirow{-4}{*}{\shortstack{QH9-stable \\ (ood)}} &
\multirow{-1}{*}{\textbf{Ours (WAD-FT)}} &
 \ptz30.81 & \ptz46.57 & 0.74 & \ptz47.32 \\


% % 300k-geo
\midrule
\rowcolor{Gray}\cellcolor{white}
& \texttt{minao} & 100.00 & 100.00 & - & 100.00 \\
& QHNet$^*$  & \ptz41.39 & \ptz53.71  & \textbf{0.47} &\ptz54.18\\

% \RC &  &
%  \ptz{32.21} & \ptz{47.08} & \textbf{0.28} & \ptz{47.36} \\

\RC & \multirow{-1}{*}{\textbf{Ours}}&
 \ptz\textbf{31.53} & \ptz\textbf{45.31} & 0.84 & \ptz\textbf{46.15} \\

% \RC &  &
%  - & - & - & - \\

\RC \multirow{-4}{*}{\shortstack{QH9-dynamic \\ (300k-geo)}} &
\multirow{-1}{*}{\textbf{Ours (WAD-FT)}} &
 \ptz 31.95 & \ptz45.73 & 0.88 & \ptz 46.61 \\


% % 300k-mol
\midrule
\rowcolor{Gray}\cellcolor{white}
& \texttt{minao}  & 100.00 & 100.00 & - & 100.00 \\
& QHNet$^*$   & \ptz41.69 & \ptz54.94  & \textbf{0.44} &\ptz55.38\\

% \RC &  &
% 1 & \ptz{32.21} & \ptz{47.08} & \textbf{0.28} & \ptz{47.36} \\

\RC & \multirow{-1}{*}{\textbf{Ours}}&
 \ptz\textbf{30.89} & \ptz\textbf{46.40} & 0.73 & \ptz{47.13} \\

% \RC &  &
% 1 & - & - & - & - \\

\RC \multirow{-4}{*}{\shortstack{QH9-dynamic \\ (300k-mol)}} &
\multirow{-1}{*}{\textbf{Ours (WAD-FT)}} &
 \ptz30.97 & \ptz 45.65 & 0.69 & \ptz\textbf{46.34} \\
\bottomrule
\end{tabular}}
\end{table}

==> table/unuse/qh9_variance.tex <==

\begin{table}[t]
\centering
\caption{{Full predictive variance results on QH9 dataset.} WA-FT implies the finetune the model with WA loss. Metrics for Ours and Ours (WA‑FT) are \texttt{means}$\pm$\texttt{std} over five random seeds. Results shown in \textbf{bold} denote the best result in each column, whereas those that are \underline{underlined} indicate the second best.}
\label{tab:qh9_variance}
\resizebox{\textwidth}{!}{
\begin{tabular}{clcccccc}
\toprule
%  &  & $H \downarrow$  & \OCC $\downarrow$  & \SC $\uparrow$ &
%  \LUMO  $\downarrow$ & \HOMO $\downarrow$ & \GAP $\downarrow$  \\
% \textbf{Dataset} & \textbf{Model} & [$\mu E_h$] &  [$\mu E_h$] &  [$\%$] &  [$\mu E_h$]  &  [$\mu E_h$] &  [$\mu E_h$] \\

 \textbf{Dataset} & \textbf{Model} & $H$ [$\mu E_h$] $\downarrow$  & \OCC~[$\mu E_h$] $\downarrow$  & \SC~[$\%$] $\uparrow$ &
 \LUMO~[$\mu E_h$]  $\downarrow$ & \HOMO~[$\mu E_h$] $\downarrow$ & \GAP~[$\mu E_h$] $\downarrow$  \\


\midrule
\midrule

%%%% SIZE-id
% \rowcolor{Gray}\cellcolor{white}
% & \texttt{1e} & \ptz0.10 & \ptz\ptz2.47& 99.99 & \ptz\ptz\ptz\ptz0.93 & \ptz\ptz\ptz1.57 & \ptz\ptz\ptz\ptz1.49 \\
% & QHNet    & 76.31  & 798.51  & 95.85 & - & - & - \\
& QHNet$^*$& \ptz77.72\ptp{0.001}  & \ptz963.45\ptp{0.001}  & 94.80\ptp{0.001} & 18257.34\ptp{0.001} & 1546.27\ptp{0.001} & 17822.62\ptp{0.001} \\
& WANet    & \ptz80.00\ptp{0.001}  & \ptz833.62\ptp{0.001}  & 96.86\ptp{0.001} & - & - & -  \\
& SPHNet   & \ptz45.48\ptp{0.001}  & \ptz334.28\ptp{0.001}  & 97.75\ptp{0.001} & - & - & -  \\


% \RC& \textbf{Ours}     & \textbf{23.44}  & \underline{123.73}  & \underline{99.48} & \ptz\ptz\underline{505.63} & \ptz\underline{181.13} & \ptz\ptz\underline{612.53}  \\

\RC& \textbf{Ours}     & \ptz\textbf{22.95}\tp{0.001}  & \ptz\underline{119.67}\tp{0.211}  & \underline{99.51}\tp{0.001} & \ptz\ptz\underline{437.96}\tp{7.452} & \ptz\underline{179.48}\tp{0.098} & \ptz\ptz\underline{553.87}\tp{7.454}  \\

\RC\multirow{-5}{*}{\shortstack{QH9-stable \\ (\texttt{id})}}
& \textbf{Ours (WA-FT)}  & \ptz\underline{23.85}\tp{0.003}  &  \ptz\textbf{101.92}\tp{0.279}  &   \textbf{99.56}\tp{0.002} & \ptz\ptz\textbf{187.48}\tp{6.434} & \ptz\ptz\textbf{92.22}\tp{0.234}  & \ptz\ptz\textbf{206.15}\tp{6.197} \\

% & \textbf{Ours (WDA-FT)}  & \textbf{21.23}  &  \ptz\ptz\textbf{71.75}  &   \textbf{99.65} & \ptz\ptz\textbf{135.08} & \ptz\ptz\textbf{70.50}  & \ptz\ptz\textbf{148.34}  \\

\midrule



%%%% SIZE-OOD
% \rowcolor{Gray}\cellcolor{white}
% & \texttt{1e} & \ptz0.10 & \ptz\ptz2.47& 99.99 & \ptz\ptz\ptz\ptz0.93 & \ptz\ptz\ptz1.57 & \ptz\ptz\ptz\ptz1.49 \\
% & QHNet    & 72.11  & 644.17  & 93.68 & - & - & -  \\
& QHNet$^*$& \ptz69.69\ptp{0.001}  & \ptz884.97\ptp{0.001}  & 93.01\ptp{0.001} & 25848.83\ptp{0.001} & 1045.99\ptp{0.001} & 25370.10\ptp{0.001}  \\
& SPHNet   & \ptz43.33\ptp{0.001}  & \ptz186.40\ptp{0.001}  & 98.16\ptp{0.001} & - & - & -  \\

% \RC& \textbf{Ours}     & \textbf{20.41}  & \ptz\underline{82.83}  & \underline{99.03} & \ptz\ptz\underline{344.05} & \ptz\underline{111.97} & \ptz\ptz\underline{301.31} \\

\RC& \textbf{Ours}     & \ptz\textbf{20.01}\tp{0.001}  & \ptz\ptz\underline{84.54}\tp{0.007}  & \underline{99.04}\tp{0.003} & \ptz\ptz\underline{321.20}\tp{1.497} & \ptz\underline{130.74}\tp{0.043} & \ptz\ptz\underline{395.83}\tp{1.510} \\

\RC\multirow{-4}{*}{\shortstack{QH9-stable \\ (\texttt{ood})}} 
& \textbf{Ours (WA-FT)}     & \ptz\underline{20.55}\tp{0.002}  & \ptz\ptz\textbf{72.64}\tp{0.018}  & \textbf{99.16}\tp{0.006} & \ptz\ptz\textbf{171.24}\tp{0.273} & \ptz\ptz\textbf{77.96}\tp{0.095} & \ptz\ptz\textbf{179.57}\tp{0.271} \\

% & \textbf{Ours (WAD-FT)}     & \underline{20.36}  & \ptz\ptz\textbf{70.30}  & \textbf{99.19} & \ptz\ptz\textbf{177.67} & \ptz\ptz\textbf{74.92} & \ptz\ptz\textbf{184.86} \\
\midrule

% %%%% 300k-geo
% \rowcolor{Gray}\cellcolor{white}
% & \texttt{1e} & \ptz0.08 & \ptz\ptz\ptz1.89 & 99.99 & \ptz\ptz\ptz\ptz1.22 & \ptz\ptz\ptz0.74 & \ptz\ptz\ptz\ptz1.19 \\
% & QHNet    & 70.03  & \ptz408.31  & 97.60 & - & - & -  \\
& QHNet$^*$& \ptz88.36\ptp{0.001}  & 1170.50\ptp{0.001} & 93.65\ptp{0.001}  & 23269.41\ptp{0.001} & 2040.06\ptp{0.001} & 22407.96\ptp{0.001}\\
& WANet    & \ptz74.74\ptp{0.001}  & \ptz416.57\ptp{0.001}  & 99.68\ptp{0.001} & - & - & -  \\
& SPHNet   & \ptz52.18\ptp{0.001}  & \ptz\underline{100.88}\ptp{0.001}  & 99.12\ptp{0.001} & - & - & -  \\

% \RC& \textbf{Ours}     & \textbf{26.73}  & \ptz112.36  & \underline{99.59} & \ptz\ptz\underline{354.66} & \ptz\underline{204.34} & \ptz\ptz\underline{515.42}\\

\RC& \textbf{Ours}     & \ptz\textbf{25.94}\tp{0.001}  & \ptz103.11\tp{0.031}  & \underline{99.59}\tp{0.001} & \ptz\ptz\underline{425.18}\tp{1.119} & \ptz\underline{175.18}\tp{0.255} & \ptz\ptz\underline{547.33}\tp{1.168}\\

\RC\multirow{-5}{*}{\shortstack{QH9-dynamic\\ (300k-\texttt{geo})}}
& \textbf{Ours (WA-FT)}     & \ptz\underline{27.12}\tp{0.002}  & \ptz\ptz\textbf{89.03}\tp{0.213}  & \textbf{99.65}\tp{0.001} & \ptz\ptz\textbf{136.63}\tp{4.661} & \ptz\ptz\textbf{84.17}\tp{0.211} & \ptz\ptz\textbf{154.68}\tp{4.449}  \\

% & \textbf{Ours (WAD-FT)}     & \textbf{25.71}  & \ptz\ptz\textbf{79.55}  & \textbf{99.68} & \ptz\ptz\textbf{123.68} & \ptz\ptz\textbf{75.53} & \ptz\ptz\textbf{138.56}  \\
\midrule

%%%% 300k-mol
% \rowcolor{Gray}\cellcolor{white}
% & \texttt{1e} & \ptz\ptz0.08 & \ptz\ptz\ptz1.89 & 99.99 & \ptz\ptz\ptz\ptz1.22 & \ptz\ptz\ptz0.74 & \ptz\ptz\ptz\ptz1.19 \\
% & QHNet    & 120.10  & 2182.06  & 89.63 & - & - & - \\
& QHNet$^*$& 121.39\ptp{0.001}  & 5554.36\ptp{0.001}  & 86.02\ptp{0.001} & 53505.09\ptp{0.001}& 4352.76\ptp{0.001} & 50424.86\ptp{0.001} \\
& SPHNet   & 108.19\ptp{0.001}  & 1724.10\ptp{0.001}  & 91.49\ptp{0.001}  & - & - & -  \\

% \RC& \textbf{Ours}     & \ptz\underline{38.14}  & \ptz\underline{282.74}  & \underline{98.79} & \ptz\underline{1237.48} & \ptz\underline{316.78} & \ptz\underline{1403.95}  \\

\RC& \textbf{Ours}     & \ptz\textbf{45.91}\tp{0.001}  & \ptz\underline{442.56}\tp{0.171}  & \underline{98.65}\tp{0.001} & \ptz\underline{1344.68}\tp{2.338} & \ptz\underline{479.71}\tp{0.150} & \ptz\underline{1605.03}\tp{2.286}  \\

\RC\multirow{-4}{*}{\shortstack{QH9-dynamic\\ (300k-\texttt{mol})}} 
& \textbf{Ours (WA-FT)}     & \ptz\underline{46.60}\tp{0.003}  & \ptz\textbf{424.75}\tp{0.324}  & \textbf{98.74}\tp{0.001} & \ptz\ptz\textbf{912.10}\tp{2.941} & \ptz\textbf{403.51}\tp{1.861} & \ptz\textbf{1047.88}\tp{2.683} \\

% & \textbf{Ours (WAD-FT)}     & \ptz\textbf{25.64}  & \ptz\textbf{111.21}  & \textbf{99.27} & \ptz\ptz\textbf{212.36} & \ptz\textbf{118.53} & \ptz\ptz\textbf{218.32} \\

\bottomrule
\end{tabular}}
\end{table}

% 0.46635
% 0.47034
% 0.49252
% 0.23689
% --
% 0.416525
% 0.583475

==> table/unuse/qh9_variance_small.tex <==
\begin{wraptable}{R}{6.2cm}
\vspace{-12pt}
\centering
\captionof{table}{\textbf{Predictive variance of \QHFlow.}}
\label{tab:qh9_flow_variance_small}
\resizebox{\linewidth}{!}{ % Optional: resize if space is limited
\begin{tabular}{llccc}
\toprule
\textbf{Data} & \textbf{Model} & $H \downarrow$ $[\mu E_h]$ & \OCC $\downarrow$ $[\mu E_h]$ & \SC $\uparrow$ $[\%]$ \\
\midrule\midrule
\arrayrulecolor{gray}
& Ours & \textbf{22.95}\tp{0.001} & {119.67}\tp{0.211} & {99.51}\tp{0.001} \\
\multirow{-2}{*}{\texttt{id}}& 
WA-FT &  {23.85}\tp{0.001} & \textbf{101.92}\tp{0.279} & \textbf{99.56}\tp{0.002} \\
\midrule

& Ours & \textbf{20.01}\tp{0.001} & \ptz{84.54}\tp{0.007} & {99.04}\tp{0.003} \\
\multirow{-2}{*}{\texttt{ood}}& 
WA-FT &  {20.55}\tp{0.002} & \ptz\textbf{72.64}\tp{0.018} & \textbf{99.16}\tp{0.006} \\
\midrule

& Ours & \textbf{25.94}\tp{0.001} & 103.26\tp{0.031} & {99.59}\tp{0.001} \\
\multirow{-2}{*}{\texttt{geo}}& 
WA-FT &  {27.12}\tp{0.002} & \ptz\textbf{89.03}\tp{0.213} & \textbf{99.65}\tp{0.001} \\
\midrule

& Ours & \textbf{45.91}\tp{0.001} & {443.56}\tp{0.171} & {98.65}\tp{0.001} \\
\multirow{-2}{*}{\texttt{mol}}& 
WA-FT &  {46.60}\tp{0.001} & \textbf{424.75}\tp{0.324} & \textbf{98.74}\tp{0.001} \\
\arrayrulecolor{black}

\bottomrule
\end{tabular}
 }
% \vspace{-10pt}
\end{wraptable}


==> table/unuse/qh9_variance_tiny.tex <==
\begin{wraptable}{R}{6cm}
\vspace{-12pt}
\centering
\captionof{table}{\textbf{Prediction variance of \QHFlow}}
\label{tab:qh9_flow_variance_small}
\resizebox{\linewidth}{!}{ % Optional: resize if space is limited
\begin{tabular}{llcc}
\toprule
\textbf{Dataset} & \textbf{Model} & $H \downarrow$ $[\mu E_h]$ & \OCC $\downarrow$ $[\mu E_h]$  \\
\midrule\midrule
& Ours & \textbf{22.95}\tp{0.001} & {119.67}\tp{0.211} \\
\multirow{-2}{*}{\texttt{id}}& 
WA-FT &  {23.85}\tp{0.001} & \textbf{101.92}\tp{0.279} \\
\midrule

& Ours & \textbf{20.01}\tp{0.001} & \ptz{84.54}\tp{0.007} \\
\multirow{-2}{*}{\texttt{ood}}& 
WA-FT &  {20.55}\tp{0.002} & \ptz\textbf{72.64}\tp{0.018} \\
\midrule

& Ours & \textbf{25.94}\tp{0.001} & 103.26\tp{0.031} \\
\multirow{-2}{*}{\texttt{geo}}& 
WA-FT &  {27.12}\tp{0.002} & \ptz\textbf{89.03}\tp{0.213}\\
\midrule

& Ours & \textbf{45.91}\tp{0.001} & {443.56}\tp{0.171}\\
\multirow{-2}{*}{\texttt{mol}}& 
WA-FT &  {46.60}\tp{0.001} & \textbf{424.75}\tp{0.324}  \\
\bottomrule
\end{tabular}
}
\vspace{-10pt}
\end{wraptable}

